AF Embeddability of the C*-Algebra of a Deaconu-Renault Groupoid

We study Deaconu-Renault groupoids corresponding to surjective local homeomorphisms on locally compact, Hausdorff, second countable, totally disconnected spaces, and we characterise when the C*-algebras of these groupoids are AF embeddable. Our main result generalises theorems in the literature for graphs and for crossed products of commutative C*-algebras by the integers. We give a condition on the surjective local homeomorphism that characterises the AF embeddability of the C*-algebra of the associated Deaconu-Renault groupoid. In order to prove our main result, we analyse homology groups for AF groupoids, and we prove a theorem that gives an explicit formula for the isomorphism of these groups and the corresponding K-theory. This isomorphism generalises Farsi, Kumjian, Pask, Sims (M\"unster J. Math, 2019) and Matui (Proc. Lond. Math. Soc, 2012), since we give an explicit formula for the isomorphism and we show that it preserves positive elements.

==> binding.tex <==
\chapter{Binding}\label{C:bin}

The Library states:
\begin{itemize}
\item Thesis must be fully bound and cased in cloth or buckram in optional colour. (I think they mean you can pick the colour!)
\item Author's surname and initials and (short) title lettered on spine. (The thesis's title, not the author's, presumably.)
\item Author's full name and full title lettered on front cover. (Again, the thesis's title, not the author's, presumably.)
\item Two copies of a PhD thesis and one copy of a Master's thesis must be deposited. A signed availability slip must accompany the thesis.
\item  The principal supervisor is responsible for the deposit.
\end{itemize}

==> delete/DELETEcrossedproducts-covariant.tex <==
\subsection{Covariant homomorphisms}
\label{section:crossedproducts:covariant}

We will define the notion of covariant homomorphism, and we will see in Proposition \ref{prop:covariant} that we can use this to obtain a homomorphism from the crossed product $A \rtimes_\alpha Z$ to a multiplier algebra. In the next subsection, we will use a covariant homomorphism to find the isomorphism $C^*(G) \rtimes_\alpha \mathbb{T} \cong C^*(G(c))$.

%We will define the notion of covariant homomorphism of a dynamical system into a multiplier algebra, and we will see how this homomorphism can be used to obtain a homomorphism between the crossed product and the same multiplier algebra. The results in this subsection will be important to study the isomorphism $C^*(G(c)) \cong C^*(G) \rtimes_{\alpha^c} \mathbb{T}$.

\begin{definition}
Let $\alpha: Z \rightarrow A$ be a dynamical system and let $B$ be a C*-algebra. Then a \newterm{covariant homomorphism} of $(A, Z, \alpha)$ into $M(B)$ is a pair $(\pi,u)$ consisting of a homomorphism $\pi: A \rightarrow M(B)$ and a strongly continuous unitary-valued homomorphism $u: Z \rightarrow UM(B)$ such that
\begin{align*}
\pi(\alpha_z(a)) = u_z \pi(a) u_z^*
\hspace{20pt}
\text{$z \in Z$, $a \in A$}.
\end{align*}
\end{definition}

Note that the definition above is defined in \cite[Definition 2.37]{Williams-crossedproducts} for $\mathcal{L}(X)$, where $X$ is a Hilbert $B$-module, which generalises our definition, as explained in \cite[Remark 2.38]{Williams-crossedproducts}.

Note that the notion of covariant homomorphism is analogous to the idea of covariant representation introduced by Definition \ref{def:covariantrepresentation}.

The following proposition shows that a covariant homomorphism induces a homomorphism from $A \rtimes_\alpha Z$ to $M(B)$.

\begin{proposition}
\cite[Proposition 2.39]{Williams-crossedproducts}
\label{prop:covariant}
Suppose that $\alpha: Z \rightarrow \mathrm{Aut}\hphantom{.}A$ is a dynamical system, and let $B$ be a C*-algebra. Fix a Haar measure $\mu$ on $Z$. If $(\pi,u)$ is a covariant homomorphism of $(A, Z, \alpha)$ into $M(B)$, then there exists a unique homomorphism $\pi \rtimes u: A \rtimes_\alpha Z \rightarrow M(B)$ such that
\begin{align*}
\pi \rtimes u(f) = \int_Z \pi(f(z))u_z d\mu(z)
\hspace{20pt}\text{$f \in C_c(Z, A)$}.
\end{align*}
\end{proposition}


==> delete/K0H0-AFbundles.tex <==
\subsection{AF bundles}
\label{subsection:K0H0:AFbundles}

Now we introduce a new class of C*-bundles, called AF bundles. For an AF bundle $\mathcal{A}$, the corresponding C*-algebra $\Gamma_0(\mathcal{A})$ is an inductive limit of C*-algebras that are locally isomorphic to C*-algebras of the form $C(V, M_n)$. This property will allow us in the next subsection to study the K-theory of $\Gamma_0(\mathcal{A})$ by applying results for $C(V, M_n)$.

We will also prove Theorem \ref{thm:AFbundlecondition} which is an analogue of Fell's theorem, in the sense that it provides conditions for which a surjection $\vartheta: \mathcal{A} \rightarrow X$ determines an AF bundle uniquely.

The notion of local representations, defined below, will be fundamental in the definition of AF bundles.

\begin{definition}
\label{def:localrepresentation}
Let $X$ be a locally compact Hausdorff second countable totally disconnected space. Let $\vartheta: \mathcal{A} \rightarrow X$ be a surjection such that $\mathcal{A}_x = \vartheta^{-1}(x)$ is a C*-algebra for all $x \in X$. Let $\Gamma$ be a subset of (not necessarily continuous) sections $f: X \rightarrow \mathcal{A}$. Let $\lbrace m_k \rbrace_{k \geq 1}$ be a sequence of natural numbers greater than zero. Define the set of indices
\begin{align*}
I = \lbrace (k,l) \in \mathbb{N}^2: k \geq 1, 1 \leq l \leq m_k \rbrace.
\end{align*}
We say that $(\Gamma_k, V_{k,l}, \alpha_{k,l}, n_{k,l})_{(k,l) \in I}$ is a \newterm{local representation} of $\Gamma$ if
\begin{enumerate}[(i)]
\item $\Gamma = \bigcup_{k=1}^\infty \Gamma_k$ is an increasing union of the C*-algebras $\Gamma_k$.

\item For every $k \geq 1$, $V_{k,1}, V_{k,2}, \hdots, V_{k,m_k}$ are disjoint compact open subsets of $X$ such that
\begin{align*}
V_{k,1} \cup \hdots \cup V_{k,m_k}
\subset
V_{k+1,1} \cup \hdots \cup V_{k+1,m_{k+1}},
\end{align*}
and that $V_{k,1} \cup \hdots \cup V_{k,m_k}$ is the \newterm{support} of $\Gamma_k$, i.e
\begin{align*}
\bigcup_{l=1}^{m_k} V_{k,l} = \overline{\lbrace x \in X: \text{  $\exists f \in \Gamma_k$ with $\Vert f(x) \Vert > 0$}\rbrace}.
\end{align*}

\item For $(k, l) \in I$, $\alpha_{k,l}: \Gamma\vert_{V_{k,l}} \rightarrow C(V_{k,l}, M_{n_{k,l}})$ is an isomorphism. Moreover, $\alpha_{k,l}$ is \newterm{support preserving}, i.e., for $f \in \Gamma_{k}\vert_{V_{k,l}}$ and $x \in V_{k,l}$, we have
\begin{align*}
f(x) = 0 \Leftrightarrow \alpha_{k,l}(f)(x) = 0.
\end{align*}
\end{enumerate}
When we believe there is little risk of confusion, we use the notation $\Gamma_{k,l} = \Gamma_k\vert_{V_{k,l}}$.
\end{definition}

\begin{remark}
Note that $\Gamma$ in Definition \ref{def:AFbundle} is a $\ast$-algebra, since it is an increasing union of C*-algebras.
\end{remark}

Now we can define AF bundles.

\begin{definition}
\label{def:AFbundle}
Let $\vartheta: \mathcal{A} \rightarrow X$ be a C*-bundle such that $X$ is totally disconnected. We say that this C*-bundle is \newterm{AF} (or an \newterm{AF bundle}) if $\Gamma_0(\mathcal{A})$ has a dense subset $\Gamma$ such that $\Gamma$ has a local representation.
\end{definition}

\begin{remark}
We have chosen the name AF bundles because, in some sense, the definition is analogous to the notion of AF algebras. Recall that an AF algebra $A$ is an inductive limit of an increasing union of C*-algebras $A_k$ with $A_k \cong M_{n_1} \oplus \cdots \oplus M_{n_k}$ (see Chapter III of Davidson's book \cite{Davidson} for more details). Similarly, if $\vartheta: \mathcal{A} \rightarrow X$ is an AF bundle, there exists a dense $\ast$-subalgebra $\Gamma$ of $\Gamma_0(\mathcal{A})$ that is an increasing of C*-algebras $\Gamma_k$ with
\begin{align*}
\Gamma_k \cong C(V_{k,1}, M_{n_{k,1}}) \oplus \cdots \oplus C(V_{k, m_k}, M_{n_{k, m_k}}).
\end{align*}
\end{remark}

In Subsection \ref{subsection:K0H0:bundles}, Fell's theorem (Theorem \ref{thm:Fell}) studies when a surjection $\vartheta: \mathcal{A} \rightarrow X$ is a C*-bundle. Here we want to do the same for AF bundles. Given the surjection $\vartheta$ and a subset $\Gamma$ of sections, with a local representation, we will give a condition that makes $\mathcal{A}$ an AF bundle where $\Gamma$ is dense in $\Gamma_0(\mathcal{A})$. In order to prove this property, we will need to check the conditions of Fell's theorem and Proposition \ref{prop:Gammadense}.

The following lemma will be used to check condition (a) of Fell's theorem.

\begin{lemma}
\label{lemma:supportpreservingnorm}
Let $X$ be a locally compact Hausdorff second countable space. Let $\vartheta: \mathcal{A} \rightarrow X$ be a surjection such that $\mathcal{A}_x = \vartheta^{-1}(x)$ is a C*-algebra for all $x \in X$. Let $\Gamma$ be a set containing some sections of $\vartheta: \mathcal{A} \rightarrow X$, and equip $\Gamma$ with the pointwise operations. Suppose that there exists a support preserving isomorphism $\alpha: \Gamma \rightarrow C(V, M_n)$ for some $n \geq 1$ and a compact open $V \subset X$. Then
\begin{align}
\label{eqn:supportpreservingnorm}
\Vert \alpha(f)(x) \Vert
= \Vert f(x) \Vert
\hspace{20pt}
\text{for $x \in V$, $f \in \Gamma$.}
\end{align}
\end{lemma}
\begin{proof}
In this proof we will use quotient C*-algebras (see \cite[Theorems 1.1.1 and 3.1.4]{Murphy}). We will find two closed ideals $I_x \subset \Gamma$ and $J_x \subset C(V, M_n)$ such that $\Gamma / I_x \cong C(V, M_n)/ J_x$ with respect to the map $f + I_x \mapsto \alpha(f) + J_x$. Moreover, we will study the norm on these quotient algebras to prove that
\begin{align*}
\Vert f(x) \Vert = \Vert f + I_x \Vert = \Vert \alpha(f) + J_x \Vert = \Vert \alpha(f)(x) \Vert.
\end{align*}

Fix $x \in X$ and let $I_x = \lbrace f \in \Gamma : f(x) = 0 \rbrace$. By the isomorphism $\alpha$, we have that $\Gamma$ is a C*-algebra and has norm
\begin{align*}
\Vert f \Vert
= \Vert \alpha(f) \Vert
= \sup_{x \in X} \Vert \alpha(f)(x) \Vert
\hspace{20pt}
\text{for }f \in \Gamma.
\end{align*}

Fix $x \in V$ and let $I_x = \lbrace f \in \Gamma: f(x) = 0 \rbrace$. Then $I_x$ is an ideal of $\Gamma$. We want to study the quotient $\Gamma/I_x$, so we need to guarantee that $I_x$ is a closed ideal of $\Gamma$.

We show that $I_x$ is closed. Let $\lbrace f_n \rbrace_{n \geq 1}$ be a sequence in $I_x$ converging to some $f \in \Gamma$. Then $\alpha(f_n) \rightarrow \alpha(f)$. By definition of the norm on $C(V, M_n)$, we have
\begin{align*}
\Vert \alpha(f)(x) \Vert
= \lim_{n \rightarrow \infty} \Vert \alpha(f_n)(x) \Vert = 0.
\end{align*}
Because $\alpha$ is support preserving, the equation above implies that $f(x) = 0$. Hence $I_x$ is a closed ideal of $\Gamma$.

Next we show that the norm in $\Gamma/I_x$ is defined by $\Vert f + I_x \Vert = \Vert f(x) \Vert$ for $f \in \Gamma$. Let $\mathcal{B}_x = \lbrace f(x) : f \in \Gamma \rbrace \subset \mathcal{A}_x$. Note that $\mathcal{B}_x$ is a $\ast$-algebra. In order to show that $\Vert f(x) \Vert = \Vert f + I_x \Vert$, we only need to show that $\mathcal{B}_x$ is $\ast$-isomorphic to $\Gamma/I_x$.

Let $\lambda: \mathcal{B}_x \rightarrow \Gamma/I_x$ be defined by
\begin{align*}
\lambda(f(x)) = f + I_x
\hspace{20pt}\text{for }
f \in \Gamma.
\end{align*}
Note that $\lambda$ is well-defined. In fact, if $f_1, f_2 \in \Gamma$ are such that $f_1(x) = f_2(x)$, then
\begin{align*}
\lambda(f_1) = f_1 + I_x = f_2 + I_x = \lambda(f_2).
\end{align*}
Applying the definition, we have that $\lambda$ is an isomorphism. Therefore $\Vert f + I_x \Vert = \Vert f(x) \Vert$ for $f \in \Gamma$.

Now we define the closed ideal $J_x \subset C(V, M_n)$. Let $J_x = \alpha(I_x)$. Then, since $\alpha$ is an isomorphism, we have
\begin{align*}
J_x = \lbrace g \in C(V,M_n) : g(x) = 0 \rbrace.
\end{align*}
Since $\alpha$ is an isomorphism, we have that $J_x$ is a closed ideal of $C(V,M_n)$. Also, $C(V, M_n)/J_x$ is a C*-algebra. By the same ideas used to find the norm of $\Gamma/I_x$, we will prove that
\begin{align*}
\Vert g + J_x \Vert
%= \inf_{h \in J_x} \Vert g + h \Vert
= \Vert g(x) \Vert
\hspace{20pt}\text{for }g \in C(V,M_n),
\end{align*}
Define the map $\mu: C(V, M_n)/J_x \rightarrow M_n$ by
\begin{align*}
\mu(g + J_x) = g(x)
\hspace{20pt}\text{for }g \in C(V,M_n)
\end{align*}
By the same arguments used for $\lambda$, we have that $\mu$ is an isomorphism. It follows that $\Vert g + J_x \Vert = \Vert g(x) \Vert$ for all $g \in C(V, M_n)$.

Next we study the isomorphism $\Gamma/I_x \cong C(V, M_n) /J_x$ and prove the rest of the lemma. Note that $\alpha$ induces an isomorphism of $\alpha_x: \Gamma/I_x \rightarrow C(V,M_n)/J_x$ given by
\begin{align*}
\alpha_x(f + I_x) = \alpha(f) + J_x
\hspace{20pt}\text{for }f \in \Gamma.
\end{align*}
Hence, for $f \in \Gamma$, we have
\begin{align*}
\Vert f(x) \Vert
= \Vert f + I_x \Vert
= \Vert \alpha_x(f + I_x) \Vert
= \Vert \alpha(f) + J_x \Vert
= \Vert \alpha(f)(x) \Vert. \tag*{\qedhere}
\end{align*}
\end{proof}

The lemma below will be used to check condition (a) of Proposition \ref{prop:Gammadense}. Recall that we need this to find a condition that makes a surjection $\vartheta: \mathcal{A} \rightarrow X$ an AF bundle.

\begin{lemma}
\label{lemma:varphif}
Let $X$ be a locally compact Hausdorff second countable totally disconnected space. Let $\vartheta: \mathcal{A} \rightarrow X$ be a surjection such that $\mathcal{A}_x = \vartheta^{-1}(x)$ is a C*-algebra for all $x \in X$. Let $\Gamma$ be a subset of (not necessarily continuous) sections $f: X \rightarrow \mathcal{A}$ such that there exists a compact open set $V \subset X$ and a support preserving isomorphism $\alpha:  \Gamma \rightarrow C(V, M_n)$ for some $n \geq 1$. Then, for every $f \in \Gamma$ and $\varphi \in C_0(X)$, we can define the product $\varphi \cdot f \in \Gamma$ by
\begin{align*}
\varphi \cdot f (x) = \varphi(x) f(x)
\hspace{20pt}\text{for }x \in X.
\end{align*}
\end{lemma}
\begin{proof}
Let $f \in \Gamma$ and $\varphi \in C_0(X)$. It follows from the continuity of $\varphi$ that $\varphi\vert_V \cdot \alpha(f) \in C(V, M_n)$. Here $\varphi\vert_V$ is the restriction of $\varphi$ to $V$. Also, the product is defined by
\begin{align*}
\varphi\vert_V \cdot \alpha(f)(x)
= \varphi(x)\alpha(f)(x)
\hspace{20pt}
\text{for }x \in V.
\end{align*}
Let $g = \alpha^{-1}(\varphi\vert_V \cdot \alpha(f)) \in \Gamma$. We will prove that $g = \varphi \cdot f$.

Since $X$ is totally disconnected, we can choose a sequence of locally constant functions $\varphi_k \in C_0(X)$ with support in $V$ such that $\varphi_k\vert_V = \varphi_k$ converges to $\varphi\vert_V$ in the supremum norm. Note that, for each $k$, we can write $\varphi_k \cdot f$ as a linear combination of elements in $\Gamma$. This implies that $\varphi_k \cdot f \in \Gamma$. Moreover, $\alpha(\varphi_k \cdot f) = \varphi_k\vert_V \cdot \alpha(f)$.

By Lemma \ref{lemma:supportpreservingnorm}, we have for every $k \geq 1$,
\begin{align}
\Vert \varphi_k \cdot f - g \Vert
&= \Vert \alpha(\varphi_k \cdot f) - \alpha(g) \Vert \nonumber\\
&= \Vert \varphi_k \cdot \alpha(f) - \alpha \circ \alpha^{-1}(\varphi\vert_V \cdot \alpha(f)) \Vert \nonumber\\
&= \Vert \varphi_k \cdot \alpha(f) - \varphi\vert_V \cdot \alpha(f) \Vert \nonumber\\
&= \Vert (\varphi_k - \varphi_V) \cdot \alpha(f) \Vert \nonumber\\
&\leq \Vert (\varphi_k - \varphi\vert_V)1_V \Vert \Vert \alpha(f) \Vert \nonumber\\
&= \Vert \varphi_k - \varphi\vert_V \Vert_\infty \Vert f \Vert. \label{eqn:varphikf}
\end{align}
Since $\Vert \varphi_k - \varphi\vert_V \Vert_\infty \rightarrow 0$, the inequality \eqref{eqn:varphikf} implies that $\Vert \varphi_k \cdot f - g \Vert \rightarrow 0$ as $k \rightarrow \infty$. Then, for each $x \in V$,
\begin{align*}
g(x)
= \lim_{k \rightarrow \infty} \varphi_k(x) f(x)
= \varphi(x) f(x).
\end{align*}
By the same limit argument, given $x \in X\setminus V$, we have $g(x) = 0$. Therefore $g = \varphi \cdot f \in \Gamma$.
\end{proof}

Finally, we find a condition that makes $\vartheta: \mathcal{A} \rightarrow X$ an AF bundle.

\begin{theorem}
\label{thm:AFbundlecondition}
Let $X$ be a locally compact Hausdorff second countable totally disconnected space. Let $\vartheta: \mathcal{A} \rightarrow X$ be a surjection such that $\mathcal{A}_x = \vartheta^{-1}(x)$ is a C*-algebra for all $x \in X$. Let $\Gamma$ be a subset of sections $f: X \rightarrow \mathcal{A}$ such that, for all $x \in X$, $\Gamma(x)$ is dense in $\mathcal{A}_x$. Let $(\Gamma_k, V_{k,l}, \alpha_{k,l}, n_{k,l})_{(k,l) \in I}$ be a local representation of $\Gamma$. Then there exists a unique topology on $\mathcal{A}$ such that $\vartheta: \mathcal{A} \rightarrow X$ is a C*-bundle. Moreover, $\mathcal{A}$ is AF and $\Gamma$ is dense in $\Gamma_0(\mathcal{A})$.
\end{theorem}
\begin{proof}
We want to apply Fell's Theorem (Theorem \ref{thm:Fell}) to show that $\mathcal{A}$ is a C*-bundle.

First we check condition (a) of the theorem. Let $f \in \Gamma$ be a section. Then there exists $k \geq 1$ such that $f \in \Gamma_k$. Let $x \in X$ be in the support of $\Gamma_k$. Then there exists a unique $l$ such that $x \in V_{k,l}$.

By Lemma \ref{lemma:supportpreservingnorm}, we have
\begin{align*}
\Vert \alpha_{k,l}(f)(y) \Vert
= \Vert f(y) \Vert
\hspace{20pt}
\text{for $y \in V_{k,l}$.}
\end{align*}
Also, $\alpha_{k,l}(f) \in C(V_{k,l}, M_{n_{k,l}})$. This implies that the map $y \mapsto \Vert f(y) \Vert$ is continuous at $x$.

Now let $x \in X$ be outside the support of $\Gamma_k$. Since this support is compact open, its complement is open. Then there exists an open neighbourhood $V$ of $x$ such that $f(y) = 0$ for all $y \in V$. This implies that the map $y \mapsto \Vert f(y) \Vert$ is continuous at $x$. Therefore, then condition (a) of Theorem \ref{thm:Fell} holds.

Note that condition (b) of Fell's theorem is satisfied by assumption. Therefore, by Fell's theorem, there exists a unique topology on $\mathcal{A}$ such that $\vartheta: \mathcal{A} \rightarrow X$ is a C*-bundle over $X$ with $\Gamma \subset \Gamma(\mathcal{A})$.

We still need to show that $\Gamma$ is dense in $\Gamma_0(\mathcal{A})$. Note that $\Gamma \subset \Gamma_0(\mathcal{A})$. In fact, given $f \in \Gamma$, we have already proved that $f \in \Gamma(\mathcal{A})$. Moreover, using the local representation of $\Gamma$, there exists $k$ such that $f \in \Gamma_k$. This implies that $f$ is supported on the compact set $V_{k,1} \cup \hdots \cup V_{k,m_k}$.

In order to show that $\Gamma$ is dense in $\Gamma_0(\mathcal{A})$, we only need to prove condition (a) of Proposition \ref{prop:Gammadense}. However, this condition is true by Lemma \ref{lemma:varphif}. Therefore, $\Gamma$ is dense in $\Gamma_0(\mathcal{A})$, which implies that $\vartheta: \mathcal{A} \rightarrow X$ is an AF bundle.
\end{proof}


==> delete/K0H0-C0XMn.tex <==
\subsection{Projections in $C_0(X, M_n)$}
\label{subsection:K0H0:C0XMn}

Here we study the equivalence of projections in $C_0(X, M_n)$, and we will see that two projections are equivalent if, and only if, they have the same trace. First we study the K-theory of $M_n$ and then we generalise the results for $C_0(X, M_n)$.

%Here we prove Proposition \ref{prop:traceCXMn}, that generalises \cite[Exercise 3.4]{RLL-Ktheory}, where the equivalence $(b) \Leftrightarrow (c)$ is shown for $X$ compact.

We begin by defining the trace on $M_n$.
\begin{definition}
Let $\mathrm{tr}: M_n \rightarrow \mathbb{C}$ be the standard trace given by
\begin{align*}
\mathrm{tr}
\begin{bmatrix}
a_{11} & a_{12} & \cdots & a_{1n} \\
a_{21} & a_{22} & \cdots & a_{2n} \\
\vdots & \vdots & \ddots & \vdots \\
a_{n1} & a_{n2} & \cdots & a_{nn}
\end{bmatrix}
= \sum_{i=1}^n a_{ii}.
\end{align*}
We call $\tr a$ the \newterm{trace} of $a \in M_n$.
\end{definition}

\begin{remark}
\label{rmk:traceproperty}
Note that $\mathrm{tr}(ab) = \mathrm{tr}(ba)$ for $a,b \in M_n$. In fact,
\begin{align*}
\mathrm{tr}(ab)
= \sum_{i=1}^n (ab)_{ii}
= \sum_{i=1}^n \sum_{j=1}^n a_{ij} b_{ji}
= \sum_{j=1}^n \sum_{i=1}^n b_{ji} a_{ij}
= \sum_{j=1}^n (ba)_{jj}
= \mathrm{tr}(ba).
\end{align*}
\end{remark}

In order to study the equivalence of projections in $M_n$, we will need the following result:
\begin{theorem} (Schur's lemma) \cite[Theorem 10.14]{PiziakOdell}
Let $a \in M_n$. Then there is a unitary matrix $u$ such that $\Lambda = u^*au$ is upper triangular. Moreover, the eigenvalues of $a$ (possibly repeated) comprise the diagonal elements of $\Lambda$.
\end{theorem}

\begin{corollary}
\label{corollary:psumv}
Let $p \in M_n$ be a projection with trace $k$. Then there are $k$ orthonormal vectors $v_1, \hdots, v_k$ such that $p = \sum_{i=1}^k v_i v_i^*$.
\end{corollary}
\begin{proof}
By Schur's lemma, there exists a unitary matrix and an upper triangular matrix $\Lambda$ such that $p = u \Lambda u^*$. Since $p$ is self-adjoint, we have that $\Lambda$ is diagonal. Moveover, the fact that $p$ is a projection implies that the elements in the diagonal of $\Lambda$ are zeros and ones.

Let $k$ be the trace of $p$. Then $k = \tr u \Lambda u^* = \tr \Lambda$ is the number of ones of $\Lambda$. We can assume that the first $k$ elements of $\mathrm{diag}\hphantom{.} \Lambda$ are ones (If this is not the case, we can find an elementary matrix $e$ such that $\widetilde{\Lambda} = e^{-1} \Lambda e$ has this property and $p = \widetilde{u} \widetilde{\Lambda} \widetilde{u}^*$ with $\widetilde{u} = u e$).

For each $i = 1, \hdots, n$, let $v_i$ be the $i^{\mathrm{th}}$ column of $u$. Then, if $i \leq k$,
\begin{align*}
pv_i = u \Lambda u^* v_i = u \Lambda e_i = u e_i = v_i
\hspace{15pt}&\text{and}\hspace{15pt}
\sum_{l=1}^k v_l v_l^* v_i = v_i. %\label{eqn:psumv1}
%\end{align*}
\intertext{If $i > k$,}
%\begin{align*}
pv_i = u \Lambda u^* v_i = u \Lambda e_i = 0
\hspace{15pt}&\text{and}\hspace{15pt}
\sum_{l=1}^k v_l v_l^* v_i = 0. %\label{eqn:psumv1}
\end{align*}
Since $v_1, \hdots, v_n$ form an orthonormal basis of $\mathbb{C}^n$, we have $p = \sum_{l=1}^k v_l v_l^*$.
\end{proof}

\begin{remark}
\label{rmk:dimp}
Note that this corollary implies that $\tr p$ is the dimension of $p(\mathbb{C}^k)$.
\end{remark}

\begin{remark}
\label{rmk:idsumv}
By the similar calculations of Corollary \ref{corollary:psumv}, we can prove that for $v_1, \hdots, v_n$ orthonormal basis of $\mathbb{C}^n$, we have $\mathrm{id} = \sum_{i=1}^n v_i v_i^*$.
\end{remark}

Now we prove the connection between the trace and the equivalence of projections in $M_n$. The equivalence $(ii) \Leftrightarrow (i)$ of the next lemma is Exercise 2.9 of R{\o}rdan, Larsen and Laustsen's book \cite{RLL-Ktheory}.
\begin{lemma}
\label{lemma:matrixtrace}
%\cite[Execise 2.9]{RLL-Ktheory}
Let $p, q$ be projections in $M_n$. Then the following are equivalent:
\begin{enumerate}[(i)]
\item $p \sim q$,
\item $\mathrm{tr}(p) = \mathrm{tr}(q)$,
\item $p \sim_u q$.
\end{enumerate}
\end{lemma}
\begin{proof}
First we show $(i) \Rightarrow (ii)$. Let $p, q \in M_n$ be two projections with $p \sim q$. Then there exists $v \in M_n$ with $p = v^*v$ and $q = vv^*$. Then
\begin{align*}
\tr p = \tr u^*u = \tr uu^* = \tr q.
\end{align*}

Now we prove $(ii) \Rightarrow (iii)$. Let $p,q \in M_n$ be projections with the same trace $k$. By Corollary \ref{corollary:psumv}, there are $v_1, \hdots, v_k$ orthonormal and $w_1, \hdots, w_k$ orthonormal such that
\begin{align*}
p = \sum_{i=1}^k v_i v_i^*
\hspace{15pt}\text{and}\hspace{15pt}
q = \sum_{i=1}^k w_i w_i^*
\end{align*}
Find $w_{k+1}, \hdots, w_n$ and $v_{k+1}, \hdots, v_n$ such that both $v_1, \hdots, v_n$ and $w_1, \hdots, w_n$ are orthonormal basis of $\mathbb{C}^n$. Let $u = \sum_{i=1}^n w_i v_i^*$. Then $u$ is unitary. In fact, by Remark \ref{rmk:idsumv},
\begin{align*}
u^*u = \sum_{i=1}^n w_i w_i^* = \mathrm{id}
\hspace{15pt}\text{and}\hspace{15pt}
uu^* = \sum_{i=1}^n v_i v_i^* = \mathrm{id}.
\end{align*}
Also, $p = u^* q u$. Indeed,
\begin{align*}
u^* q u
&= \sum_{i=1}^n v_i w_i^* q u \\
&= \sum_{i=1}^n v_i w_i^* \left( \sum_{j=1}^k w_j w_j^* \right) u \\
&= \sum_{i=1}^k v_i w_i^* w_i w_i^* u
\hspace{15pt}\text{since the $w_i$ are orthonormal}\\
&= \sum_{i=1}^k v_i w_i^* u \\
&= \sum_{i=1}^k v_i w_i^* \sum_{j=1}^n w_j v_j^* \\
&= \sum_{i=1}^k v_i w_i^* w_i v_i^* \\
&= \sum_{i=1}^k v_i v_i^* \\
&= p.
\end{align*}
Then $(iii)$ holds.

Finally, we show $(iii) \Rightarrow (i)$. If $(iii)$ is true, there exists a unitary such that $p = u^* q u$. Then $q = upu^*$. Let $v = up$. Then $v^*v = p$ and $vv^* = q$. Therefore $p \sim q$.
\end{proof}

\begin{remark}
Note that the implication $(iii) \Rightarrow (i)$ of the Lemma above is a known result for more general C*-algebras. See \cite[Proposition 2.2.7]{RLL-Ktheory}.
\end{remark}
Now that we know the connection between the trace and projections in $M_n$, we want to generalise this for $C_0(X, M_n)$ when $X$ has certain topological properties.

The following proposition will be used to show that, for a projection $p \in C_0(X, M_n)$, the trace $\tr p$ is locally constant.

\begin{proposition} \cite[Propositions 2.2.4 and 2.2.7]{RLL-Ktheory}
\label{prop:closeprojections}
Let $p, q$ be projections in a C*-algebra $A$. If $\Vert p - q \Vert < 1$, then $p \sim_u q$.
\end{proposition}

Now we define the trace operator on $\mathcal{P}(C_0(X, M_n))$.

\begin{lemma}
\label{lemma:tracewelldefined}
Let $X$ be a locally compact Hausdorff second countable totally disconnected space, and let $n \geq 1$. Then there exists a map $\mathrm{tr}: \mathcal{P}(C_0(X, M_n)) \rightarrow C_c(X, \mathbb{N})$ given by
\begin{align}
\label{eqn:continuoustrace}
\mathrm{tr}(p)(x) = \mathrm{tr}(p(x)),
\end{align}
for $p \in \mathcal{P}(C_0(X, M_n))$ and $x \in X$. We denote $\mathrm{tr}(p)$ to be the \newterm{trace} of $p$.
\end{lemma}
\begin{proof}
It is straightforward from \eqref{eqn:continuoustrace} that the map is linear on $\mathcal{P}(C_0(X, M_n))$. So we only need to prove that it is well-defined.

\begin{itemize}
\item $\mathrm{tr}(p) \in C(X, \mathbb{N})$

Let $p \in \mathcal{P}(C_0(X, M_n))$. Given $x \in X$, Remark \ref{rmk:dimp} implies that
\begin{align*}
\mathrm{tr}(p)(x) = \mathrm{tr}(p(x)) = \dim (p(x)(\mathbb{C}^n)) \in \mathbb{N}.
\end{align*}
Then $\mathrm{tr}(p)$ assumes values in $\mathbb{N}$.

We still need to prove that $\mathrm{tr}(p)$ is continuous. Fix $x \in X$. Since $p$ is continuous, there exists an open neighbourhood $V \subset X$ of $x$ such that
\begin{align}
\label{eqn:tracewelldefined1}
\Vert p(x) - p(y) \Vert < 1
\text{\hspace{10pt}for }
y \in V.
\end{align}
Then, for $y \in V$, Proposition \ref{prop:closeprojections} and Lemma \ref{lemma:matrixtrace} imply that $\tr(p(x)) = \tr(p(y))$. Hence, $\mathrm{tr}(p)$ is constant on $V$. Since $x$ is arbitrary, we have that $\mathrm{tr}(p)$ is continuous, and then $\mathrm{tr}(p) \in C(X, \mathbb{N})$.

\item $\mathrm{tr}(p)$ is compactly supported

Let $p \in \mathcal{P}(C_0(X, M_n))$. Then there exists a compact subset $K \subset X$ such that
\begin{align}
\label{eqn:tracewelldefined2}
\Vert p(x) - 0 \Vert
= \Vert p(x) \Vert
< 1
\text{\hspace{10pt}for all }
x \in X \setminus K.
\end{align}
Let $x \in X \setminus K$. By \eqref{eqn:tracewelldefined2}, Proposition \ref{prop:closeprojections} and Lemma \ref{lemma:matrixtrace},
%. Lemma \ref{lemma:matrixtrace} implies that
\begin{align*}
\mathrm{tr}(p(x))
= \mathrm{tr}(0)
= 0.
\end{align*}
Hence $\mathrm{tr}(p)$ is compactly supported and, therefore, it is well-defined. \qedhere
\end{itemize}
\end{proof}

\begin{remark}
\label{rmk:projectioncompactlysupported}
Let $X$ be a locally compact Hausdorff second countable totally disconnected space. Note that every projection in $C_0(X, M_n)$ is an element of $C_c(X, M_n)$. In fact, let $p \in \mathcal{P}(C_0(X, M_n))$. By Lemma \ref{lemma:tracewelldefined}, its trace is compactly supported. Let $K$ be the compact support of $\mathrm{tr}(p)$. By Lemma \ref{lemma:matrixtrace}, we have that, for $x \in X \setminus K$,
\begin{align*}
\dim(p(x)\mathbb{C}^n)
= \mathrm{tr}(p(x))
= 0.
\end{align*}
Then $p(x) = 0$. Therefore $p \in C_c(X, M_n)$.
\end{remark}

%\begin{definition}
%Two projections $p, q$ in a C*-algebra $A$ are said to be \newterm{unitarily equivalent}, denoted $p \sim_u q$, when $p = u^*qu$ for a unitary $u \in \widetilde{A}$.
%\end{definition}

%\begin{proposition}
%\label{prop:usim}
%\cite[Proposition 5.2.10]{Wegge-Olsen-Ktheory}
%Let $p, q$ be two projections in a C*-algebra. If $p \sim_u q$, then $p \sim q$.
%\end{proposition}

Now we prove the main result of the subsection.

\begin{proposition}%{prop:traceCXMn}
\label{prop:traceCXMn}
Let $X$ be a locally compact Hausdorff second countable totally disconnected space. Let $p, q \in C_c(X, M_n)$ be two projections. Then the following are equivalent:
\begin{enumerate}[(i)]
\item $p \sim q$,
\item $\tr p = \tr q$,
\item For every compact subset $K \subset X$ such that $p, q$  vanish outside $K$, and there is a $u \in C_c(X, M_n)$ supported on $K$ such that
\begin{align*}
u^*u = uu^* = \mathrm{id} 1_K
\hspace{15pt}\text{and}\hspace{15pt}
 p = u^* q u.
\end{align*}
\end{enumerate}
\end{proposition}
\begin{proof}
Let us prove $(i) \Rightarrow (ii)$. Suppose that $p, q \in C_0(X, M_n)$ are two projections with $p \sim q$. Then there exists $v \in C_0(X, M_n)$ such that $p = v^*v$ and $q = vv^*$. Then, by Remark \ref{rmk:traceproperty} and by the definition of the trace on $C_0(X, M_n)$, we have $\mathrm{tr}(p) = \mathrm{tr}(q)$. Thus, $(ii)$ holds.

Now we prove $(ii) \Rightarrow (iii)$. Let $p, q \in C_c(X, M_n)$ be projections with the same trace. Remark \ref{rmk:projectioncompactlysupported} implies that $p, q \in C_c(X, M_n)$. Choose an arbitrary compact subset $K \subset X$ such that both $p$ and $q$ vanish outside $K$.

Since $p$ and $q$ are continuous, and using the topological properties of $K$, we can find a collection of elements $x_1, \hdots, x_m \in K$ and a partition $V_1, \hdots, V_m$ of $K$ by disjoint compact open subsets such that, for each $i = 1, \hdots, m$, we have
\begin{align}
\label{eqn:traceCXMn1}
x_i \in V_i,
\hspace{10pt}
\Vert p(y) - p(x_i) \Vert < \tfrac{1}{2},
\text{\hspace{10pt}and }
\Vert q(y) - q(x_i) \Vert < \tfrac{1}{2},
\text{\hspace{15pt}for }
y\in V_i.
\end{align}

Let $i = 1, \hdots, m$. By assumption, $\mathrm{tr}(p(x_i)) = \mathrm{tr}(q(x_i))$. It follows from Lemma \ref{lemma:matrixtrace} that there exists an unitary $v_i \in M_n$ such that $p(x_i) = v_i^* q(x_i) v_i$.

Let
\begin{align*}
\widetilde{p} = \displaystyle\sum_{i=1}^m p(x_i)1_{V_i},
\text{\hspace{10pt}}
\widetilde{q} = \displaystyle\sum_{i=1}^m q(x_i)1_{V_i}
\text{\hspace{10pt}and\hspace{10pt}}
v = \sum_{i=1}^m v_i 1_{V_i}.
\end{align*}
Then $\widetilde{p}$ and $\widetilde{q}$ are projections in $C_0(X, M_n)$. Also, $\widetilde{p} = v^* \widetilde{q} v$ and $v^*v = vv^* = \mathrm{id}1_K$.

Using the norm of $C_0(X, M_n)$, equation \eqref{eqn:traceCXMn1} implies that
\begin{align}
\label{eqn:traceCXMn2}
\Vert p - \widetilde{p} \Vert \leq \tfrac{1}{2}
\text{\hspace{10pt}and\hspace{10pt}}
\Vert q - \widetilde{q} \Vert \leq \tfrac{1}{2}.
\end{align}

Let $A \subset C_0(X, M_n)$ be the $\ast$-subalgebra of functions supported on $K$. Then $A$ is a unital C*-algebra with unit $\mathrm{id} 1_K$. By equation \eqref{eqn:traceCXMn2} and Proposition \ref{prop:closeprojections}, there are unitary elements $u_p, u_{q} \in A$ such that
\begin{align*}
p = u_p^* \widetilde{p} u_p
\hspace{15pt}\text{and}\hspace{15pt}
\widetilde{q} = u_{q}^* q u_{q}.
\end{align*}

Note that $u_p$ and $u_{q}$ are unitary in $A$, not necessarily in $C_0(X, M_n)$. Then
\begin{align*}
u_p^* u_p = u_p u_p^* = \mathrm{id}1_K
\hspace{15pt}\text{and}\hspace{15pt}
u_{q}^* u_{q} = u_{q} u_{q}^* = \mathrm{id} 1_K.
\end{align*}
Let $u = u_{q} v u_p$. Then
\begin{align*}
p = u^* q u
\hspace{15pt}\text{and}\hspace{15pt}
u^*u = uu^* = \mathrm{id} 1_K.
\end{align*}
Therefore $(iii)$ holds.

Finally, we prove $(iii) \Rightarrow (i)$. Suppose $(iii)$ holds. Fix a compact subset $K \subset X$ containing the supports of $p$ and $q$.  Let $v = qu$. Then, by assumption,
\begin{align*}
v^* v = u^* q u = p,
\end{align*}
and
\begin{align*}
v v^*
&= q u u^* q \\
&= q (\mathrm{id} 1_K) q \\
&= q q \hspace{45pt}\text{$1_K q = q$ because $q$ has support in $K$,} \\
&= q.
\end{align*}
Therefore $(i)$ is true.
\end{proof}

The following lemma implies that the trace is preserved under isomorphisms from the C*-algebra to itself.

\begin{lemma}
\label{lemma:innerautomorphism}
Let $T: M_n \rightarrow M_n$ be an isomorphism. Then there exists a unitary $u \in M_n$ such that $Ta = uau^*$ for all $a \in M_n$.
\end{lemma}

The lemma above follows from \cite[Example II.5.5.14]{Blackadar} in Blackadar's book. Such automorphism $\varphi$ with $\varphi(a) = uau^*$ is called \newterm{inner}.

The following proposition will be used later to show that the trace on $\Gamma_0(\mathcal{A})$ is well-defined.

\begin{proposition}
\label{prop:tracepreservedbyisoCXMn}
Let $X$ be a compact Hausdorff second countable totally disconnected space. Let $\varphi: C(X, M_n) \rightarrow C(X, M_n)$ be an isomorphism which is \newterm{support preserving}, i.e., such that for $a \in C(X, M_n)$,
\begin{align*}
\varphi(a)(x) = 0 \Leftrightarrow a(x) = 0
\hspace{25pt}
\text{for $x \in X$.}
\end{align*}
Then, for every projection $p \in C(X, M_n)$, we have $\mathrm{tr}(\varphi(p)) = \mathrm{tr}(p)$.
\end{proposition}
\begin{proof}
Using quotient C*-algebras, we will show that $\varphi$ induces isomorphisms $\varphi_x: M_n \rightarrow M_n$ with $\varphi_x(f(x)) = \varphi(f)(x)$, for $f \in C(X, M_n)$. Then we will apply Lemma \ref{lemma:innerautomorphism} to prove that the traces of projections are preserved under $\varphi$.

Fix $x \in X$ and let $I_x = \lbrace f \in C(X, M_n) : f(x) = 0 \rbrace$. It is straightforward that $I_x$ is an ideal of $C(X, M_n)$. The definition of the norm on $C(X, M_n)$ implies that $I_x$ is also closed. Because $I_x$ is a closed ideal, we have that $C(X, M_n)/I_x$ is a C*-algebra.

Let $q: C(X, M_n) \rightarrow C(X, M_n)/I_x$ be the quotient map. We will show that $\varphi$ induces an isormorphism $\phi: C(X, M_n)/I_x \rightarrow C(X, M_n)/I_x$. Before we do this, we need to prove that $\varphi(I_x) = I_x$.

Suppose $f \in I_x$. Then $f(x) = 0$. Since $\varphi$ is support preserving, we have $\varphi(f)(x) = 0$ and, thus, $\varphi(f) \in I_x$. This implies that $\varphi(I_x) \subset I_x$. By the same argument, $I_x \subset \varphi(I_x)$. Then $\varphi(I_x) = I_x$.

Now we can define the isomorphism $\phi: C(X, M_n)/I_x \rightarrow C(X, M_n)/I_x$ by
\begin{align*}
\phi(f + I_x) = \varphi(f) + I_x.
\end{align*}
Note that the following diagram is commutative.
\begin{equation*}
\begin{tikzcd}
C(X, M_n) \arrow{r}{\varphi}[swap]{} \arrow{d}{q}[swap]{} &
C(X, M_n) \arrow{d}{q}[swap]{} \\
C(X,M_n)/I_x \arrow{r}{\phi}[swap]{} &
C(X,M_n)/I_x
\end{tikzcd}
\end{equation*}
Next, we will define an isomorphism $\mu: C(X, M_n)/I_x \rightarrow M_n$ by
\begin{align*}
\mu(f + I_x) = f(x)
\hspace{25pt}
\text{for }f \in C(X, M_n).
\end{align*}
Then there exists an isomorphism $\varphi_x: M_n \rightarrow M_n$ such that the diagram below is commutative.
\begin{equation*}
\begin{tikzcd}
C(X, M_n) \arrow{r}{\varphi}[swap]{} \arrow{d}{q}[swap]{} &
C(X, M_n) \arrow{d}{q}[swap]{} \\
C(X,M_n)/I_x \arrow{r}{\phi}[swap]{} \arrow{d}{\mu}[swap]{}&
C(X,M_n)/I_x \arrow{d}{\mu}[swap]{}\\
M_n \arrow{r}{\varphi_x}[swap]{} & M_n
\end{tikzcd}
\end{equation*}
Then, for every $f \in C(X, M_n)$, we have
\begin{align}
\varphi_x(f(x))
&= \varphi_x(\mu(f + I_x)) \nonumber\\
&= \varphi_x \circ \mu \circ q(f) \nonumber\\
&= \mu \circ q \circ \varphi(f) \nonumber\\
&=\mu(\varphi(f) + I_x)\nonumber\\
&= \varphi(f)(x). \label{eqn:varphixf}
\end{align}
By Lemma \ref{lemma:innerautomorphism}, there exists a unitary $u_x \in M_n$ such that $\varphi_x(a) = u_x a u_x^*$ for all $a \in M_n$. Then
\begin{align*}
\tr(\varphi(f))(x) &=
\tr(\varphi(f)(x)) \\
&= \tr \varphi_x(f(x)) \hspace{20pt}\text{by \eqref{eqn:varphixf}}\\
&= \tr(u_x f(x) u_x^*) \\
&= \tr(f(x)) \\
&= \tr f(x).
\end{align*}
Since $x \in X$ is arbitrary, we have $\tr \varphi(f) = \tr f$ for $f \in C(X, M_n)$.
\end{proof}

%Let $\varphi: C(X, M_n) \rightarrow C(X, M_n)$ be an isomorphism. Then, for every projection $p \in C(X, M_n)$, $\varphi(


==> delete/K0H0-K0H0.tex <==
\subsection{The isomorphism for AF groupoids}
\label{section:K0H0:K0H0}

As we mentioned in the beginning of Section \ref{section:K0H0} (see page \pageref{section:K0H0}), we want to find an alternative proof for the isomorphism $K_0(C^*(G)) \cong H_0(G)$ given by Farsi et al \cite[Corollary 5.4]{FKPS} for AF groupoids. We want to find an alternative proof because it is not clear from their result whether this map preserves positive elements.

Note that an AF groupoid $G = \displaystyle\lim_\rightarrow G_n$ is an inductive limit of groupoids of the form $G_n \cong R(\sigma_n)$, where the maps $\sigma_n$ have the topological properties studied in the previous subsection.

The functors $K_0$ and $H_0$ are continuous with respect to inductive limits. So, if we find the isomorphisms $K_0(C^*(G_n)) \cong H_0(G_n)$, then we can apply the continuity to prove our result $K_0(C^*(G)) \cong H_0(G)$.

We begin by studying how groupoid isomorphisms induce isomorphisms of K-groups and homology groups. As a consequence, we will be able to apply the results from the previous subsection to study the isomorphisms $K_0(C^*(G_n)) \cong H_0(G_n)$. Then, we apply inductive limits to prove the isomorphism $K_0(C^*(G)) \cong H_0(G)$.

The following lemma shows that groupoid isomorphisms induce isomorphisms of the corresponding C*-algebras.

\begin{lemma}
\label{lemma:isoGHinducesCastiso}
Let $G, H$ be Hausdorff second countable ample amenable groupoids. Let $\gamma: G \rightarrow H$ be an isomorphism. Then there exists a unique isomorphism $T: C^*(G) \rightarrow C^*(H)$ such that
\begin{align*}
T(f)(h) = f \circ \gamma^{-1}(h)
\hspace{20pt}
\text{for $f \in C_c(G)$, $h \in H$.}
\end{align*}
Also, $T(C_c(G)) = C_c(H)$.
\end{lemma}
\begin{proof}
Let $T_0: C_c(G) \rightarrow C_c(H)$ be defined by
\begin{align*}
T_0(f)(h) = f \circ \gamma^{-1}(h)
\hspace{20pt}
\text{for $f \in C_c(G)$, $h \in H$.}
\end{align*}
It is straightforward that $T_0$ is a well-defined bijection. We claim that $T_0$ is a $\ast$-isomorphism. In fact, given $f_1, f_2, f \in C_c(G)$ and $g \in G$, we have
\begin{align*}
T_0(f^*)(g)
= f^* \circ \gamma^{-1}(g)
= \overline{f(\gamma^{-1}(g))^{-1})}
= \overline{f \circ \gamma^{-1}(g^{-1})}
= T(f)^*(g),
\end{align*}
and
\begin{align*}
T_0(f_1 \cdot f_2)(g)
& = (f_1 \cdot f_2)(\gamma^{-1}(g)) \\
& = \sum_{h_1 h_2 = \gamma^{-1}(g)} f_1(h_1) f_2(h_2)\\
&= \sum_{g_1 g_2 = g} f_1(\gamma^{-1}(g_1))f_2(\gamma^{-1}(g_2))
\hspace{20pt}\text{with $h_1 = \gamma^{-1}(g_1)$, $h_2 = \gamma^{-1}(g_2)$}\\
&= (f_1 \circ \gamma^{-1} \cdot f_2 \circ \gamma^{-1})(g) \\
&= T_0(f_1) \cdot T_0(f_2)(g).
\end{align*}
Then $T_0$ is a $\ast$-isomorphism. In order to extend this to an isomorphism $T: C^*(G) \rightarrow C^*(H)$, we only need to prove that $T_0$ is an isometry.

Let $x \in G$. Define $U_x: \ell^2(G_x) \rightarrow \ell^2(H_{\gamma(x)})$ by the isomorphism such that $U_x \delta_g = \delta_{\gamma(g)}$ for $g \in G_x$. Then, for $f \in C_c(G)$ and $g \in G_x$, we have
\begin{align*}
\pi_{\gamma(x)}(T_0(f)) \delta_{\gamma(g)}
&= \sum_{h \in H_{r(\gamma(g))}} T_0(f)(h) \delta_{h\gamma(g)} \\
&= \sum_{y \in G_{r(g)}} T_0(f)(\gamma(y)) \delta_{\gamma(y)\gamma(g)}
\hspace{20pt}\text{with $h = \gamma(y)$}\\
&= \sum_{y \in G_{r(g)}} f(y) \delta_{\gamma(yg)} \\
&= \sum_{y \in G_{r(x)}} f(y) U_x \delta_{yg}\\
&= U_x \pi_x(f)\delta_g.
\end{align*}
Thus $\pi_{\gamma(x)}(T_0(f)) = U_x \pi_x(f)$. Since $U_x$ is an isometry, we have $\Vert \pi_{\gamma(x)}(T_0(f)) \Vert = \Vert \pi_x(f) \Vert$. Because $G, H$ are amenable and $\gamma$ is an isomorphism, we have
\begin{align*}
\Vert T_0(f) \Vert
= \sup_{x \in G^{(0)}} \Vert \pi_{\gamma(x)}(T_0(f)) \Vert
= \sup_{x \in G^{(0)}} \Vert \pi_x(f) \Vert
= \Vert f \Vert.
\end{align*}
This implies that $T_0$ is an isometry. Therefore, we can extend $T_0$ uniquely to an isomorphism $T: C^*(G) \rightarrow C^*(H)$.
\end{proof}

\begin{remark}
\label{rmk:inducedisoK0}
It follows from Lemma \ref{lemma:isoGHinducesCastiso} that $\gamma$ induces a unique positive isomorphism $K_0(T): K_0(C^*(G)) \rightarrow K_0(C^*(H))$ such that
\begin{align*}
K_0(T)([p]_{K_0(G)}) = [(p_{ij} \circ \gamma^{-1})_{i,j}]_{K_0(H)}
\hspace{20pt}
\text{for $p \in \mathcal{P}_n(C_c(G))$.}
\end{align*}
\end{remark}

Now we prove that the isomorphism $\gamma: G \rightarrow H$ also induces an isomorphism between $H_0(G)$ and $H_0(H)$.

\begin{lemma}
\label{lemma:isoGHinducesH0iso}
Let $G, H$ be Hausdorff second countable ample amenable groupoids. Let $\gamma: G \rightarrow H$ be an isomorphism. Then there exists a positive isomorphism $S: H_0(H) \rightarrow H_0(G)$ such that
\begin{align}
\label{eqn:isoGHinducesH0iso}
S([f]_{H_0(H)}) = [f \circ \gamma]_{H_0(G)}
\hspace{20pt}
\text{for $f \in C_c(H)$.}
\end{align}
\end{lemma}
\begin{proof}
We only need to show that two functions $f_1, f_2 \in C_c(H^{(0)}, \mathbb{Z})$ are equivalent in $H_0(H)$ if, and only if, $f_1 \circ \gamma$ and $f_2 \circ \gamma$ are equivalent in $H_0(G)$.

Let $f_1, f_2 \in C_c(H^{(0)}, \mathbb{Z})$ be equivalent in $H_0(H)$. Then there exists $F \in C_c(H, \mathbb{Z})$ such that $f_1 = f_2 + \partial_1 F$. Then, for every $x \in G^{(0)}$, we have
\begin{align*}
f_1 \circ \gamma(x)
&= f_2 \circ \gamma(x) + \partial_1 F(\gamma(x)) \\
&= f_2 \circ \gamma(x) + s_\ast(F)(\gamma(x)) - r_\ast(F)(\gamma(x)) \\
&= f_2 \circ \gamma(x) + \sum_{g \in G_{\gamma(x)}} [F(g) - F(g^{-1})] \\
&= f_2 \circ \gamma(x) + \sum_{h \in G_x} [F(\gamma(h)) - F(\gamma(h^{-1}))]
\hspace{15pt}\text{with $g = \gamma(h)$}\\
&= f_2 \circ \gamma(x) + \partial_1(F \circ \gamma)(x).
\end{align*}
Then $f_1 \circ \gamma \sim f_2 \circ \gamma$.

Now suppose that $f_1 \circ \gamma \sim f_2 \circ \gamma$. Since $\gamma^{-1}$ is an isomorphism, we have by the same arguments that $f_1 \sim f_2$. Therefore $S$ is well-defined. It is straightforward from equation \eqref{eqn:isoGHinducesH0iso} that $S$ is a positive isomorphism.
\end{proof}

Suppose that $\gamma: G_n \rightarrow R(\sigma_n)$ is an isomorphism. Then, by Remark \ref{rmk:inducedisoK0} and Lemma \ref{lemma:isoGHinducesH0iso}, we have the isomorphisms $K_0(T): K_0(T): K_0(C^*(G_n)) \rightarrow K_0(R(\sigma_n)$ and $S: H_0(R(\sigma_n)) \rightarrow H_0(G_n)$. Recall from the previous section that we have the isomorphism $\nu: K_0(C^*(R(\sigma))) \rightarrow H_0(R(\sigma))$. Combining these maps, we can obtain the isomorphism $K_0(C^*(G_n)) \cong H_0(G_n)$ by
\begin{equation*}
\begin{tikzcd}
K_0(C^*(G_n)) \arrow[r, "K_0(T)"]
& K_0(C^*(R(\sigma_n))) \arrow[r, "\nu"]
& H_0(R(\sigma_n)) \arrow[r, "S"]
& H_0(G_n).
\end{tikzcd}
\end{equation*}

In order to find a formula for the isomorphism above, we will define the a trace operator on $\mathcal{P}_\infty(C^*(R(\sigma_n)))$ induced by the trace on $\mathcal{P}_\infty(C^*(R(\sigma)))$.

The following lemma studies the equivalence in $H_0(G)$ for $G \cong R(\psi)$. Later we will apply this lemma for the groupoids $G_n \cong R(\sigma_n)$.

\begin{lemma}
\label{lemma:traceH0G}
Let $G$ be a topological groupoid such that $G^{(0)}$ is locally compact Hausdorff second countable totally disconnected. Let $W$ be a locally compact Hausdorff second countable totally disconnected space. Let $\psi: G^{(0)} \rightarrow W$ be a surjective local homeomorphism. Suppose that $G$ be is isomorphic to $R(\psi)$. Then, for $f_1, f_2 \in C_c(G^{(0)}, \mathbb{Z})$, we have
\begin{align*}
f_1 \sim f_2
\Leftrightarrow
\sum_{g \in G_x} f_1(r(g)) = \sum_{g \in G_x} f_2(r(g))
\hspace{20pt}\text{for all }x \in G^{(0)}.
\end{align*}
\end{lemma}
\begin{proof}
Let $\gamma: G \rightarrow R(\psi)$ be the isomorphism of $G$ and $R(\psi)$. Then $G$ is second countable ample Hausdorff and $H_0(G)$ is well-defined. Then, for $f_1, f_2 \in C_c(G^{(0)}, \mathbb{Z})$, we have
\begin{align*}
f_1 \sim f_2 \text{ in }H_0(G)
&\ \Leftrightarrow f_1 \circ \gamma^{-1} \sim f_2 \circ \gamma^{-1} \text{ in }H_0(R(\sigma)).
%\hspace{20pt}\text{by Lemma \ref{lemma:isoGHinducesH0iso}.}
\end{align*}
Then Lemma \ref{lemma:isoGHinducesH0iso} implies that this is equivalent to
\begin{align*}
\sum_{v: \sigma(v) = \sigma(u)} f_1 \circ \gamma^{-1}(v) = 
\sum_{v: \sigma(v) = \sigma(u)} f_2 \circ \gamma^{-1}(v)
\hspace{20pt}\text{for all $u \in G^{(0)}$}.
%, by Lemma \ref{lemma:traceH0Rsigma}}
\end{align*}
Rewriting the sums above using groupoid notation, we obtain
\begin{align*}
\sum_{h \in R(\psi)_u} f_1 \circ \gamma^{-1}(r(h)) = 
\sum_{h \in R(\psi)_u} f_2 \circ \gamma^{-1}(r(h))
\hspace{20pt}\text{for all $u \in G^{(0)}$}.
\end{align*}
Using the change of variables $h = \gamma(g)$ and $u = \gamma(x)$, the equation above is equivalent to
\begin{align*}
\sum_{g \in G_x} f_1(r(g)) = \sum_{g \in G_x} f_2(r(g))
\hspace{20pt}\text{for all $x \in G^{(0)}$}. \tag*{\qedhere}
\end{align*}
\end{proof}

Now we define a trace for a groupoid $G$ isomorphic to $R(\psi)$.

\begin{lemma}
\label{lemma:traceGRpsi}
Let $G$ be a topological groupoid such that $G^{(0)}$ is locally compact Hausdorff second countable totally disconnected. Let $W$ be locally compact Hausdorff second countable totally disconnected spaces, and let $\psi: G^{(0)} \rightarrow W$ be a surjective local homeomorphism with continuous section $\varphi: W \rightarrow G^{(0)}$. Suppose that there exists an isomorphism $\gamma: G \rightarrow R(\psi)$. Let $X = G^{(0)}$. Then we can define a unique function $\tr_{\gamma, \varphi}: \mathcal{P}_\infty(C^*(G)) \rightarrow C_c(G^{(0)}, \mathbb{Z})$ such that
\begin{enumerate}[(i)]
\item For $x \in G^{(0)}$, $p \in \mathcal{P}(C_c(G))$,
\begin{align*}
\tr_{\gamma,\varphi} p(x)
= \begin{cases}
\displaystyle\sum_{g \in G_x} p(r(g)) & \text{if } x \in \gamma^{-1}(X_\varphi), \\
0 & \text{otherwise.}
\end{cases}
\end{align*}

\item $\tr_{\gamma, \varphi} p = \sum_{i=1}^n \tr_{\gamma, \varphi} p_{ii}$ for $p \in \mathcal{P}_n(C^*(G))$, $n \geq 1$.

\item For $p, q \in \mathcal{P}_\infty(C^*(G))$,
\begin{align*}
p \sim_0 q \Leftrightarrow \tr_{\gamma,\varphi} p =  \tr_{\gamma,\varphi} q.
\end{align*}

\item given $V \subset G^{(0)}$ compact open, we have that $1_V \sim \tr_{\gamma, \varphi} 1_V$ in $H_0(G)$.
\end{enumerate}
\end{lemma}
\begin{proof}
Let $T: C^*(G) \rightarrow C^*(R(\psi))$ be the isomorphism given by Lemma \ref{lemma:isoGHinducesCastiso}. Note that $\tr_\varphi$ is a map from $\mathcal{P}_\infty(C^*(R(\psi)))$ to $C_c(G^{(0)}, \mathbb{Z})$. Then we can define $\tr_{\gamma, \varphi}: \mathcal{P}_\infty(C^*(G)) \rightarrow C_c(G^{(0)}, \mathbb{Z})$ by
\begin{align*}
\tr_{\gamma,\varphi} p(x) = \tr_\varphi Tp(\gamma(x))
\hspace{20pt}
\text{for $p \in \mathcal{P}_\infty(C^*(R(\psi)))$, $x \in G^{(0)}$.}
\end{align*}
We will show that this map satisfies properties (i)-(iv).
\begin{enumerate}[(i)]
\item For $p \in \mathcal{P}(C_c(G))$ and $x \in \gamma^{-1}(X_\varphi)$, we have $Tp \in \mathcal{P}(C_c(R(\psi)))$. Then
\begin{align*}
\tr_{\gamma, \varphi} p(x)
&= \tr_\varphi Tp(\gamma(x)) \\
&= \sum_{u: \psi(u) = \psi(\gamma(x))} Tp(u,u)
\hspace{20pt}\text{since $\gamma(x) \in X_\varphi$}\\
&= \sum_{h \in R(\psi)_{\gamma(x)}} Tp(r(h))\\
&= \sum_{g \in G_x} Tp(r(\gamma(g)))
\hspace{20pt}\text{using the change of variables $h = \gamma(g)$} \\
&=\sum_{g \in G_x} p(\gamma^{-1}(r(\gamma(g))))
\hspace{20pt}\text{by definition of $T$}\\
&= \sum_{g \in G_x} p(r(g)).
\end{align*}
Given $x \in G^{(0)} \setminus \gamma^{-1}(X_\varphi)$, we have
\begin{align*}
\tr_{\gamma,\varphi} p(x)
= \tr_\varphi Tp(\gamma(x))
= 0,
\end{align*}
since $\gamma(x) \notin X_\varphi$. Then property (i) holds.

\item Let $p \in \mathcal{P}_n(C^*(G))$, $n \geq 1$ and $x \in X$. Then $Tp \in \mathcal{P}_n(C^*(R(\psi)))$ and
\begin{align*}
\tr_{\gamma,\varphi} p(x)
= \tr_\varphi Tp(\gamma(x))
= \sum_{i=1}^n \tr_\varphi(Tp)_{ii}(\gamma(x))
= \sum_{i=1}^n \tr_{\gamma,\varphi} p_{ii}(x).
\end{align*}

\item Let $p, q \in \mathcal{P}_\infty(C^*(G))$. Since $T$ is an isomorphism, we have
\begin{align*}
p \sim_0 q \text{ in $K_0(C^*(G))$ }
&\Leftrightarrow
Tp \sim_0 Tq \text{ in $K_0(C^*(R(\psi)))$} \\
&\Leftrightarrow
\tr_{\varphi} Tp = \tr_\varphi Tq \\
&\Leftrightarrow
\tr_{\varphi} Tp(\gamma(x)) = \tr_\varphi Tq(\gamma(x))
\hspace{20pt}\text{for all $x \in G^{(0)}$},
\end{align*}
because $\gamma$ is an isomorphism. Then
\begin{align*}
p \sim_0 q \text{ in $K_0(C^*(G))$ }
&\Leftrightarrow
\tr_{\gamma, \varphi} p = \tr_{\gamma, \varphi} q.
\end{align*}
\item Let $V \subset G^{(0)}$ be a compact open. Fix $p = 1_V \in C_c(G^{(0)}, \mathbb{Z})$.

Note that, for $u \in X$, $x = \gamma(\varphi(\psi(\gamma(u))))$ is the unique element in $r(G_{\gamma(u)})$ such that $\gamma^{-1}(x) \in X_\varphi$. Then
\begin{align*}
\sum_{y \in r(G_{\gamma(u)})} \tr_{\gamma, \varphi} p(y)
= \tr_{\gamma, \varphi} p(x)
= \sum_{y \in r(G_x)} p(y)
= \sum_{y \in r(G_{\gamma(u)})} p(y).
\end{align*}
By Lemma \ref{lemma:traceH0G}, we have that $p \sim \tr_{\gamma, \varphi} p$ in $H_0(G)$. Since $p = 1_V$, item (iv) holds.
\end{enumerate}
We still need to prove that $\tr_{\gamma, \varphi}$ is unique. Properties (i) and (ii) show that $\tr_{\gamma, \varphi}$ is uniquely defined on $\mathcal{P}_\infty(C_c(G))$. Let $p \in \mathcal{P}_\infty(C^*(G))$. By Lemma \ref{lemma:equivqinPnCcR}, there exists $\widetilde{q} \in \mathcal{P}_\infty(C_c(R(\psi)))$ such that $Tp \sim \widetilde{q}$ in $K_0(C^*(R(\psi)))$. Let $q = T^{-1}\widetilde{q}$. Then $p \sim q$ in $K_0(C^*(G))$. Property (iii) shows that
\begin{align*}
\tr_{\gamma, \varphi} p = \tr_{\gamma, \varphi}  q.
\end{align*}
Therefore $\tr_{\gamma, \varphi}$ is the unique function satisfying properties (i)-(iv).
\end{proof}

Note that the previous lemma defines the isomorphisms $K_0(C^*(G_n)) \cong H_0(G_n)$ using the traces on $\mathcal{P}_\infty(C^*(G_n))$. Using inductive limits, we want to show that these traces operators induce an isomorphism $K_0(C^*(G)) \cong H_0(G)$. We will do this in Theorem \ref{thm:K0H0positive} by applying Lemma \ref{lemma:homomorphisminductive} on page \pageref{lemma:homomorphisminductive}. The following lemma will be needed to apply Lemma \ref{lemma:homomorphisminductive}.

\begin{lemma}
\label{lemma:tracegamma1gamma2}
Let $X, W_1, W_2$ be locally compact Hausdorff second countable totally disconnected spaces. For $i = 1,2$, let $\psi_i: X \rightarrow W_i$ be a surjective local homeomorphism with continuous sections $\varphi_i: W_i \rightarrow X$. Let $G, H$ be topological groupoids with $G^{(0)} = H^{(0)} = X$ such that $G \subset H$ and that there are isomorphisms $\gamma_1: G \rightarrow R(\psi_1)$ and $\gamma_2: H \rightarrow R(\psi_2)$. Then, for every $p \in \mathcal{P}_\infty(C^*(G))$, we have
\begin{align*}
\tr_{\gamma_1, \varphi_1} p \sim \tr_{\gamma_2, \varphi_2} p
\text{ in }H_0(H).
\end{align*}
\end{lemma}
\begin{proof}
We will prove this lemma by applying Lemma \ref{lemma:traceH0G}. In order to apply the mentioned lemma, we will show that, for every $x \in X$,
\begin{align}
\label{eqn:sumtracegammai}
  \sum_{h \in H_x} \tr_{\scriptscriptstyle \gamma_1, \varphi_1} p(r(h))
= \sum_{h \in H_x} \tr_{\scriptscriptstyle \gamma_2, \varphi_2} p(r(h)).
\end{align}
Before we calculate the sums above, we will try to understand when those traces are non-zero. Note that, for $y \in X$, Lemma \ref{lemma:traceGRpsi} implies that, for $y \in X$,
\begin{align}
\label{eqn:yu1y}
\tr_{\scriptscriptstyle \gamma_1, \varphi_1} p(y) \neq 0
\Rightarrow y \in \gamma_1^{-1}(X_\varphi)
\Rightarrow y = \gamma_1^{-1}(\varphi_1(\psi_1(\gamma_1(y)))),
\end{align}
because $\gamma_1(y) \in X_\varphi$ if, and only if, $\gamma_1(y) = \varphi_1(\psi_1(\gamma_1(y)))$. Similarly,
\begin{align*}
%\label{eqn:yu2y}
\tr_{\scriptscriptstyle \gamma_2, \varphi_2} p(y) \neq 0
\Rightarrow
y = \gamma_2^{-1}(\varphi_2(\psi_2(\gamma_2(y)))).
\end{align*}
To simplify our notation, let $u_i: X \rightarrow \gamma_i^{-1}(X_{\varphi_i})$ be the composition $u_i = \gamma_i^{-1} \circ \varphi_i \circ \psi_i \circ \gamma_i$ for $i = 1,2$.

Note that, for $x \in X$, we have $r(G_x) = r(G_{u_1(x)})$. In fact, let $a = \gamma_1(x)$ and $b = \varphi_1(\psi_1(a))$. Then $(a,b) \in R(\psi_1)$. Let $g = \gamma_1^{-1}(a,b) \in G$. Then $g$ has range $r(g) = \gamma_1^{-1}(a) = x$ and source
\begin{align*}
s(g) = \gamma_1^{-1}(b) = \gamma_1^{-1}(\varphi_1(\psi_1(a)))
= \gamma_1^{-1}(\varphi_1(\psi_1(\gamma_1(x))))
= u_1(x).
\end{align*}
Therefore, $r(G_x) = r(G_{u_1(x)})$. By the same arguments, we have $r(H_x) = r(H_{u_2(x)})$.

Now we will start to evaluate \eqref{eqn:sumtracegammai}. Fix $x \in X$. Then
\begin{align}
\sum_{g \in G_x} \tr_{\scriptscriptstyle \gamma_1, \varphi_1} p(r(g))
&= \tr_{\scriptscriptstyle \gamma_1, \varphi_1} p(u_1(x))
\hspace{15pt}\text{by \eqref{eqn:yu1y},} \nonumber\\
&= \sum_{g \in G_{u_1(x)}} p(r(g))
\hspace{15pt}\text{by Lemma \ref{lemma:traceGRpsi},} \nonumber\\
&= \sum_{g \in G_x} p(r(g))
\hspace{30pt}\text{since $r(G_x) = r(G_{u_1(x)})$.} \label{eqn:traceGx0}
\end{align}

Since $G$ is \'etale, we can find a countable (possibly finite) family $I \subset X$ such that we have the disjoint union
\begin{align*}
r(H_x) = \bigcup_{y \in I} r(G_y).
\end{align*}
Then we have
\begin{align}
\sum_{h \in H_x} \tr_{\scriptscriptstyle\gamma_1, \varphi_1} p(r(h))
&= \sum_{y \in I} \sum_{g \in G_x} \tr_{\scriptscriptstyle\gamma_1, \varphi_1} p(r(g)) \nonumber\\
&= \sum_{y \in I} \sum_{g \in G_x} p(r(g)) \nonumber \label{eqn:traceGx}\\
&= \sum_{h \in H_x} p(r(h)).
\end{align}
By similar arguments used to find \eqref{eqn:traceGx0}, we have
\begin{align}
\sum_{h \in H_x} \tr_{\scriptscriptstyle\gamma_2, \varphi_2} p(r(h))
= \sum_{h \in H_x} p(r(h)) \label{eqn:traceHx}
\end{align}
It follows from equations \eqref{eqn:traceGx} and \eqref{eqn:traceHx} that
\begin{align*}
\sum_{h \in H_x} \tr_{\scriptscriptstyle\gamma_1, \varphi_1} p(r(h))
= \sum_{h \in H_x} \tr_{\scriptscriptstyle\gamma_2, \varphi_2} p(r(h))
\end{align*}
Since $x \in X$ is arbitrary, Lemma \ref{lemma:traceH0G} implies that $\tr_{\scriptscriptstyle\gamma_1, \varphi_1} p \sim \tr_{\scriptscriptstyle\gamma_2, \varphi_2} p$ in $H_0(H)$.
\end{proof}

Finally, we give a formula for the isomorphism $K_0(C^*(G)) \cong H_0(G)$ when $G$ is an AF groupoid.

\begin{theorem}
\label{thm:K0H0positive}
Let $X$ be a locally compact Hausdorff second countable totally disconnected space. Let $G$ be a topological groupoid such that $G = \displaystyle\lim_\rightarrow G_n$, where $G^{(0)} = X$ and, for each $n \geq 1$,
\begin{enumerate}[(i)]
\item $\psi_n: X \rightarrow W_n$ is a surjective local homeomorphism between locally compact Hausdorff second countable totally disconnected spaces.
\item $\psi_n$ has continuous section $\varphi_n: W_n \rightarrow X$.
\item There exists an isomorphism $\gamma_n: G_n \rightarrow R(\psi_n)$.
\end{enumerate}
Then there exists a positive isomorphism $\mu: K_0(C^*(G)) \rightarrow H_0(G)$ such that, for all $n \geq 1$, $p \in \mathcal{P}_\infty(C^*(G_n))$, we have
\begin{align*}
\mu([p]_0) = [ \tr_{\gamma_n, \varphi_n} p ].
\end{align*}
Moreover, we have $\mu([1_V]_0) = [1_V]$ for all $V \subset G^{(0)}$ compact open.
\end{theorem}
\begin{proof}
To avoid confusion, we will use the following notation in this proof: for each $n \geq 0$,
\begin{itemize}
\item $[\hphantom{f}]_{K,n}$ denotes the equivalence class in $K_0(C^*(G_n))$,
\item $[\hphantom{f}]_{H,n}$ denotes the equivalence class in $H_0(G_n)$,
\item $[\hphantom{f}]_{0}$ denotes the equivalence class in $K_0(C^*(G))$, and
\item $[\hphantom{f}]$ denotes the equivalence class in $H_0(G)$.
\end{itemize}

First we define the isomorphisms $\mu_n: K_0(C^*(G_n)) \rightarrow H_0(G_n)$, and then we apply Lemma \ref{lemma:homomorphisminductive} to prove that $\mu$ is a positive isomorphism.

Fix $n \geq 1$. By Lemma \ref{lemma:traceGRpsi}, we can define $\mu_n: K_0(C^*(G_n)) \rightarrow H_0(G_n)$, a positive isomorphism such that
\begin{align*}
\mu_n([p]_{K,n}) &= [\tr_{\gamma,\varphi} p]_{H,n}
\hspace{20pt}\text{for $p \in \mathcal{P}(C^*(G_n))$, and}\\
\mu_n([1_V]_{K,n}) &= [1_V]_{H,n}
\hspace{37pt}\text{for $V \subset X$ compact open.}
\end{align*}
Note that $H_0(G) = \displaystyle\lim_\rightarrow H_0(G_n)$ and $K_0(C^*(G)) = \displaystyle\lim_\rightarrow K_0(C^*(G_n))$ as inductive limits of ordered groups by Remark \ref{rmk:limK0}. For each $n \geq 0$, let $i_n: K_0(C^*(G_n)) \rightarrow K_0(C^*(G_{n+1}))$ and $j_n: H_0(G_n) \rightarrow H_0(G_{n+1})$ be the conecting morphisms, and let $\alpha_n: K_0(C^*(G_n)) \rightarrow K_0(C^*(G))$ and $\beta_n: H_0(G_n) \rightarrow H_0(G)$ be the inclusion morphisms such that
\begin{align*}
i_n([p]_{K,n}) = [p]_{K,n+1}
\hspace{15pt}\text{and}\hspace{15pt}
\alpha_n([p]_{K,n}) = [p]_0
\hspace{15pt}\text{for $p \in \mathcal{P}_\infty(C^*(G))$;}\\
j_n([f]_{H,n}) = [f]_{H,n+1}
\hspace{15pt}\text{and}\hspace{15pt}
\beta_n([f]_{H,n}) = [f]
\hspace{28pt}\text{for $f \in C_c(X, \mathbb{Z})$.}
\end{align*}

In order to apply Lemma \ref{lemma:homomorphisminductive}, we need to prove that $\mu_{n+1} \circ i_n = j_n \circ \mu_n$ for all $n \in \mathbb{N}$. In fact, given $n \geq 0$ and $p \in \mathcal{P}_n(C^*(G))$, we have
\begin{align*}
j_n \circ \mu_n([p]_{K,n})
&= j_n([\tr_{\gamma_n, \varphi_n} p]_{K,n})\\
&= [\tr_{\gamma_n, \varphi_n} p]_{K,n+1} \\
&= [\tr_{\gamma_{n+1}, \varphi_{n+1}} p]_{K,n+1}
\hspace{20pt}\text{by Lemma \ref{lemma:tracegamma1gamma2}}\\
&= \mu_{n+1}([p]_{K,n+1}) \\
&= \mu_{n+1} \circ i_n([p]_{K,n}).
\end{align*}
Then, by Lemma \ref{lemma:homomorphisminductive} on page \pageref{lemma:homomorphisminductive}, there exists a unique positive isomomorphism $\mu: K_0(C^*(G)) \rightarrow H_0(G)$ making the diagram commutative for all $n$.
\begin{equation*}
\begin{tikzcd}
K_0(C^*(G)) \arrow[r, "\mu_n"] \arrow[d, "\alpha_n"]
& H_0(G_n) \arrow[d, "\beta_n"] \\
K_0(C^*(G)) \arrow[r, "\mu"] &
H_0(G)
\end{tikzcd}
\end{equation*}
Then, for $p \in \mathcal{P}_\infty(C^*(G_n))$, $n \geq 1$, we have
\begin{align*}
\mu([p]_0) = \mu(\alpha_n([p]_{K,n})) = \beta_n(\mu_n([p]_{K,n})) = \beta_n([\tr_{\gamma_n, \varphi_n} p ]_{H,n})
= [\tr_{\gamma_n, \varphi_n} p].
\end{align*}
Moreover, for $V \subset X$ compact open,
\begin{align*}
\mu([1_V]_0) &= [\tr_{\gamma_0, \varphi_0} 1_V ] \\
&= \beta_0([\tr_{\gamma_0, \varphi_0} 1_V ]_{H,0}) \\
&= \beta_0([1_V]_{H,0})
\hspace{15pt}\text{by item (iv) of Lemma \ref{lemma:traceGRpsi}} \\
&= [1_V]. \tag*{\qedhere}
\end{align*}
\end{proof}

\newc{
\begin{remark}
It follows from Theorem \ref{thm:K0H0positive} that $K_0(B)$ is generated by the elements $[1_V]_0$, for $V \subset X$ compact open. This is true because the functions $1_V$ span $C_c(X, \mathbb{Z})$ and $\mu$ is an isomorphism.
\end{remark}
}
\newc{
\begin{remark}
\label{rmk:KOH0generatedby1V}
By the same arguments of the previous remark, $\mu: K_0(C^*(G)) \rightarrow H_0(G)$ is the unique isomorphism such that $\mu([1_V]_0) = [1_V]$ for all $V \subset X$ compact open.
\end{remark}
}


==> delete/K0H0-Ktheory-BH.tex <==
\subsubsection{Projections in $B(\mathcal{H})$}
\label{subsection:K0H0:Ktheory:BH}

Here we study some properties of projections on a Hilbert space. Using these properties, we prove Corollary \ref{corollary:polarequivproj}. This corollary is not very intuitive, but it will be used to show Proposition \ref{prop:equivalenceGamma} in Subsection \ref{subsection:K0H0:Ktheory:Gamma}, that proves that the equivalence of two projections in the dense $\ast$-algebra $\Gamma$ of $\Gamma_0(\mathcal{A})$ does not depend on the properties of the completion $\Gamma_0(\mathcal{A})$. This proposition will be used in Proposition \ref{prop:traceGamma} to show that, after we define the trace on a dense subset $\mathcal{P}(\Gamma)$, we can extend its definition uniquely to $\mathcal{P}(\Gamma_0(\mathcal{A}))$.

We use results from Murphy's book \cite[Section 2.3]{Murphy}. We also use the ideas from Corollary IV.1.3 of Davidson's book \cite{Davidson}.

We begin by studying partial isometries on a Hilbert space.

\begin{definition}
A continuous linear map $u: H_1 \rightarrow H_2$ between Hilbert spaces $H_1$, $H_2$ is a \newterm{partial isometry} if $u$ is isometric on $(\ker u)^\perp$, that is, $\Vert u(x) \Vert = \Vert x \Vert$ for all $x \in (\ker u)^\perp$.
\end{definition}

\begin{theorem}
\label{thm:partialisometry}
\cite[Theorem 2.3.3]{Murphy}
Let $H_1$, $H_2$ be Hilbert spaces and $u \in B(H_1, H_2)$. Then the following are equivalent:
\begin{enumerate}[(i)]
\item $u = uu^*u$.
\item $u^*u$ is a projection.
\item $uu^*$ is a projection.
\item $u$ is a partial isometry.
\end{enumerate}
\end{theorem}

\begin{lemma}
\label{lemma:keruu}
Let $H$ be a Hilbert space. If $u \in B(H)$ is a partial isometry, then
\begin{align*}
\ker u = \ker u^*u
\text{\hspace{15pt}and\hspace{15pt}}
\ker u^* = \ker uu^*.
\end{align*}
\end{lemma}
\begin{proof}
It is straightforward that $\ker u \subset \ker u^*u$. Let $x \in \ker u^*u$. Then, by Theorem \ref{thm:partialisometry},
\begin{align*}
ux = u(u^*ux) = u0 = 0.
\end{align*}
Then $x \in \ker u$. Therefore $\ker u = \ker u^*u$. Since $u^*$ is also a partial isometry, it follows that $\ker u^* = \ker uu^*$.
\end{proof}

The polar decomposition, stated below, associates a partial isometry for every bounded operator on a Hilbert space.

\begin{theorem}
\label{thm:polar}
\cite[Theorem 2.3.4]{Murphy}\cite[Proposition 15.3.7]{Wegge-Olsen-Ktheory} (Polar decomposition) Let $a$ be a continuous linear operator on a Hilbert space $H$. Then there is a unique partial isometry $u \in B(H)$ such that
\begin{align*}
a = u \vert a \vert,
\hspace{10pt}
\ker(u) = \ker(a)
\text{\hspace{10pt}and\hspace{10pt}}
\ker(u^*) = \ker(a^*).
\end{align*}
Moreover, $u^*a = \vert a \vert$.
\end{theorem}

The following lemma shows that projections on a Hilbert space are determined by their kernels.

\begin{lemma}
\label{lemma:samekernalProjections}
Let $H$ be a Hilbert space. Let $p, q \in B(H)$ be two projections. Then $p = q$ if, and only if, $\ker p = \ker q$.
\end{lemma}
\begin{proof}
The implication $(\Rightarrow)$ is obvious, so we will only prove the converse.

Note that
\begin{align*}
H = \ker p \oplus \mathrm{im\hphantom{.}} p = \ker q \oplus \mathrm{im\hphantom{.}} q.
\end{align*}
Since $\ker p = \ker q$, we have $\mathrm{im\hphantom{.}} p = \mathrm{im\hphantom{.}} q$.

Let $x \in \mathrm{im\hphantom{.}} p$. Then $x = px = qx$. So $p$ and $q$ coincide on $\mathrm{im\hphantom{.}} p$. If $x \in \ker p$, we have by assumption that $px = qx = 0$. Hence, $p$ and $q$ also coincide on $\ker p$. Therefore, $p = q$.
\end{proof}

The next lemma gives a condition that makes an operator $T$ and a projection $P$ have the same kernel. After this lemma, we will combine the lemma with the polar decomposition to find a partial isometry $v$ such that $P = v^*v$.

\begin{lemma}
\label{lemma:sameKernelInterval}
Let $H$ be a Hilbert space. Let $T, P \in B(H)$ be such that $P$ is a projection. Suppose that there are positive numbers $\varepsilon$ and $n$ such that
\begin{align*}
\varepsilon P \leq T^*T \leq nP.
\end{align*}
Then $\ker P = \ker T$.
\end{lemma}
\begin{proof}
Let $x \in H$. Then
\begin{align*}
\Vert Tx \Vert^2
= \langle Tx, Tx \rangle
= \langle T^*Tx, x \rangle
\leq n\langle Px, x \rangle
= n\langle Px, Px \rangle
= n\Vert Px \Vert^2,
\end{align*}
and
\begin{align*}
\varepsilon \Vert Px \Vert^2
= \varepsilon \langle Px, Px \rangle
= \varepsilon \langle P^*Px, x \rangle
= \varepsilon \langle Px, x \rangle
\leq \varepsilon \langle T^*T x, x \rangle
= \varepsilon \Vert Tx \Vert^2.
\end{align*}
Then $Tx = 0$ if, and only if, $Px = 0$.
\end{proof}

\begin{lemma}
\label{lemma:intervalprojectionpolar}
Let $H$ be a Hilbert space. Let $x \in B(H)$ have polar decomposition $x = v \vert x \vert$, and let $p \in B(H)$ be a projection. Let $\varepsilon, M$ be positive numbers.
\begin{enumerate}[(a)]
\item If $\varepsilon p \leq x^*x \leq M p$, then $p = v^*v$.
\item If $\varepsilon p \leq x x^* \leq M p$, then $p = vv^*$.
\end{enumerate}
\end{lemma}
\begin{proof}
We prove item (a). If (a) holds, Lemma \ref{lemma:sameKernelInterval} implies that $p$ and $x$ have the same kernel. By the polar decomposition and Lemma \ref{lemma:keruu},
\begin{align*}
\mathrm{ker}(p) = \mathrm{ker}(x) = \mathrm{ker}(v) = \mathrm{ker}(v^*v).
\end{align*}
Then Lemma \ref{lemma:samekernalProjections} implies that $p = v^*v$.

The item proof of item (b) is analogous.
\end{proof}

Given a projection $p \in B(H)$ and an element $x \in B(H)$ with polar decomposition $x = v \vert x \vert$. The following proposition gives a condition that makes $p = v^*v$. This result is similar to  Corollary IV.1.3 of Davidson's book \cite{Davidson}.

%\label{lemma:vvp}
\begin{proposition}
\label{prop:vvp}
Let $H$ be a Hilbert space. Let $p, q \in B(H)$ be two projections, and let $x \in B(H)$ be such that $\Vert x \Vert < 3/2$. Suppose that $x$ has the polar decomposition $x = v \vert x \vert$. Moreover, assume that $x = qxp$.
\begin{enumerate}[(a)]
\item If $\Vert x^*x - p \Vert < 1/2$, then $p = v^*v$.
\item If $\Vert xx^* - q \Vert < 1/2$, then $q = vv^*$.
\end{enumerate}
\end{proposition}
\begin{proof}
Here we prove item (a). If we show that $\frac{1}{2} p \leq x^*x \leq \frac{3}{2}p$, then Lemma \ref{lemma:intervalprojectionpolar} implies that $p = v^*v$.

Let us show that $x^*x \leq \frac{3}{2} p$. By Lemma \ref{lemma:keruu} and the polar decomposition, we have
\begin{align}
\label{eqn:kervvx}
\mathrm{ker}(v^*v) = \ker v = \ker x.
\end{align}
Since $x = qxp$ and $p, q$ are projections, then we have $x = xp$. This implies that $\ker x \supset \ker p$. Then, by \eqref{eqn:kervvx}, $\ker p \subset \ker v^*v$. Then
\begin{align*}
v^*v \leq p.
\end{align*}
By using the polar decomposion $x = v \vert x \vert$, and by multiplying both sides of the inequality above by $\vert x \vert$ to the left and to the right, we get
\begin{align*}
x^*x
= \vert x \vert v^* v \vert x \vert
\leq \vert x \vert p \vert x \vert.
\end{align*}
Note that $\vert x \vert p \vert x \vert \leq \Vert x \Vert^2$. This happens because $\vert x \vert \leq \Vert x \Vert \mathrm{id}$. Then
\begin{align*}
x^*x \leq \vert x \vert p \vert x \vert \leq \Vert x \Vert^2 p \leq \frac{3}{2} p.
\end{align*}
Now we show that $\frac{1}{2} p \leq x^*x$. Since $\Vert x^*x - p \Vert < \frac{1}{2}$, we have
\begin{align*}
p (p - x^* x)p
&\leq p \Vert x^*x - p \Vert p
\leq \frac{1}{2} p \\
\Rightarrow 
p + p(p - x^*x)p
&\leq p + \frac{1}{2}p \\
\Rightarrow
p - \frac{1}{2}p
&\leq p - p(p - x^*x)p \\
\Rightarrow
\frac{p}{2}
&\leq p - p + px^*xp \\
\Rightarrow
\frac{p}{2}
&\leq px^*xp = x^*x,
\hspace{25pt}\text{since $x = xp$.}
%\frac{p}{2} &< p - p (p - x^*x)p \\
%\Rightarrow 
%\frac{p}{2} &< p - p + px^*x p \\
%\Rightarrow 
%\frac{p}{2} &< x^* x.
\end{align*}
Then $\frac{1}{2} p \leq x^* x \leq \frac{3}{2} p$. Therefore $p = v^*v$.

We can prove item (b) by similar arguments, using the fact that $x^* = x^* q = \vert x \vert v^*$.
\end{proof}

\begin{corollary}
\label{corollary:polarequivproj}
Let $p, q \in B(H)$ be two projections. Let $x \in B(H)$ have polar decomposition $x = v \vert x \vert$, and suppose that $x = q x p$. If
\begin{align*}
\Vert x \Vert < \frac{3}{2},
\hspace{10pt}
\Vert x^* x - p \Vert < \frac{1}{2},
\hspace{10pt}\text{and}\hspace{10pt}
\Vert xx^* - q \Vert < \frac{1}{2},
\end{align*}
then $p = v^*v$ and $ q = vv^*$.
\end{corollary}

%The definition of the trace on $\mathcal{P}(\Gamma_0(\mathcal{A}))$ gives a formula for the trace of projections in the dense subset $\Gamma$. We need to guarantee that the trace is well-defined, i.e., that it has a unique extension to $\mathcal{P}(\Gamma_0(\mathcal{A}))$. We do this by proving that the trace is constant for equivalent projections in $\Gamma$, and we also study the relation between equivalence of projections in $\Gamma$ and in $\Gamma_0(\mathcal{A})$.

%One of the things we will prove in \obs{Proposition 4.38} of Subsection \obs{ref} is that two projections in $\Gamma$ are equivalent in $\Gamma_0(\mathcal{A})$ if, and only if, they are also equivalent in $\Gamma$. In other words, if two projections $p, q \in \Gamma$ are equivalent in $\Gamma_0(\mathcal{A})$, then there exists $v \in \Gamma$ such that $p = v^* v$ and $q = vv^*$.

%The proof of that proposition uses the main result of this subsection, given by Proposition \obs{ref}. Before we prove the proposition, we need to study some properties of projections and partial isometries on a Hilbert space.


==> delete/K0H0-Ktheory-Gamma.tex <==
\subsubsection{Projections in $\Gamma_0(\mathcal{A})$}
\label{subsection:K0H0:Ktheory:Gamma}

We will study the equivalence of projections in $\Gamma_0(\mathcal{A})$. We will define a trace operator $\tr_{\scriptscriptstyle{\Gamma},1}$ for projections in $\Gamma_0(\mathcal{A})$, and we will show that two projections are equivalent if, and only if, they have the same trace. The construction of the trace depends on the choice of a dense subset $\Gamma \subset \Gamma_0(\mathcal{A})$.

Although we will define the trace for $\mathcal{P}(\Gamma_0(\mathcal{A}))$, we will find its formula only for projections in $\Gamma$. In order to show that the trace is still well-defined, we need to study the equivalence of projections in $\Gamma_0(\mathcal{A})$ and in $\Gamma$. We begin by showing in Proposition \ref{prop:pinGamma} that any projection in the C*-algebra $\Gamma_0(\mathcal{A})$ is equivalent to some projection in $\Gamma$. The proof uses the ideas from \cite[Lemma III.3.1]{Davidson}.

\begin{theorem}
\label{thm:inversecontinuous}
\cite[Theorem 1.2.3]{Murphy} Let $A$ be a unital Banach algebra. If $a \in A$ is invertible and $b \in A$ is such that $\Vert b - a \Vert < \Vert a^{-1} \Vert^{-1}$, then $b$ is invertible.
\end{theorem}

%Here I only used that Gamma_k is an increasing union
\begin{proposition}
\label{prop:pinGamma}
Let $\vartheta: \mathcal{A} \rightarrow X$ be an AF bundle, and let $\Gamma \subset \Gamma_0(\mathcal{A})$ be a dense subset with a local representation. Given a projection $p \in \Gamma_0(\mathcal{A})$, there exists a projection $q \in \Gamma$ such that $p \sim q$.
\end{proposition}
\begin{proof}
First we will find a self-adjoint element $z \in \Gamma$ that approximates $p$. Then, we will study the spectrum of $z$. Finally, using the functional calculus, we will find a projection $q \in \Gamma$ such that $p \sim q$.

Let $p \in \Gamma_0(\mathcal{A})$ be a projection. Since $\Gamma$ is dense in $\Gamma_0(\mathcal{A})$, there exists $y \in \Gamma$ such that $\Vert p - y \Vert < 1/3$. Let $z = (y + y^*)/2 \in \Gamma$. Note that $p$ and $z$ are self-adjoint. Moreover,
\begin{align*}
\Vert p - z \Vert
= \left\Vert \frac{p + p^*}{2} - \frac{y + y^*}{2}\right\Vert
\leq 2 \frac{\Vert p - y \Vert}{2}
 < \frac{1}{3}.
\end{align*}

In order to study the spectrum of $z$, we will apply Theorem \ref{thm:inversecontinuous}. Note that $\sigma(p) \subset \lbrace 0,1 \rbrace$. Since $p$ is self-adjoint then, for $\lambda \notin \lbrace 0,1 \rbrace$, we have by the functional calculus that
\begin{align*}
\Vert (p - \lambda 1)^{-1} \Vert
= \max_{t \in \sigma(p)} \frac{1}{\vert \lambda -t \vert}
\leq \max \left\lbrace \frac{1}{\vert \lambda \vert}, \frac{1}{\vert 1 - \lambda \vert} \right\rbrace
= \frac{1}{\min \lbrace \vert \lambda \vert, \vert 1 - \lambda \vert \rbrace}.
\end{align*}
If $\lambda \in \mathbb{R}$ is such that $\vert \lambda \vert > \frac{1}{3}$ or $\vert \lambda - 1 \vert > \frac{1}{3}$, then
\begin{align*}
\Vert (z - \lambda 1) - (p - \lambda 1) \Vert
= \Vert p - z \Vert
< \frac{1}{3} \leq \min \lbrace \vert \lambda \vert, \vert \lambda - 1 \vert \rbrace
\leq \Vert (p-\lambda 1)^{-1} \Vert^{-1}.
\end{align*}
By Theorem \ref{thm:inversecontinuous}, we have that $z - \lambda 1$ is invertible. In other words, $\lambda \notin \sigma(z)$. Therefore
\begin{align}
\label{eqn:sigmazintervals}
\sigma(z) \subset \left[-\frac{1}{3}, \frac{1}{3} \right] \cup \left[\frac{2}{3}, \frac{4}{3} \right].
\end{align}

Using the continuous functional calculus for normal operators, we obtain a projection $q = \chi_{\left\lbrace \frac{2}{3}, \frac{4}{3} \right\rbrace}(z) \in \Gamma$. Moreover,
\begin{align*}
\Vert p - q \Vert
&\leq \Vert p - z \Vert
+ \Vert z - \chi_{\left\lbrace \frac{2}{3}, \frac{4}{3} \right\rbrace}(z) \Vert\\
&= \Vert p - z \Vert
+ \max_{t \in \sigma(z)} \vert t - \chi_{\left\lbrace \frac{2}{3}, \frac{4}{3} \right\rbrace}(t) \vert\\
&\leq \Vert p - z \Vert
+ \max_{t \in [-\frac{1}{3}, \frac{1}{3}] \cup [\frac{2}{3}, \frac{4}{3} ]} \vert t - \chi_{\left\lbrace \frac{2}{3}, \frac{4}{3} \right\rbrace}(t) \vert
\text{\hspace{30pt}by \eqref{eqn:sigmazintervals}}\\
&=  \Vert p - z \Vert + \frac{1}{3} \\
&< \frac{1}{3} + \frac{1}{3}\\
&= \frac{2}{3}.
\end{align*}
Therefore, $p \sim q$ by Proposition \ref{prop:closeprojections}.
\end{proof}

Now we study the equivalence of projections in $\Gamma$. The following proposition says that if two of them are equivalent in $\Gamma_0(\mathcal{A})$, then they are equivalent in $\Gamma$. Later, when we define the trace on $\mathcal{P}(\Gamma_0(\mathcal{A}))$, this property will be used to show that two projections are equivalent if, and only if, they have the same trace.

\begin{proposition}
\label{prop:equivalenceGamma}
Let $\vartheta: \mathcal{A} \rightarrow X$ be an AF bundle, and let $\Gamma \subset \Gamma_0(\mathcal{A})$ be a dense subset with a local representation $(\Gamma_k, V_{k,l}, \alpha_{k,l}, n_{k,l})_{(k,l) \in I}$. Given two projections $p, q \in \Gamma$ such that $p \sim q$ in $\Gamma_0(\mathcal{A})$, then there exists $v \in \Gamma$ such that $p = v^*v$ and $q = vv^*$.
\end{proposition}
\begin{proof}
Recall that the projections in $\Gamma$ can be seen locally as elements of $C(V, M_n) \cong B(C(V, \mathbb{C}^n))$. With this idea in mind, we want to apply Corollary \ref{corollary:polarequivproj} to find $v$. So, we want to find an $f \in \Gamma$ that satisfies analogous conditions of the corollary, i.e., $f = qfp$,
\begin{align*}
\Vert f \Vert < \frac{3}{2},
\hspace{15pt}
\Vert f^*f - p \Vert < \frac{1}{2},
\hspace{15pt}\text{and }
\Vert ff^* - q \Vert < \frac{1}{2}.
\end{align*}

Let $p, q \in \Gamma$ be two projections which are equivalent in $\Gamma_0(\mathcal{A})$. Then there exists $s \in \Gamma_0(\mathcal{A})$ satisfying $p = s^*s$ and $q = ss^*$. Let $u = qsp$. Then $u = qup$. Moreover, by expanding the formulas of the projections $p$ and $q$, we have
\begin{align*}
u^*u = p
\hspace{15pt}\text{and}\hspace{15pt}
uu^* = q.
\end{align*}
Since $u$ is a partial isometry, we have $\Vert u \Vert \geq 1$.

Note that the operations in $\Gamma_0(\mathcal{A})$ are continuous. Then there exists $0 < \delta < 1/2$ such that, for $a \in \Gamma_0(\mathcal{A})$ with $\Vert a - u \Vert < \delta$, we have
\begin{align}
\label{eqn:aaminusuu}
\Vert a^*a - p \Vert < \frac{1}{2}
\hspace{15pt}\text{and}\hspace{15pt}
\Vert aa^* - q \Vert < \frac{1}{2}.
\end{align}

Since $\Gamma$ is dense in $\Gamma_0(\mathcal{A})$, there exists $h \in \Gamma$ such that $\Vert h - u \Vert < \delta$. By definition of $\Gamma$, there is a $k$ such that $h, p, q$ are in the C*-algebra $\Gamma_k$. Let $f = q h p \in \Gamma_k$. Then $f = q f p$ and
\begin{align*}
\Vert f - u \Vert
= \Vert q h p - q u p \Vert
\leq \Vert q \Vert \Vert h - u \Vert \Vert p \Vert < \delta.
\end{align*}
Then equation \eqref{eqn:aaminusuu} holds if we replace $a$ by $f$.

By Definition \ref{def:AFbundle}, there are disjoint compact open subsets $V_{k,1}, V_{k,2}, \hdots, V_{k,m_k} \subset X$ such that, for every $l$, there exists $n_{k,l} \geq 1$ and an isomorphism
\begin{align}
\label{eqn:Gammakl}
\Gamma_{k,l} = \Gamma_{k}\vert_{V_{k,l}} \cong C(V_{k,l}, M_{n_{k,l}}) \cong B(C(V_{k,l}, \mathbb{C}^{n_{k,l}})).
\end{align}

Using the isomorphism \eqref{eqn:Gammakl}, we can apply the results of the polar decomposition directly on the elements of $\Gamma_{k,l}$. Set $f_{l} = f_{V_{k,l}}$. Then there exists a partial isometry $v_l \in \Gamma_{k,l}$ such that $f_{l}$ has the polar decomposition below.
\begin{align*}
f_{l} = v_l \vert f_{l} \vert.
\end{align*}
Let $u_l = u\vert_{V_{k,l}}$, $p_l = p\vert_{V_{k,l}}$ and $q_l = q\vert_{V_{k,l}}$. Since equation \eqref{eqn:aaminusuu} holds for $f$, the definitions of $f_l$ and $u_l$ imply that
\begin{align}
\label{eqn:flul}
\Vert f_l - u_l \Vert < \delta < \frac{1}{2},
\hspace{15pt}
\Vert f_l^* f_l - p_l \Vert < \frac{1}{2}
\hspace{15pt}\text{and}\hspace{15pt}
\Vert f_l f_l^* - q_l \Vert < \frac{1}{2}.
\end{align}
Also,
\begin{align}
\label{eqn:flbound}
\Vert f_l \Vert
\leq \Vert f_l - u_l \Vert + \Vert u_l \Vert
< \frac{1}{2} + 1
= \frac{3}{2}.
\end{align}
By equations \eqref{eqn:flul} and \eqref{eqn:flbound}, we can apply Corollary \ref{corollary:polarequivproj}. Then $v_l^* v_l = p_l$ and $v_l v_l^* = q_l$. Since the operations in $\Gamma_k$ are pointwise, if we define $v = \sum_{l=1}^{m_k} v_l \in \Gamma_k$, then $p = v^*v$ and $q = vv^*$.
\end{proof}

%When we define the trace $\tr_{\scriptscriptstyle\Gamma, 1}$ on $\Gamma$, its definition will depend locally on the isomorphism $\Gamma_{k,l} \cong C(V_{k,l}, M_{n_{k,l}})$ and on the natural trace of $C(V_{k,l}, M_{n_{k,l}})$, defined in Subsection \ref{subsection:KtheoryAF:C0XMn}. We need to guarantee that the trace does not depend on the choice of $k$. The lemma below will be used later to prove this property.

%We will use the results below to show that the trace of $p$ does not depend on the choice of $k$.

Let $\mathcal{A}$ be an AF bundle, and $\Gamma$ be a dense subset of $\Gamma_0(\mathcal{A})$ with a local representation. We know that $\Gamma$ is an increasing union of C*-algebras $\Gamma_k$ that are locally isomorphic to C*-algebras of the form $C(V, M_n)$. Using these isomorphisms, we can define a trace operator on $\mathcal{P}(\Gamma_k)$ for each $k$. We hope that these traces are compatible, i.e., that they do not depend on the choice of $k$, so that we can extend the definition of the trace to $\mathcal{P}(\Gamma_0(\mathcal{A}))$. The next lemma will be helpful to show that this is true.

\begin{lemma}
\label{lemma:diagramCXMninclusion}
Let $\vartheta: \mathcal{A} \rightarrow X$ be an AF bundle. Let $V \subset X$ be a compact open subset. Let $A \subset B$ be two subsets of $\Gamma_0(\mathcal{A})$ such that $A \cong C(V, M_m)$. Assume also that there is a support preserving isomorphism $\beta_0: B \rightarrow C(V, M_n)$. Let $i: A \hookrightarrow B$ be the inclusion map, and let $j: C(V, M_m) \rightarrow C(V, M_n)$ be given by
\begin{align}
\label{eqn:jCXMm}
j(f)(x) = \begin{bmatrix} f(x) & 0 \\ 0 & 0 \end{bmatrix}
\hspace{20pt}
\text{for }
f \in C(V, M_m), x \in X.
\end{align}
Then there are support preserving isomorphisms $\alpha: A \rightarrow C(V, M_m)$ and $\beta: B \rightarrow C(V, M_n)$ such that the diagram below is commutative.
$$
\begin{tikzcd}
A \arrow{r}{i}[swap]{} \arrow{d}{\alpha}[swap]{} &
B \arrow{d}{\beta}[swap]{} \\
C(V,M_m) \arrow{r}{j}[swap]{} &
C(V, M_n)
\end{tikzcd}
$$
\end{lemma}
\begin{proof}
Let $\beta_0: B \rightarrow C(V, M_n)$ be a support preserving isomorphism. We claim that $\tr \beta_0 (1_A) \equiv m$.

Let $\mu \in C(V, \mathbb{N})$ be given by $\mu(x) = \tr \beta_0(1_A)(x)$. By Proposition \ref{prop:traceCXMn}, there exists a unitary $u \in C(V, M_n)$ such that
\begin{align}
\label{eqn:ubeta1au}
[u^* \beta_0(1_A) u](x) = \begin{bmatrix}
\mathrm{id}_{\mu(x)} & 0 \\ 0 & 0
\end{bmatrix}
\hspace{20pt}\text{for $x \in V$.}
\end{align}
Let $V_1, V_2, \hdots, V_k$ be a partition of $V$ such that, for $i = 1, \hdots, k$, $\mu$ is constant on $V_i$ assuming value $\mu_i$. Then \eqref{eqn:ubeta1au} implies that
\begin{align}
\label{eqn:ubetaAusub}
u^* \beta_0(A) u \subset \bigoplus_{i=1}^k C(V_i, M_{\mu_i} \oplus 0_{n-\mu_i}).
\end{align}
Since
\begin{align}
\label{eqn:ubetaAcong}
u^* \beta_0(A) u \cong \beta_0(A) \cong A \cong C(V, M_m),
\end{align}
we have $m = \mu_1 = \hdots = \mu_k$. Then $\tr \beta_0(1_A) \equiv m$. Moreover, \eqref{eqn:ubetaAusub} and \eqref{eqn:ubetaAcong} imply that
\begin{align*}
u^*\beta_0(A) u = C(V, M_m \oplus 0_{n-m}).
\end{align*}

Let $\beta: B \rightarrow C(V, M_n)$ be the isomorphism given by $\beta(f) = u^* \beta_0(f) u$. Then $\beta$ is support preserving and $\beta(A) = C(V, M_m \oplus 0_{n-m})$. So we have the commutative diagram below.

\begin{equation*}
\begin{tikzcd}
A \arrow[hookrightarrow]{r}{i} \arrow{d}{\beta\vert_A}&
B \arrow{d}{\beta} \\
C(V, M_m \oplus 0_{n-m}) \arrow[hookrightarrow]{r}{} &
C(V, M_n)
\end{tikzcd}
\end{equation*}
Let $q: C(V, M_m \oplus 0_{n-m}) \rightarrow C(V, M_m)$ be the isomorphism given by $q(f)(x) = (f(x)_{ij})_{1 \leq i,j \leq m}$. Let $\alpha = q \circ \beta\vert_A$. Then $\alpha$ is support preserving and the following diagram is commutative.
\begin{equation*}
\begin{tikzcd} %[to path={..controls + (1.5,0.5) and +(-1,0.8).. (\tikztotarget)}]
A \arrow{r}{i} \arrow{d}{\beta\vert_A} \ar[dd,"\alpha",bend right=80,looseness=2,swap]
& B \arrow{d}{\beta}\\
C(V, M_m \oplus 0_{n-m}) \arrow[hookrightarrow]{r}{} \arrow{d}{q} 
& C(V, M_n) \\
C(V, M_m) \arrow{ur}{j}
\end{tikzcd}
\end{equation*}
Therefore the result holds.
\end{proof}

Now we define the trace $\tr_{\scriptscriptstyle \Gamma, 1}$ on $\Gamma_0(\mathcal{A})$.

\begin{proposition}
\label{prop:traceGamma}
Let $\vartheta: \mathcal{A} \rightarrow X$ be an AF bundle. Let $\Gamma \subset \Gamma_0(\mathcal{A})$ be a dense subset that has a local representation.Then we can define uniquely an operator $\tr_{\scriptscriptstyle\Gamma,1}: \mathcal{P}(\Gamma_0(\mathcal{A})) \rightarrow C(X, \mathbb{N})$ by
\begin{align}
\label{eqn:traceGamma}
\tr_{\scriptscriptstyle\Gamma,1} p(x) = \tr(\alpha_{k,l}(p\vert_{V_{k,l}})(x))
\hspace{25pt}\text{for $x \in V_{k,l}$, $p \in \mathcal{P}(\Gamma_k)$, $(k,l) \in I$,}
\end{align}
where $(\Gamma_k, V_{k,l}, \alpha_{k,l}, n_{k,l})_{(k,l) \in I}$ is a local representation of $\Gamma$. Given $p \in \mathcal{P}(\Gamma_0(\mathcal{A}))$, we say that $\tr_{\scriptscriptstyle\Gamma,1} p$ is the \newterm{trace} of $p$. Moreover, for $p,q \in \mathcal{P}(\Gamma_0(\mathcal{A}))$, we have that $p \sim q$ if, and only if, $\tr_{\scriptscriptstyle\Gamma,1} p = \tr_{\scriptscriptstyle\Gamma,1} q$.
\end{proposition}
\begin{proof}
First we show that the trace is well-defined on $\mathcal{P}(\Gamma)$. Then we extend the definition to $\mathcal{P}(\Gamma_0(\mathcal{A}))$.

Note that, to calculate \eqref{eqn:traceGamma}, we need to choose:
\begin{enumerate}[(i)]
%\item a dense subset $\Gamma$ satisfying the conditions of Definition \ref{def:AFbundle},
\item the family $\lbrace \Gamma_k \rbrace_{ k\geq 1}$ with $\Gamma = \cup_{k=1}^\infty \Gamma_k$,
\item the compact open sets  $V_{k,l}$ for $(k,l) \in I$,
\item the isomorphisms $\alpha_{k,l}: \Gamma_{k,l} \rightarrow C(V_{k,l}, M_{n_{k,l}})$,
\item $k$ such that $p \in \Gamma_k$.
\end{enumerate}
We need to show that \eqref{eqn:traceGamma} does not depend on any of those things. We also need to prove that $\tr_{\scriptscriptstyle\Gamma,1} p \in C_c(X, \mathbb{N})$ for all $p \in \mathcal{P}(\Gamma_0(\mathcal{A}))$. Since the case $p = 0$ is obvious, we suppose here that $p \neq 0$.

\begin{enumerate}[(a)]
\item It does not depend on $k$

Suppose that (i)-(iii) are fixed. Given a non-zero $p \in \mathcal{P}(\Gamma)$, we can choose $k \geq 1$ such that $p \in \Gamma_k$. Since $\Gamma_k \subset \Gamma_{k+1}$, we have $p \in \Gamma_{k+1}$.

Let $x \in X$ be such that $p(x) \neq 0$. Then there are $l_0, l_1$ such that $x \in V_{k,l_0}\cap V_{k+1, l_1}$. Also, there are support preserving isomorphisms $\alpha_{k,l_0}:\Gamma_{k,l_0} \rightarrow C(V_{k,l_0}, M_{n_{k,l_0}})$ and $\alpha_{k+1,l_1}:\Gamma_{k+1,l_1} \rightarrow C(V_{k+1,l_1}, M_{n_{k+1,l_1}})$. To simplify our notation, we let $m = n_{k,l_0}$ and $n = n_{k+1,l_1}$.

Let $V = V_{k,l_0} \cap V_{k+1, l_1}$. Since $\alpha_{k,l_0}$ and $\alpha_{k+1, l_1}$ are support preserving, if we let $\alpha_0$ be the restriction of $\alpha_{k,l_0}$ to $\Gamma_{k,l_0}\vert_V$ and $\beta_0$ be the restriction of $\alpha_{k+1, l_1}$ to $\Gamma_{k+1, l_1}\vert_V$, then
\begin{align*}
\alpha_0: \Gamma_{k,l_0}\vert_V \rightarrow C(V, M_m)
\hspace{15pt}\text{and}\hspace{15pt}
\beta_0: \Gamma_{k+1,l_1}\vert_V \rightarrow C(V, M_{n})
\end{align*}
are support preserving isomorphisms. By Lemma \ref{lemma:diagramCXMninclusion}, we can find support preserving isomorphisms $\alpha: \Gamma_{k,l_0}\vert_V \rightarrow C(V, M_m)$ and $\beta: \Gamma_{k+1,l_1}\vert_V \rightarrow C(V, M_n)$ such that the diagram below is commutative, where $i$ and $j$ are as in that lemma.
$$
\begin{tikzcd}
\Gamma_{k,l_0}\vert_V \arrow{r}{i}[swap]{} \arrow{d}{\alpha}[swap]{} &
\Gamma_{k+1,l_1}\vert_V \arrow{d}{\beta}[swap]{} \\
C(V,M_m) \arrow{r}{j}[swap]{} &
C(V, M_n)
\end{tikzcd}
$$
Then
\begin{align*}
\tr \alpha_{k,l_0}(p)(x)
&= \tr \alpha_0(p)(x) \text{\hspace{40pt}by definition of $\alpha_0$}\\
&= \tr \alpha(p)(x) \text{\hspace{45pt}by Proposition \ref{prop:tracepreservedbyisoCXMn}}\\
&= \tr j (\alpha(p))(x) \text{\hspace{32pt}by definition of $j$}\\
&= \tr \beta(p)(x) \text{\hspace{47pt}since the diagram above commutes}\\
&= \tr \beta_0(p)(x) \text{\hspace{43pt}by Proposition \ref{prop:tracepreservedbyisoCXMn}}\\
&= \tr \alpha_{k+1, l_1}(p)(x).
\end{align*}
Note that, in the equation above, $\tr \alpha_0(p)(x) = \tr \alpha(p)(x)$ because $\alpha \circ \alpha_0^{-1}: C(V, M_m) \rightarrow C(V, M_m)$ is a support preserving isomorphism. This allows us to apply Proposition \ref{prop:tracepreservedbyisoCXMn} to get the equality. The same argument holds for $\tr \beta(p)(x) = \tr \beta_0(p)(x)$.
\item $\tr_{\scriptscriptstyle\Gamma,1}$ does not depend on $\alpha_{k,l}$

Suppose that (i) and (ii) are fixed. Let Let $k \geq 1$ and $p \in \mathcal{P}(\Gamma_k)$. Choose $x \in X$ such that $p(x) \neq 0$. Then there exists $l$ such that $x \in V_{k,l}$ and there is a support preserving isomorphism $\alpha_{k,l}: \Gamma_{k,l} \rightarrow C(V_{k,l}, M_{n_{k,l}})$. Suppose that $\alpha: \Gamma_{k,l} \rightarrow  C(V, M_{n_{k,l}})$ is another support preserving isomorphism. Then Proposition \ref{prop:tracepreservedbyisoCXMn} implies that
\begin{align*}
\tr\alpha_{k,l}(p)(x) = \tr\alpha(p)(x).
\end{align*}

\item the trace $\tr_{\scriptscriptstyle\Gamma,1}$ does not depend on the sets $V_{k,l}$

Suppose that (i) is fixed. Suppose that, for each $k$, there are two partitions $\lbrace V_{k,l} \rbrace_{l \geq 1}$ and $\lbrace W_{k,l} \rbrace_{l \geq 1}$ of the support of $\Gamma_k$, and isomorphisms $\alpha_{k,l}: \Gamma_k\vert_{V_{k,l}} \rightarrow C(V_{k,l}, M_{m_{k,l}})$ and $\beta_{k,l}: \Gamma_k\vert_{W_{k,l}} \rightarrow C(W_{k,l}, M_{n_{k,l}})$ for $k,l \geq 1$.

Given $p \in \mathcal{P}(\Gamma)$, there exists $k \geq 1$ such that $f \in \Gamma_k$. Let $x \in X$. Then there are $l_0, l_1$ such that $x \in V_{l_0} \cap W_{l_1}$. Let $V = V_{l_0} \cap W_{l_1}$. Note that
\begin{align*}
\Gamma_k\vert_V
= (\Gamma_k\vert_{V_{k,l_0}})_V
= (\Gamma_k\vert_{W_{k,l_1}})_V.
\end{align*}

Let $\alpha$ be the restriction of $\alpha_{k,l_0}$ to $\Gamma_{k}\vert_V$, and let $\beta$ be the restriction of $\beta_{k,l_1}$ to $\Gamma_{k}\vert_V$. Then
\begin{align*}
\alpha: \Gamma_{k}\vert_V \rightarrow C(V, M_{n_0})
\hspace{15pt}\text{and}\hspace{15pt}
\beta: \Gamma_{k}\vert_V \rightarrow C(V, M_{n_1})
\end{align*}
are support preserving isomorphisms for some $n_0, n_1$. This implies that $n \coloneqq n_0 = n_1$. Since $\alpha$ and $\beta$ are support preserving, Proposition \ref{prop:tracepreservedbyisoCXMn} implies that
\begin{align*}
\tr(\alpha_{k,l}(p)(x))
= \tr(\alpha(p)(x))
= \tr(\beta(p)(x))
= \tr(\beta_{k,l}(p)(x)).
\end{align*}

\item the trace $\tr_{\scriptscriptstyle\Gamma,1}$ does not depend on the increasing family $\lbrace \Gamma_k \rbrace_{k \geq 1}$ with $\Gamma = \cup_{k=1}^\infty \Gamma_k$

The proof of this item uses almost the same arguments from item (a). Suppose $\lbrace\Gamma_{k}\rbrace_{k \geq 1}$ and $\lbrace\widetilde{\Gamma}_{k}\rbrace_{k \geq 1}$ are two families of increasing subsets satisfying the conditions of Definition \ref{def:AFbundle}. That is, we have
\begin{align}
\label{eqn:unionGammak}
\Gamma
= \bigcup_{k = 1}^\infty \Gamma_k
= \bigcup_{k = 1}^\infty \widetilde{\Gamma}_k.
\end{align}
Moreover, for every $k$, the support of $\Gamma_k$, $\widetilde{\Gamma}_k$ has partitions $\lbrace V_{k,l} \rbrace_{l \geq 1}$ and $\lbrace \widetilde{V}_{k,l} \rbrace_{l \geq 1}$, respectively, such that, for every $k, l$, we have the support preserving isomorphisms
\begin{align*}
\alpha_{k,l}: \Gamma_{k,l}\vert_{V_{k,l}} \rightarrow C(V,M_{m_{k,l}})
\hspace{15pt}\text{and}\hspace{15pt}
\beta_{k,l}: \widetilde{\Gamma}_{k,l}\vert_{\widetilde{V}_{k,l}} \rightarrow C(\widetilde{V},M_{n_{k,l}}),
\end{align*}
where $\Gamma_{k,l} = \Gamma_{k}\vert_{V_{k,l}}$ and $\widetilde{\Gamma}_{k,l} = \widetilde{\Gamma}_{k}\vert_{\widetilde{V}_{k,l}}$.

Let $p \in \mathcal{P}(\Gamma)$ be a non-zero projection. Since \eqref{eqn:unionGammak} are increasing unions, we can choose $k_1, k_2$ such that $p \in \Gamma_{k_1} \subset \widetilde{\Gamma}_{k_2}$. Now fix $x \in X$ with $p(x) \neq 0$. Then there are $l_1, l_2$ such that $x \in V_{k_1, l_1} \cap \widetilde{V}_{k_2, l_2}$, and we have the support preserving isomorphisms
\begin{align*}
\alpha_{k_1, l_1}: \Gamma_{k_1}\vert_{V_{k_1,l_1}} \rightarrow C(V_{k_1,l_1}, M_{m_{k_1, l_1}})
\hspace{7pt}\text{and}\hspace{7pt}
\beta_{k_2, l_2}: \widetilde{\Gamma}_{k_2}\vert_{V_{k_2,l_2}} \rightarrow C(V_{k_2,l_2}, M_{n_{k_2, l_2}}).
\end{align*}

Let $V = V_{k_1, l_1} \cap \widetilde{V}_{k_2, l_2}$. Let $\alpha_0$ be the restriction of $\alpha_{k_1, l_1}$ to $\Gamma_{k_1}\vert_V$, and let $\beta_0$ be the restriction of $\beta_{k_2, l_2}$ to $\Gamma_{k_2}\vert_V$. Since $\alpha_{k_1, l_1}$ and $\beta_{k_2, l_2}$ are support preserving, we have the following support preserving isomorphisms
\begin{align*}
\alpha_0: \Gamma_{k_1}\vert_{V} \rightarrow C(V, M_m)
\hspace{15pt}\text{and}\hspace{15pt}
\beta_0: \widetilde{\Gamma}_{k_2}\vert_{V} \rightarrow C(V, M_n),
\end{align*}
where $m = m_{k_1, l_1}$ and $m = n_{k_2, l_2}$. Since $\Gamma_{k_1} \subset \widetilde{\Gamma}_{k_2}$, we must have $m \leq n$.

By Lemma \ref{lemma:diagramCXMninclusion}, there are support preserving isomorphisms
\begin{align*}
\alpha: \Gamma_{k_1}\vert_V \rightarrow C(V, M_m)
\hspace{15pt}\text{and}\hspace{15pt}
\beta: \widetilde{\Gamma}_{k_2}\vert_V \rightarrow C(V, M_n)
\end{align*}
making the diagram below commutative, where $i$ and $j$ are as in the lemma.

$$
\begin{tikzcd}
\Gamma_{k_1}\vert_V \arrow{r}{i}[swap]{} \arrow{d}{\alpha}[swap]{} &
\widetilde{\Gamma}_{k_2}\vert_V \arrow{d}{\beta}[swap]{} \\
C(X,M_m) \arrow{r}{j}[swap]{} &
C(X, M_n)
\end{tikzcd}
$$

Then
\begin{align*}
\tr(\alpha_{k_1,_l1}(f\vert_{V_{k_1,l_1}})(x))
&=\tr(\alpha_0(f\vert_V)(x))\\
&=\tr(\alpha(f\vert_V)(x)) \hspace{20pt}\text{by item (b)}\\
&= \tr(j \circ \alpha(f)(x))\\
&= \tr(\beta \circ i(f)(x)) \hspace{17pt}\text{by the diagram above}\\
&= \tr(\beta(f)(x))\\
&= \tr(\beta_0(f)(x)) \hspace{27pt}\text{by item (b)}\\
&= \tr(\beta_{k_2, l_2}(f)(x)).
\end{align*}

Thus, the trace $\tr_{\scriptscriptstyle\Gamma,1}$ does not depend on the choice of the family $\lbrace \Gamma_k \rbrace_{k \geq 1}$.

\item $\tr_{\scriptscriptstyle\Gamma,1} p \in C_c(X, \mathbb{N})$ for all $p \in \mathcal{P}(\Gamma)$

Let $p \in \mathcal{P}(\Gamma)$. There exists $k \geq 1$ such that $p \in \Gamma_k$. Let $V_{k,1}, V_{k,2}, \hdots, V_{k,m_k}$ be a partition of the support of $\Gamma_k$ such that, for each $l$, there exists a support preserving isomorphism $\alpha_{k,l}: \Gamma_{k,l} \rightarrow C_c(V_{k,l}, M_{n_{k,l}})$. Note that, for each $l$, we have $p \vert_{V_{k,l}} \in \Gamma_{k,l}$. Then, by definition of $\alpha_{k,l}$ and by Lemma \ref{lemma:tracewelldefined},
\begin{align*}
\tr \alpha_{k,l}(p \vert_{V_{k,l}}) \in C(V_{k,l}, \mathbb{N}).
\end{align*}
Since $p \in \Gamma_k$ and $\Gamma_k$ has support $V_{k,1} \cup \cdots \cup V_{k,m_k}$, we can write
\begin{align*}
\tr_{\scriptscriptstyle\Gamma,1} p = \sum_{l=1}^{m_k} \tr \alpha_{k,l}(p \vert_{V_{k,l}}) 1_{V_{k,l}},
\end{align*}
which implies that $\tr p \in C_c(X, \mathbb{N})$.

\item for $\Gamma$ fixed, we can extend the trace uniquely to $\mathcal{P}(\Gamma_0(\mathcal{A}))$. Also the trace distinguish projections up to equivalence

First we show that, for $q_1, q_2 \in \mathcal{P}(\Gamma)$ with $q_1 \sim q_2$, we have $	\tr_{\scriptscriptstyle\Gamma,1} q_1 = \tr_{\scriptscriptstyle\Gamma,1} q_2$. In fact, given two equivalent projections $q_1, q_2 \in \Gamma$, Proposition \ref{prop:equivalenceGamma} implies that there is a $u \in \Gamma$ such that $q_1 = u^*u$ and $q_2 = uu^*$. Let $k \geq 1$ be such that $p,q,u \in \Gamma_k$. Given $x \in X$, there exists $l \geq 1$ such that $x \in V_{k,l}$. Then
\begin{align*}
\tr q_1(x)
&= \tr(\alpha_{k,l}(q_1 \vert_{V_{k,l}})(x))\\
&= \tr(\alpha_{k,l}(u\vert_{V_{k,l}}^*u \vert_{V_{k,l}})(x))\\
&= \tr(\alpha_{k,l}(u\vert_{V_{k,l}})^*\alpha_{k,l}(u\vert_{V_{k,l}}))(x))\\
&= \tr(\alpha_{k,l}(u\vert_{V_{k,l}})\alpha_{k,l}(u\vert_{V_{k,l}})^*)(x))\\
&= \tr(\alpha_{k,l}(uu^*) \vert_{V_{k,l}})(x))\\
&= \tr(\alpha_{k,l}(q_2) \vert_{V_{k,l}})(x))\\
&=\tr q_2(x).
\end{align*}
Then $\tr q_1 = \tr q_2$.

Now we extend the definition of trace to $\mathcal{P}(\Gamma_0(\mathcal{A}))$. Let $p \in \Gamma_0(\mathcal{A})$. Then, by Proposition \ref{prop:pinGamma} implies that there exists $q \in \mathcal{P}(\Gamma)$ such that $p \sim q$. Then we can define $\tr_{\scriptscriptstyle\Gamma,1} p = \tr_{\scriptscriptstyle\Gamma,1} q$ because, as we have proved, this does not depend on the choice of $q \in \mathcal{P}(\Gamma)$ with $p \sim q$. Therefore $\tr_{\scriptscriptstyle\Gamma,1}$ is well-defined. Moreover, two projections in $\Gamma_0(\mathcal{A})$ are equivalent if, and only if, they have the same trace. \qedhere

%\item the trace does not depend on the choice of $\Gamma$.
\end{enumerate}
\end{proof}


==> delete/K0H0-Ktheory-main.tex <==
\subsubsection{K-theory of $\Gamma_0(\mathcal{A})$}
\label{subsection:K0H0:Ktheory:main}

Now we study the K-theory of $\Gamma_0(\mathcal{A})$. In the previous subsection we investigated the equivalence of projections in $\Gamma_0(\mathcal{A})$.

Note that the K-theory of this C*-algebra depends on the equivalence of projections in $M_n(\Gamma_0(\mathcal{A}))$, for $n$ arbitrary. We will show that $M_n(\Gamma_0(\mathcal{A})) \cong \Gamma_0(\mathcal{A}^{(n)})$, where $\mathcal{A}^{(n)}$ is an AF bundle. This isomorphism will allow us to use the results of the previous subsection to understand the K-theory of $\Gamma_0(\mathcal{A})$.

We begin by defining the set $\mathcal{A}^{(n)}$.

\begin{definition}
\label{def:AFndefinitions}
Let $\vartheta: \mathcal{A} \rightarrow X$ be an AF bundle. Given $n \geq 1$, we define
\begin{enumerate}[(a)]
\item the set $\mathcal{A}^{(n)} = \lbrace a : a \in M_n(\mathcal{A}_x), x \in X \rbrace$,

\item the map $\vartheta^{(n)}: \mathcal{A}^{(n)} \rightarrow X$ by
\begin{align*}
\vartheta^{(n)}(a) = \vartheta(a_{11})
\hspace{25pt}\text{for }a = (a_{ij})_{1 \leq i,j \leq n}.
\end{align*}
For each $x \in X$, we equip $\mathcal{A}^{(n)}_x = (\vartheta^{(n)})^{-1}(x)$ with the operations and the norm such that $\mathcal{A}^{(n)}_x = M_n(\mathcal{A}_x)$.

\item the set $\Gamma_\vartheta^{(n)}$ of (not necessarily continuous) sections $f: X \rightarrow \mathcal{A}^{(n)}$,

\item the map $\nu_n: M_n(\Gamma_0(\mathcal{A})) \rightarrow \Gamma_\vartheta^{(n)}$ by
\begin{align}
\label{eqn:nunformula}
\nu_n(f)(x) = (f_{ij}(x))_{i \leq i,j \leq n}
\hspace{20pt}\text{for }f = (f_{ij})_{1 \leq i,j \leq n} \in M_n(\Gamma_0(\mathcal{A})),
\end{align}

\item the sets $\Gamma^{(n)}= \nu_n(M_n(\Gamma))$ and $\Gamma^{(n)}_k= \nu_n(M_n(\Gamma_k))$, for $k \geq 1$.
\end{enumerate}
\end{definition}

The following lemma will be needed later to show that $\Gamma_0(\mathcal{A}^{(n)}) \cong M_n(\Gamma_0(\mathcal{A}))$.

\begin{lemma}
\label{lemma:nuninjectivehomo}
Let $\vartheta: \mathcal{A} \rightarrow X$ be an AF bundle, and fix $n \geq 1$. Then $\nu_n: M_n(\Gamma_0(\mathcal{A})) \rightarrow \Gamma_\vartheta^{(n)}$ is an injective $\ast$-homomorphism.
\end{lemma}
\begin{proof}
Note that $\Gamma_\vartheta^{(n)}$ is a $\ast$-algebra if we equip it with the pointwise operations. We show that $\nu_n$ is an homomorphism. It is straightforward that $\nu_n$ is linear. Let $f, g \in \Gamma_\vartheta^{(n)}$ and $x \in X$. Then
\begin{align*}
\nu_n(f g)(x) = ( (fg)_{ij}(x))
= \sum_{k=1}^n f_{ik}(x) g_{kj}(x)
= \nu_n(f)(x) \nu_n(g)(x)
= [\nu_n(f) \nu_n(g)](x),
\end{align*}
and
\begin{align*}
\nu_n(f^*)(x) = (f_{ij}^*(x)) = {f_{ji}(x)}^* = \nu_n(f)^*(x).
\end{align*}
Then $\nu_n$ is a homomorphism.

Finally, we prove that $\nu_n$ is injective. Suppose that $\nu(f) = 0$. Then, we have that each $f_{ij} = 0$. Thus $f = 0$. Therefore $\nu_n$ is injective.
\end{proof}

The result of the next lemma will be used to prove that $\mathcal{A}^{(n)}$ is an AF bundle.

\begin{lemma}
\label{lemma:alphaklnnormpreserving}
Let $\vartheta: \mathcal{A} \rightarrow X$ be an AF bundle. Let $\Gamma$ be a dense subset with local representation $(\Gamma_k, V_{k,l}, \alpha_{k,l}, n_{k,l})_{(k,l) \in I}$. Fix $n \geq 1$ and $(k,l) \in I$. Then we can define the map $\alpha_{k,l}^{(n)}: \Gamma_k^{(n)}\vert_{V_{k,l}} \rightarrow C(V_{k,l}, M_{n n_{k,l}})$ by
\begin{align*}
\alpha_{k,l}^{(n)}(\nu_n(f))(x) = (\alpha_{k,l}(f_{ij})(x))_{i,j}.
\end{align*}
Moreover, $\alpha_{k,l}^{(n)}$ is a support preserving isomorphism and satisfies the equation
\begin{align*}
\Vert \alpha_{k,l}^{(n)}(\nu_n(f))(x) \Vert
= \Vert \nu_n(f)(x) \Vert
\end{align*}
for $f \in M_n(\Gamma)$ and $x \in X$.
\end{lemma}
\begin{proof}
We begin by showing that $\alpha_{k,l}^{(n)}$ is well-defined. Let $f \in M_n(\Gamma_{k,l})$ and $x \in X$. By definition of $\alpha_{k,l}$, we have $\alpha_{k,l}(f_{ij})(x) \in M_{n_{k,l}}$ for all $i,j$ and for $x \in V_{k,l}$. Then $\alpha_{k,l}^{(n)}(\nu_n(f))(x) \in M_{nn_{k,l}}$.

Now we show that $\alpha_{k,l}^{(n)}(\nu_n(f))$ is continuous. Fix $x \in X$ and  Let $\varepsilon > 0$. Then there exists $V_\varepsilon \subset V_{k,l}$ containing $x$ such that, for $y \in V_\varepsilon$,
\begin{align}
\label{eqn:alphaklncontinuous}
\Vert \alpha_{k,l}(f_{ij})(y) - \alpha_{k,l}(f_{ij})(x) \Vert
< \frac{\varepsilon}{n^2}
\hspace{20pt}\text{for $i, j =1, \hdots,n$.}
\end{align}
By the inequality \eqref{eqn:alphaklncontinuous},
\begin{align*}
\Vert \alpha_{k,l}^{(n)}(\nu_n(f))(x) - \alpha_{k,l}^{(n)}(\nu_n(f))(y) \Vert
\leq \sum_{i,j = 1}^n \Vert \alpha_{k,l}(\nu_n(f_{ij}))(x) - \alpha_{k,l}(\nu_n(f_{ij}))(y) \Vert
< \varepsilon.
\end{align*}
Then $\alpha_{k,l}^{(n)}(f)$ is continuous and, therefore, $\alpha_{k,l}^{(n)}$ is well-defined.

Next we prove that $\alpha_{k,l}^{(n)}$ is a $\ast$-homomorphism. It is straightforward that this map is linear. Let $f, g \in \Gamma_k^{(n)}\vert_{V_{k,l}}$ and fix $x \in V_{k,l}$. Then

\begin{align*}
\alpha_{k,l}^{(n)}(\nu_n(fg))(x)
&= (\alpha_{k,l}(fg)_{ij}(x))_{1 \leq i,j \leq n}\\
&= \alpha_{k,l} \left( \sum_{p =1}^n [f_{ip}g_{pj}](x) \right)\\
&= \sum_{p=1}^n [\alpha_{k,l}(f_{ip}) \alpha_{k,l}(g_{pj})](x)\\
&= [\alpha_{k,l}^{(n)}(f)\alpha_{k,l}^{(n)}(g)](x),
\end{align*}
and
\begin{align*}
\alpha_{k,l}^{(n)}(\nu_n(f)^*)(x) = (\alpha_{k,l}(f^*)_{ij}(x))_{1 \leq i,j \leq n}
= (\alpha(f)_{ji}(x)^*)_{1 \leq i,j \leq n}
= \alpha_{k,l}^{(n)}(\nu_n(f))^*(x).
\end{align*}
Thus $\alpha_{k,l}^{(n)}$ is a homomorphism.

Now we show that $\alpha_{k,l}^{(n)}$ is support preserving. Let $f \in M_n(\Gamma_k\vert_{V_{k,l}})$ and $x \in V_{k,l}$. Suppose that $\alpha_{k,l}^{(n)}(\nu_n(f))(x) = 0$. Then, for each $i,j$,
\begin{align*}
\alpha_{k,l}^{(n)}(f_{i,j}(x)) = 0 \Rightarrow f_{i,j}(x) = 0.
\end{align*}
Since $i,j$ is arbitrary, we have $f(x) = 0$. Then $\alpha_{k,l}^{(n)}$ is support preserving. By Lemma \ref{lemma:supportpreservingnorm}, we have
\begin{align*}
\Vert \alpha_{k,l}^{(n)}(\nu_n(f))(x) \Vert
= \Vert \nu_n(f)(x) \Vert
\end{align*}
for $f \in M_n(\Gamma)$ and $x \in X$.
\end{proof}

\begin{proposition}
\label{prop:AnAFbundle}
Let $\vartheta: \mathcal{A} \rightarrow X$ be an AF bundle and fix $n \geq 1$. Let $\Gamma$ be a dense subset of $\Gamma_0(\mathcal{A})$ with local representation $(\Gamma_k, V_{k,l}, \alpha_{k,l}, n_{k,l})_{(k,l) \in I}$. Then there exists a unique topology on $\mathcal{A}^{(n)}$ such that $\vartheta^{(n)}: \mathcal{A}^{(n)} \rightarrow X$ is a C*-bundle. Moreover, $\Gamma^{(n)}$ is dense in $\Gamma_0(\mathcal{A}^{(n)})$ and has local representation $(\Gamma_k^{(n)}, V_{k,l}, \alpha_{k,l}^{(n)}, nn_{k,l})_{(k,l) \in I}$. In particular, $\vartheta^{(n)}: \mathcal{A}^{(n)} \rightarrow X$ is AF.
\end{proposition}
\begin{proof}
We will prove this result by applying Theorem \ref{thm:AFbundlecondition}.

Note that, for every $x \in X$, $\mathcal{A}_x^{(n)} = M_n(\mathcal{A}_x)$ is a C*-algebra. We need to prove that $\Gamma^{(n)}(x)$ is dense in $\mathcal{A}_x^{(n)}$ for all $x \in X$. In fact, fix $x \in X$ and let $a = (a_{ij})_{i,j} \in \mathcal{A}_x^{(n)}$. Since $\Gamma(x)$ is dense in $\mathcal{A}_x$ by Lemma \ref{lemma:Gammaxdense}, then for every $i,j$ there exists $f_{ij} \in \Gamma$ such that
\begin{align*}
\Vert f_{ij}(x) - a_{ij} \Vert < \frac{\varepsilon}{n^2}.
\end{align*}
Let $f = (f_{ij})_{i,j} \in M_n(\Gamma)$. Then $\nu_n(f) \in \Gamma^{(n)}$ and
\begin{align*}
\Vert \nu_n(f)(x) - a \Vert
\leq \sum_{i,j=1}^n \Vert f_{ij}(x) - a_{ij} \Vert < \varepsilon.
\end{align*}
Hence $\Gamma^{(n)}(x)$ is dense in $\mathcal{A}_x^{(n)}$.

We also need to prove that $(\Gamma_k^{(n)}, V_{k,l}, \alpha_{k,l}^{(n)}, nn_{k,l})_{(k,l) \in I}$ is a local representation of $\Gamma^{(n)}$. So we verify the conditions of Definition \ref{def:localrepresentation}.

Since $\nu_n: M_n(\Gamma) \rightarrow \Gamma_\vartheta^{(n)}$ is an injective $\ast$-homomorphism by Lemma \ref{lemma:nuninjectivehomo}, then we have that $\Gamma^{(n)} = \cup_{k = 1}^\infty \Gamma_k^{(n)}$ is an increasing union of C*-algebras. Then condition (i) of Definition \ref{def:localrepresentation} holds.

Now we check condition (ii) of the same definition. We already know that
\begin{align*}
\bigcup_{l=1}^{m_k} V_{k,l} \subset \bigcup_{l=1}^{m_{k+1}} V_{k+1,l}
\hspace{20pt}
\text{for $k \geq 1$}
\end{align*}
because $(\Gamma_k, V_{k,l}, \alpha_{k,l}, n_{k,l})$ is a local representation of $\Gamma$. We need to prove that, for $k \geq 1$, $V_{k,1} \cup \hdots \cup V_{k,m_k}$ is the support of $\Gamma_k^{(n)}$.

Let $x \in X$ be such that there exists an $f = (f_{ij})_{i,j} \in M_n(\Gamma_k)$ with $\Vert \nu(f)(x) \Vert > 0$. Then there exist $i,j$ with $\Vert f_{ij}(x) \Vert > 0$. This implies that $x$ is in the support of $\Gamma_k$, i.e., $x \in \cup_{l=1}^{m_k} V_{k,l}$. Since $x$ is arbitrary and the union $\cup_{l=1}^{m_k} V_{k,l}$ is closed, we have
\begin{align*}
\overline{\lbrace x \in X : \exists f \in \Gamma_k^{(n)} \text{ with } \Vert f(x) \Vert > 0 \rbrace}
\subset
\bigcup_{l=1}^{m_k} V_{k,l}.
\end{align*}
Now we prove that the union of $V_{k,l}$ is a subset of the support of $\Gamma_k^{(n)}$. Fix $x \in \cup_{l=1}^{m_k} V_{k,l}$ and let $W$ be a neighbourhood of $x$. Since $\cup_{l=1}^{m_k} V_{k,l}$ is the support of $\Gamma_k$, then there is a $g \in \Gamma_k$ and $y \in W$ such that $\Vert g(x) \Vert > 0$. Let $f \in M_n(\Gamma_k)$ be such that $f = (f_{ij})_{i,j}$ with $f_{11} = g$ and $f_{ij} = 0$ for $(i,j) \neq (1,1)$. Then
\begin{align*}
\Vert \nu(f)(y) \Vert = \Vert g(y) \Vert > 0.
\end{align*}
Since the neighbourhood $W$ of $x$ is arbitrary, we have that $x$ is in the support of $\Gamma_k^{(n)}$. Then condition (ii) of Definition \ref{def:localrepresentation} holds.

Condition (iii) of Definition \ref{def:localrepresentation} is satisfied by Lemma \ref{lemma:alphaklnnormpreserving}. Therefore, by Theorem \ref{thm:AFbundlecondition}, there exists a unique topology on $\mathcal{A}$ such that $\vartheta^{(n)}: \mathcal{A}^{(n)} \rightarrow X$ is a C*-bundle.Moreover, $\mathcal{A}^{(n)}$ is an AF bundle such that $\Gamma^{(n)}$ is dense in $\Gamma_0(\mathcal{A}^{(n)})$ and $\Gamma^{(n)}$ has local representation $(\Gamma^{(n)}_k, V_{k,l}, \alpha_{k,l}^{(n)}, nn_{k,l})_{(k,l) \in I}$.
\end{proof}

Using the maps $\alpha^{(n)}_{k,l}$, we can prove that $M_n(\Gamma_0(\mathcal{A})) \cong \Gamma_0(\mathcal{A}^{(n)})$.

\begin{corollary}
\label{corollary:nuniso}
Let $\vartheta: \mathcal{A} \rightarrow X$ be an AF bundle and let $n \geq 1$. Let $\Gamma$ be a dense subset of $\Gamma_0(\mathcal{A})$ with local representation $(\Gamma_k, V_{k,l}, \alpha_{k,l}^{(n)}, n_{k,l})_{k,l \geq 1}$. Then $\nu_n(M_0(\Gamma_0(\mathcal{A}))) = \Gamma_0(\mathcal{A}^{(n)})$. From now on, $\nu_n$ denotes the isomorphism $\nu_n: M_n(\Gamma_0(\mathcal{A})) \rightarrow \Gamma_0(\mathcal{A}^{(n)})$ defined by \eqref{eqn:nunformula} on page \pageref{eqn:nunformula}.
\end{corollary}
\begin{proof}
We know from \ref{lemma:nuninjectivehomo} that $\nu_n$ is an injective $\ast$-homomorphism. By Definition  \ref{def:AFndefinitions}, $\Gamma^{(n)} = \nu_n(\Gamma)$. Note that $\Gamma$ is dense in $\Gamma_0(\mathcal{A})$ by assumption. Also, $\Gamma^{(n)}$ is dense in $\Gamma_0(\mathcal{A}^{(n)})$ by Proposition \ref{prop:AnAFbundle}. Therefore $\nu_n(\Gamma_0(\mathcal{A})) = \Gamma_0(\mathcal{A}^{(n)})$.
\end{proof}

Now that we know that $M_n(\Gamma_0(\mathcal{A}))$ is isomorphic to $\Gamma_0(\mathcal{A}^{(n)})$, we will use this isomorphism to extend the definition of the trace $\tr_{\scriptscriptstyle\Gamma,1}$ to $\mathcal{P}_\infty(\Gamma_0(\mathcal{A}))$.

\begin{proposition}
\label{prop:traceGammaextension}
Let $\vartheta: \mathcal{A} \rightarrow X$ be an AF bundle. Then there exists a unique operator $\tr_{\scriptscriptstyle\Gamma}: \mathcal{P}_\infty(\Gamma_0(\mathcal{A})) \rightarrow C_c(X, \mathbb{N})$ such that
\begin{enumerate}[(i)]
\item $\tr_{\scriptscriptstyle\Gamma} p = \sum_{i=1}^n \tr_{\scriptscriptstyle\Gamma,1} p_{ii}$ for $p \in \mathcal{P}_n(\Gamma)$,
\item Given $n \geq1$, $p, q \in \mathcal{P}_n (\Gamma_0(\mathcal{A}))$, we have
\begin{align*}
p \sim q \Leftrightarrow \tr_{\scriptscriptstyle\Gamma} p = \tr_{\scriptscriptstyle\Gamma} q.
\end{align*}
\end{enumerate}
\end{proposition}
\begin{proof}
We divide the proof into three parts:
\begin{enumerate}[(a)]
\item First we define $\tr_{\scriptscriptstyle\Gamma,n}: \mathcal{P}_n(\Gamma) \rightarrow C_c(X, \mathbb{N})$ by
\begin{align*}
\tr_{\scriptscriptstyle\Gamma,n} p = \sum_{i=1}^n \tr_{\scriptscriptstyle\Gamma,1} p_{ii}
\end{align*}
and show that it is well-defined.

\item Then we prove that, for $p, q \in \mathcal{P}_n(\Gamma)$,
\begin{align*}
p \sim q \Leftrightarrow \tr_{\scriptscriptstyle\Gamma,n} p = \tr_{\scriptscriptstyle\Gamma,n} q.
\end{align*}

\item Finally, we extend the definition of trace uniquely to $\mathcal{P}_\infty(\Gamma_0(\mathcal{A}))$.
\end{enumerate}

In (a), to show that $\tr_{\scriptscriptstyle\Gamma,n}$ is well-defined, we will need the isomorphism $\nu_n$ from $M_n(\Gamma_0(\mathcal{A}))$ to $\Gamma_0(\mathcal{A}^{(n)})$. Let $p \in M_n(\Gamma)$. Then there exists $k$ such that $p_{ij} \in \Gamma_k$ for all $i,j$. Given $x$ in the support of $\Gamma_k$, there exists $l$ such that $x \in V_{k,l}$. Then
\begin{align*}
\tr_{\scriptscriptstyle\Gamma^{(n)},1} \nu_n(p)(x)
&= \tr(\alpha_{k,l}^{(n)}(\nu_n(p)(x)) \\
&= \tr( (\alpha_{k,l}(p_{ij}))_{1 \leq i,j \leq n}(x)) \\
&= \sum_{i=1}^n \tr(\alpha_{k,l}(p_{ii})(x)) \\
&= \sum_{i=1}^n \tr p_{ii}(x) \\
&= \tr_{\scriptscriptstyle\Gamma,n} p(x)
\end{align*}
Now suppose that $x \in X$ is not in the support of $\Gamma_k$. Then
\begin{align*}
\tr_{\scriptscriptstyle\Gamma, 1} \nu_n(p)(x) = 0 = \tr_{\scriptscriptstyle\Gamma, n} p(x).
\end{align*}
Therefore,
\begin{align}
\label{eqn:trGamman}
tr_{\scriptscriptstyle\Gamma,n} p = \tr_{\scriptscriptstyle\Gamma^{(n)},1} \nu_n(p) \in C_c(X, \mathbb{N}).
\end{align}
Hence $\tr_{\scriptscriptstyle\Gamma,n} p$ is well-defined.

Now we prove item (b). Let $p, q \in \mathcal{P}_n(\Gamma)$. Then there exists $k$ such that $p, q \in \mathcal{P}_n(\Gamma_k)$. Then
\begin{align}
p \sim q\text{ in }\mathcal{P}_n(\Gamma)
&\Leftrightarrow \nu_n(p) \sim \nu_n(q)
\text{ in }\mathcal{P}(\Gamma_0(\mathcal{A}^{(n)}))
\hspace{20pt}\text{ by the isomorphism $\nu_n$}\nonumber\\
&\Leftrightarrow \tr_{\scriptscriptstyle\Gamma,1} \nu_n(p) = \tr_{\scriptscriptstyle\Gamma,1} \nu_n(q)
\hspace{55pt}\text{by Proposition \ref{prop:traceGamma}}\nonumber\\
&\Leftrightarrow \tr_{\scriptscriptstyle\Gamma,n} p = \tr_{\scriptscriptstyle\Gamma,n} q
\hspace{92pt}\text{by \eqref{eqn:trGamman}.}\label{eqn:psimqGamman}
\end{align}

Now we prove (c). Let $n \geq 1$ and $p \in \mathcal{P}_n(\Gamma_0(\mathcal{A}))$. By Proposition  \ref{prop:pinGamma}, there exists $q \in \mathcal{P}_n(\Gamma)$ such that $\nu_n(p) \sim \nu_n(q)$ in $\Gamma_0(\mathcal{A}^{(n)})$. Then we can define
\begin{align*}
\tr_{\scriptscriptstyle\Gamma} p = \tr_{\scriptscriptstyle\Gamma, n} q.
\end{align*}
By the equivalence \eqref{eqn:psimqGamman}, $\tr_{\scriptscriptstyle\Gamma} p$ does not depend on the choice of $q$ satisfying $\nu_n(p) \sim \nu_n(q)$ in $\Gamma_0(\mathcal{A}^{(n)})$. Moreover, two elements of $\mathcal{P}_n(\Gamma_0(\mathcal{A}))$ are equivalent if, and only if, they have the same trace.
\end{proof}

\begin{corollary}
\label{corollary:psimqAFbundle}
Let $\vartheta: \mathcal{A} \rightarrow X$ be an AF bundle. Given $p, q \in \mathcal{P}_\infty(\Gamma_0(\mathcal{A}))$.  Then $p \sim q$ if, and only if, $\tr_{\scriptscriptstyle\Gamma} p =\tr_{\scriptscriptstyle\Gamma} q$. 
\end{corollary}
\begin{proof}
Let $p, q \in \mathcal{P}_\infty(\Gamma_0(\mathcal{A}))$. Then there are $m,n$ such that $p \in \mathcal{P}_m(\Gamma_0(\mathcal{A}))$ and $q \in \mathcal{P}_n(\Gamma_0(\mathcal{A}))$. Suppose $m \leq n$, swaping $p$ and $q$ if necessary.

If $m = n$, the result holds from Proposition \ref{prop:traceGammaextension}. %If $m < n$, we have that $p \sim q$ if, and only if $p \oplus 0_{n-m} \sim q$ in $\mathcal{P}_n(\Gamma_0(\mathcal{A}))$.

Assume $m < n$. It also follows from Proposition \ref{prop:traceGammaextension} that
\begin{align*}
p \oplus 0_{n-m} \sim q
\Leftrightarrow
\tr_{\scriptscriptstyle\Gamma}(p \oplus 0_{n-m}) = \tr_{\scriptscriptstyle\Gamma} q.
\end{align*}
Note that $p \sim p \oplus 0_{n-m}$. If we show that $\tr_{\scriptscriptstyle\Gamma} p = \tr_{\scriptscriptstyle\Gamma}(p \oplus 0_{n-m})$, then the result holds. But, by Proposition \ref{prop:traceGammaextension},
\begin{align*}
\tr_{\scriptscriptstyle\Gamma}(p \oplus 0_{n-m})
= \sum_{i=1}^m \tr_{\scriptscriptstyle \Gamma, 1} (p \oplus 0_{n-m})
= \sum_{i=1}^n \tr_{\scriptscriptstyle \Gamma, 1} p_{ii}
= \tr_{\scriptscriptstyle \Gamma} p.
\end{align*}
Therefore the result holds.
\end{proof}


==> delete/K0H0-Ktheory.tex <==
\subsection{K-theory for AF bundles}
\label{subsection:K0H0:Ktheory}

In this subsection, we study the K-theory of $\Gamma_0(\mathcal{A})$, where $\mathcal{A}$ is an AF bundle. We will define a trace operator on $\mathcal{P}_\infty(\Gamma_0(\mathcal{A}))$, and we will show that two projections are equivalent if, and only if, they have the same trace.

Our strategy is to generalise the results from Appendix \ref{appendix:C0XMn} to AF bundles. In that subsection, we defined a trace operator on $\mathcal{P}(C_0(X, M_n))$ that distinguishes projections up to equivalence.

Note that, by construction, $\Gamma_0(\mathcal{A})$ is the completion of an increasing union $\Gamma$ of C*-algebras $\Gamma_k$, which are locally isomorphic to C*-algebras of the form $C(V, M_n)$ for some $V$ compact open set. This property will allow us to apply the results of Appendix \ref{appendix:C0XMn} to define a trace operator on $\mathcal{P}(\Gamma_0(\mathcal{A}))$ that characterises the equivalence of projections.

Note, however, that the K-theory of $\Gamma_0(\mathcal{A})$ depends on the equivalence of projections in $\mathcal{P}_\infty(\Gamma_0(\mathcal{A}))$, not just $\mathcal{P}(\Gamma_0(\mathcal{A}))$. Fortunately, we have found a way to define a trace operator on $\mathcal{P}_\infty(\Gamma_0(\mathcal{A}))$ by using similar techniques to $\mathcal{P}(\Gamma_0(\mathcal{A}))$.

The main argument used to define the trace on $\mathcal{P}_\infty(\Gamma_0(\mathcal{A}))$ is the proof of the isomorphism $\mathcal{P}_n(\Gamma_0(\mathcal{A})) \cong \mathcal{P}(\Gamma_0(\mathcal{A}^{(n)}))$, where $\mathcal{A}^{(n)}$ is an AF bundle induced by $\mathcal{A}$. This isomorphism will allow us to define the trace on $\mathcal{P}_\infty(\Gamma_0(\mathcal{A}))$ with the properties we want.

We begin by studying some properties of projections in a C*-algebra $B(\mathcal{H})$ in Subsection \ref{subsection:K0H0:Ktheory:BH}. We will need these properties to show that we can define a trace for projections in $\Gamma$ and extend it uniquely to $\mathcal{P}(\Gamma_0(\mathcal{A}))$. Then, in Subsection \ref{subsection:K0H0:Ktheory:Gamma}, we define the trace on $\mathcal{P}(\Gamma_0(\mathcal{A}))$ and show that it characterises the equivalence of projections in $\Gamma_0(\mathcal{A})$. In Subsection \ref{subsection:K0H0:Ktheory:main}, we extend this result to $\mathcal{P}_\infty(\Gamma_0(\mathcal{A}))$, which allows us to study the K-theory of $\Gamma_0(\mathcal{A})$.

\Ninput{K0H0-Ktheory-BH}
\Ninput{K0H0-Ktheory-Gamma}
\Ninput{K0H0-Ktheory-main}


==> delete/K0H0-Rsigma.tex <==
\subsection{$C^*(R(\sigma))$ as an AF bundle}
\label{section:K0H0:Rsigma}
We will prove that $C^*(R(\sigma))$ is isomorphic to the C*-algebra $\Gamma_0(\mathcal{A}_\varphi)$, where $\vartheta_\varphi: \mathcal{A}_\varphi \rightarrow X_\varphi$ is an AF bundle. It is important to know this isomorphism because it will allow us to apply the results of the previous sections to study the K-theory of the C*-algebras of AF groupoids.

The C*-algebra $C^*(R(\sigma))$ inspired the notion of AF bundles. We wanted to show that the elements of the dense $\ast$-algebra $C_c(R(\sigma))$ can be understood locally as elements of bundles of the form $C(V, M_n)$. We wanted to do this because the K-theory of $C(V, M_n)$ is known, as seen on Appendix \ref{appendix:C0XMn}.

The definition of the reduced norm on $C^*(R(\sigma))$ seems to indicate that this C*-algebra corresponds to a C*-bundle. In fact, recall from \cite[Proposition 3.3.1]{sims2017hausdorff} that, for each $f \in C_c(R(\sigma))$,
\begin{align*}
\Vert f \Vert = \sup_{x \in X} \Vert \pi_x(f) \Vert,
\end{align*}
where each $\pi_x(f)$ is an element of the C*-algebra $B(\ell^2(R(\sigma)_x))$.

Note, however, that the representations $\pi_x: C^*(R(\sigma)) \rightarrow B(\ell^2(R(\sigma)_x))$ are not independent. In fact, by applying \cite[Proposition 3.3.1]{sims2017hausdorff} for $R(\sigma)$, we have that, for every $y \in X$ with $\sigma(y) = \sigma(x)$, there exists a unitary operator $U_{(y,x)}: \ell^2(R(\sigma)_y) \rightarrow \ell^2(R(\sigma)_x)$ such that
\begin{align}
\label{eqn:piyunitary}
\pi_y(f) = U_{(y,x)} \pi_x(f) U_{(y,x)}^*
\hspace{15pt}\text{for }f \in C_c(R(\sigma)).
\end{align}

We believe this dependence could be a problem because, when we study bundles on a topological space $X$, the only thing we need of the space is its topology. We do not know if we can find a bundle where the constraint above is satisfied, so we we want to avoid this dependence.

In order to avoid the constraint mentioned above, we will consider a subset $X_\varphi \subset X$ such that, for each $y \in X$, there exists a unique $x \in X_\varphi$ with $\sigma(x) = \sigma(y)$. In the definition of this set, we consider a continuous section $\varphi: X \rightarrow X$ of $\sigma$ and we define the set $X_\varphi = \varphi(\sigma(X))$.

We will show that, for each $f \in C_c(R(\sigma))$, we can see the map $x \in X_\varphi \mapsto \pi_x(f)$ locally as an element of $C(V, M_n)$.

If we look at the definition of $\pi_x(f)$, we can think of it as a matrix. Indeed, by \cite[Proposition 3.3.1]{sims2017hausdorff} to $R(\sigma)$, we have
\begin{align}
\label{eqn:pixf}
\pi_x(f)\delta_{(y, x)} = \sum_{z : \sigma(z) = \sigma(x)} f(z,y) \delta_{(z,x)}.
\end{align}
Since $f$ is compactly supported, we can find $x_0 = x, x_1, \hdots, x_n$ such that $f(y,z) \neq 0$ implies $y,z \in \lbrace x_0, \hdots, x_n \rbrace$. This will let us represent $\pi_x(f)$ by the finite dimensional matrix
\begin{align}
\label{eqn:pixfmatrix}
\pi_x(f) = [ f(x_j, x_i) ]_{0 \leq i,j \leq n}.
\end{align}
Using the topological properties of $\sigma$, we can find disjoint compact open neighbourhoods $V_i$ of $x_i$, for $i= 0, \hdots, n$, such that $\sigma(V_0) = \sigma(V_i)$ and $\sigma$ is injective on each $V_i$. This allows us to write \eqref{eqn:pixfmatrix} as
\begin{align*}
\pi_x(f) = [f(\sigma\vert_{V_j}^{-1}(\sigma(x)), \sigma\vert_{V_i}^{-1}(\sigma(x))]_{0 \leq i,j \leq n}.
\end{align*}

The topological properties of $f$ and $\sigma$ imply that the map $y \mapsto \pi_y(f)$ is continuous on $V_0$, i.e., we can see $\pi(f)$ locally as an element of $C(V_0, M_n)$. Using this idea we will prove that $\mathcal{A}_\varphi$ is AF and that we have the isomorphism $\pi_\varphi: C^*(R(\sigma)) \rightarrow \Gamma_0(\mathcal{A}_\varphi)$ given by
\begin{align*}
\pi_\varphi(f)(x) = \pi_x(f)
\hspace{15pt}
\text{for }
f \in C_c(R(\sigma)), x \in X_\varphi.
\end{align*}

We begin this subsection by defining the elements needed to build the AF bundle. Then we define the candidate local representation for $\vartheta_\varphi: \mathcal{A}_\varphi \rightarrow X$. Finally, we prove that $\mathcal{A}_\varphi$ is, in fact, an AF bundle with $\Gamma_0(\mathcal{A}_\varphi) \cong C^*(R(\sigma))$.

The next lemma shows that a surjection $\sigma:X \rightarrow W$ always have a continuous section $\varphi$, which we will use to define the bundle $\mathcal{A}_\varphi$. The ideas of the next lemma are taken from the proof of \cite[Theorem 4.10]{FKPS} by Farsi et al.

\newc{
\begin{lemma}
\label{lemma:continuoussection}
Let $X, W$ be locally compact Hausdorff second countable totally disconnected spaces. Let $\sigma: X \rightarrow W$ be a surjective local homeomorphism. Then $\sigma$ has a continuous section $\varphi: W \rightarrow X$. Moreover, $\varphi$ is a local homeomorphism
\end{lemma}
}
\begin{proof}
Using the topological properties of $X$ and $W$, and using the fact that $\sigma$ is a local homeomorphism, we can choose a cover $\lbrace \mathcal{U}_n \rbrace_{n=1}^\infty$ of $X$ by compact open sets such that $\sigma$ is injective on each $\mathcal{U}_n$.

We will define a sequence $\lbrace V_n \rbrace_{n=1}^\infty$ such that $\lbrace \sigma(V_n) \rbrace_{n=1}^\infty$ will be a partition of $X$. Let $V_1 = \mathcal{U}_1$ and, for every $n \geq 0$, set
\begin{align*}
V_{n+1} = \mathcal{U}_{n+1} \setminus \sigma\vert_{\mathcal{U}_n}^{-1} \left( \sigma \left( \bigcup_{i=1}^n \mathcal{U}_i \right) \right)
=  \mathcal{U}_{n+1} \setminus \bigcup_{i=1}^n \sigma\vert_{\mathcal{U}_n}^{-1} (\sigma(\mathcal{U}_i )).
\end{align*}
Note that each $V_n$ is compact open, and that $\sigma$ is injective on each $V_n$. Also, for every $n \geq 0$, we have that $\sigma(V_n)$ is compact and
\begin{align*}
\sigma(V_{n+1}) = \sigma(\mathcal{U}_{n+1}) \setminus \bigcup_{i=1}^n \sigma(\mathcal{U}_i).
\end{align*}
Then the sets $\sigma(V_n)$ are pairwise disjoint. Moreover, since $\lbrace \mathcal{U}_n \rbrace_{n=1}^\infty$ covers $X$, and $\sigma$ is surjective, then we have
\begin{align*}
\bigcup_{n=1}^\infty \sigma(V_n)
&= \sigma(\mathcal{U}_1) \cup
\bigcup_{n=0}^\infty \left(\sigma(\mathcal{U}_{n+1}) \setminus \bigcup_{i=1}^n \sigma(\mathcal{U}_i) \right)\\
&= \bigcup_{n=1}^\infty \sigma(\mathcal{U}_n)\\
&= \sigma \left(\bigcup_{n=1}^\infty \mathcal{U}_n \right)\\
&= \sigma(X)\\
&= W.
\end{align*}
Therefore $\lbrace \sigma(V_n) \rbrace_{n=1}^\infty$ is a partition of $W$.

Let $\varphi: X \rightarrow W$ be such that, for all $n \geq 1$, $\varphi\vert_{\sigma(V_n)}: \sigma(V_n) \rightarrow V_n$ is defined by
\begin{align}
\label{eqn:continuossection}
\varphi\vert_{\sigma(V_n)} = \sigma\vert_{V_n}^{-1}.
\end{align}
Then $\varphi$ is a continuous function by definition. Moreover, $\varphi$ is a local homeomorphism. Finally, we show that $\varphi$ is a section. Let $w \in W$. Then there exists a unique $n \geq 1$ such that $w \in \sigma(V_n)$. Then, by \eqref{eqn:continuossection}, we have
\begin{align*}
\sigma(\varphi(w)) = \sigma( \sigma\vert_{\sigma(V_n)}^{-1}(w)) = w.
\end{align*}
Therefore $\varphi$ is a continuous section.
\end{proof}



\begin{definition}
Let $X, W$ be locally compact Hausdorff second countable totally disconnected spaces. Let $\sigma: X \rightarrow W$ be a surjective local homeomorphism. Let $\varphi: W \rightarrow X$ be a continuous section of $\sigma$. Then we define the set
$X_\varphi
= \lbrace x \in X: x = \varphi(\sigma(x)) \rbrace = \varphi(\sigma(X)).
$
\end{definition}

Note that $X_\varphi \subset X$ is open because $\sigma$ and $\varphi$ are local homeomorphisms.

\begin{remark}
Let $\sigma:X \rightarrow W$ be a surjective local homeomorphism between locally compact Hausdorff second countable totally disconnected spaces. Given $x \in X$, we can extend $\pi_x$ uniquely to a representation $\pi_x: C^*(R(\sigma)) \rightarrow B(\ell^2(R(\sigma)_x)$. From now on, we will denote $\pi_x$ by the representation $\pi_x: C^*(R(\sigma)) \rightarrow B(\ell^2(R(\sigma)_x)$.
\end{remark}

Now we define the candidate set $\mathcal{A}_\varphi$ for the AF bundle. We equip this set with the surjection $\vartheta_\varphi: \mathcal{A}_\varphi \rightarrow X_\varphi$.

\begin{definition}
\label{def:AFvarphi}
Let $\sigma: X \rightarrow W$ be a surjective local homeomorphism between locally compact Hausdorff second countable totally disconnected spaces. Fix a continuous section $\varphi: W \rightarrow X$ of $\sigma$ such that $\varphi$ is a local homeomorphism. Define the set
\begin{align*}
\mathcal{A}_\varphi = \lbrace (x,a) : a \in \pi_x(C^*(R(\sigma)), x \in X_\varphi \rbrace,
\end{align*}
and the map $\vartheta_\varphi: \mathcal{A}_\varphi \rightarrow X_\varphi$ by 
\begin{align*}
\vartheta_\varphi(x,a) = x
\hspace{20pt}
\text{for }
(x,a) \in \mathcal{A}_\varphi.
\end{align*}
We equip $(\mathcal{A}_\varphi)_x = \vartheta^{-1}_\varphi(x) = \lbrace x \rbrace \times \pi_x(C^*(R(\sigma)))$ with the operations of $\pi_x(C^*(R(\sigma)))$ on the second coordinate. Then we have that $(\mathcal{A}_\varphi)_x$ is a C*-algebra isomorphic to $\pi_x(C^*(R(\sigma)))$.
\end{definition}

Now we define the candidate map for the isomorphism $C^*(R(\sigma)) \cong \Gamma_0(\mathcal{A}_\varphi)$.

\begin{definition}
\label{def:pivarphi}
Consider the notation from Definition \ref{def:AFvarphi}. Let $\Gamma_{\vartheta_\varphi}$ denote the set of (not necessarily continuous) sections $f: X_\varphi \rightarrow \mathcal{A}_\varphi$. Let $\pi_\varphi: C_c(R(\sigma)) \rightarrow \Gamma_{\vartheta_\varphi}$ be defined by
\begin{align*}
\pi_\varphi(f)(x) = \pi_x(f)
\hspace{20pt}\text{for $f \in C_c(R(\sigma))$, $x \in X_\varphi$.}
\end{align*}
\end{definition}

\begin{lemma}
\label{lemma:pihomomorphism}
The map $\pi_\varphi$ is an injective $\ast$-homomorphism.
\end{lemma}
\begin{proof}
It is straightforward that $\pi_\varphi$ is linear. Since each $\pi_x$ is a representation, we have that $\pi_\varphi$ is a $\ast$-homomorphism.

The equation \eqref{eqn:piyunitary} on page \pageref{eqn:piyunitary} implies that, for every $f \in C_c(R(\sigma))$,
\begin{align}
\Vert f \Vert
&= \sup_{y \in X} \Vert \pi_y(f) \Vert \nonumber\\
&= \sup_{y \in X} \Vert U_{(y, \varphi(\sigma(y)))} \pi_{\varphi(\sigma(y))}(f) U_{(y, \varphi(\sigma(y)))}^* \Vert \nonumber\\
&= \sup_{y \in X} \Vert \pi_{\varphi(\sigma(y))}(f) \Vert \nonumber\\
&= \sup_{x \in X_\varphi} \Vert \pi_x(f) \Vert. \label{eqn:reducednormvarphi}
\end{align}
If $\pi_\varphi(f) = 0$, then \eqref{eqn:reducednormvarphi} implies that $f = 0$. Thus $\pi_\varphi$ is injective.
\end{proof}

Now that we have the map $\pi_\varphi$, we will define the subset $\Gamma_\varphi = \pi_\varphi(C_c(R(\sigma)))$. Later we will prove that this subset is dense in $\Gamma_0(\mathcal{A}_\varphi)$.

\begin{definition}
\label{def:Gammavarphi}
Using the notation of Definition \ref{def:AFvarphi}, let $\Gamma_\varphi = \pi_\varphi(C_c(R(\sigma)))$. Moreover, given a compact open subset $\mathcal{U} \subset R(\sigma)$, let $\Gamma_\varphi(\mathcal{U}) = \pi_\varphi(C_c(\mathcal{U}))$.
\end{definition}

We want to show that $\Gamma_\varphi$ is a dense $\ast$-algebra in $\Gamma_0(\mathcal{A}_\varphi)$ and that it has a local representation. In order to find the local representation, we will find an increasing family of open subsets $\mathcal{U}_k$, and we will use these sets to define the $\ast$-algebras $\Gamma_{\varphi, k} = \Gamma_\varphi(\mathcal{U}_k)$.

The subsets $\mathcal{U}_k$ will have a property that will guarantee that each $\Gamma_{\varphi, k}$ is a C*-algebra, and this property will also help us to find the support of each $\Gamma_{\varphi, k}$, which is needed to check condition (ii) of Definition \ref{def:localrepresentation}. The property of these subsets is that  $\mathcal{U}_k = \widetilde{\mathcal{U}}_k$, in the notation below. 

%We have defined the candidate for the dense $\ast$-algebra $\Gamma_\varphi$ of $\Gamma_0(\mathcal{A}_\varphi)$. Now we want to find its local representation. This $\ast$-algebra will be the union of an increasing family of C*-algebras $\Gamma_{\varphi, k}$, with $\Gamma_{\varphi, k} = \pi_\varphi(C(\mathcal{U}_k))$ for an increasing sequence of open subsets $\mathcal{U}_k$.

%The subsets $\mathcal{U}_k$ will have two properties: $C(\mathcal{U}_k)$ will be a C*-algebra, and $r(\mathcal{U}_k)$ will be the support of $\Gamma_{\varphi, k}$. The first property and Lemma \ref{lemma:pihomomorphism} will imply that $\Gamma_k$ is a C*-algebra. Note that the second property implies that $r(\mathcal{U}_k) \subset r(\mathcal{U}_{k+1})$. This fact will be helpful to check property (ii) of Definition \ref{def:localrepresentation}.

%In order to have the properties mentioned above, the subsets will be such that $\mathcal{U}_k = \widetilde{\mathcal{U}}_{k}$ in the notation we will introduce now.

%One property these subsets have in common is that $\mathcal{U}_k = \widetilde{\mathcal{U}}_k$. We define the map $\mathcal{U} \mapsto \widetilde{\mathcal{U}}$ below.

\begin{definition}
Let $\sigma: X \rightarrow W$ be a surjective local homeomorphism between locally compact Hausdorff second countable totally disconnected spaces. Let $\varphi: W \rightarrow X$ be a continuous section of $\sigma$. If $\mathcal{U} \subset R(\sigma)$  is compact open, we define
\begin{align*}
\widetilde{\mathcal{U}}
= \lbrace (x,y) \in R(\sigma) : x,y \in r(\mathcal{U}) \cup s(\mathcal{U}) \cup \varphi(r(\mathcal{U})) \rbrace.
\end{align*}
\end{definition}

\begin{remark}
\label{rmk:UinUtilde}
If $\mathcal{U} \subset R(\sigma)$ is compact open as above, then $\mathcal{U} \subset \widetilde{\mathcal{U}}$ and $\widetilde{\mathcal{U}} = \widetilde{\widetilde{\mathcal{U}}}$. Also, $\widetilde{\mathcal{U}}$ is compact open by the topological properties of $r, s, \sigma$ and $\varphi$. If $\mathcal{U}_1 \subset \mathcal{U}_2$ are compact open subsets of $R(\sigma)$, then $\widetilde{\mathcal{U}}_1 \subset \widetilde{\mathcal{U}}_2$.
\end{remark}

\begin{remark}
Suppose that $\mathcal{U} = \widetilde{\mathcal{U}}$. Then $\mathcal{U}$ is closed under the groupoid operations. This implies that $C(\mathcal{U})$ is a $\ast$-algebra.
\end{remark}

Now we define the subsets $\mathcal{U}_V^\varphi$. This definition will help us to prove the isomorphisms $\Gamma_{\varphi,k}\vert_{V_{k,l}} \cong C((\mathcal{U}_{k})_{V_{k,l}}^\varphi) \cong C({V_{k,l}}, M_{n_{k,l}})$.

\begin{definition}
Let $\sigma: X \rightarrow W$ be a surjective local homeomorphism between locally compact Hausdorff second countable totally disconnected spaces. Let $\varphi: W \rightarrow X$ be a continuous section of $\sigma$. Given $\mathcal{U} \subset R(\sigma)$ a compact open set, and $V \subset X_\varphi$ a compact open set, we define the set
\begin{align*}
\mathcal{U}^\varphi_V = \lbrace (x,y) \in \mathcal{U}: \varphi(\sigma(x)) \in V \rbrace.
\end{align*}
\end{definition}

\begin{remark}
Note that $\mathcal{U}^\varphi_V$ is compact open, since $\mathcal{U}$ is compact open and $\varphi \circ \sigma$ is a local homeomorphism.
\end{remark}

\begin{lemma}
\label{lemma:UVIprod}
Let $\sigma: X \rightarrow W$ be a surjective local homeomorphism between locally compact Hausdorff second countable totally disconnected spaces. Let $\varphi: W \rightarrow X$ be a continuous section of $\sigma$ which is also a local homeomorphism. If $\mathcal{U} \subset R(\sigma)$ is a compact open set such that $\mathcal{U} = \widetilde{\mathcal{U}}$, then there exists a partition $V_1, \hdots, V_m$ of $\varphi(r(\mathcal{U}))$ such that for each $i = 1,\hdots, m$, there are pairwise disjoint subsets $V_{i,1} = V_i, V_{i,2}, \hdots, V_{i,n_i} \subset X$ where
\begin{enumerate}[(i)]
\item $\sigma$ is injective on $V_{i,j}$ for all $i,j$.
\item $\sigma(V_{i,j}) = \sigma(V_{i,l})$ for all $i = 1, \hdots, m$ and $j,l = 1, \hdots, n_i$.
\item For each $i$, we have
\begin{align*}
\mathcal{U}_{V_i}^\varphi = R(\sigma) \cap \bigcup_{j, l = 1}^n V_{i,j} \times V_{i,l}.
\end{align*}
\end{enumerate}
\end{lemma}
\begin{proof}
Since $\sigma$ and $r$ are local homeomorphisms, then $\varphi(r(\mathcal{U})) \subset X_\varphi$ is compact open. 

Let $x \in \varphi(r(\mathcal{U}))$. Then $\sigma^{-1}(\sigma(x)) \cap r(\mathcal{U})$ is compact. This implies that there are disjoint compact open sets $\mathcal{O}_{x,1}, \hdots, \mathcal{O}_{x,n_x} \subset X$ that cover $\sigma^{-1}(\sigma(x)) \cap r(\mathcal{U})$ and such that
\begin{enumerate}[(a)]
\item $x \in \mathcal{O}_{x,1} \subset X_\varphi$.
\item $\sigma$ is injective on $\mathcal{O}_{x,j}$ for $j = 1, \hdots, n_x$.
\item $\sigma(\mathcal{O}_{x,j}) = \sigma(\mathcal{O}_{x,1})$ for $j =1, \hdots, n_x$.
\item $\sigma^{-1}(\sigma(\mathcal{O}_{x,1})) \cap r(\mathcal{U}) = \mathcal{O}_{x,1} \cup \hdots \cup \mathcal{O}_{x,n_x}$.
\end{enumerate}
Since $\varphi(r(\mathcal{U}))$ is compact, we can choose $x_1, \hdots, x_m$ such that $\mathcal{O}_{x_1, 1} \cup \hdots \cup \mathcal{O}_{x_m, 1} = \varphi(r(\mathcal{U}))$.

For each $i = 1,\hdots, m$, define $n_i = n_{x_i}$ and
\begin{align*}
V_i =
\begin{cases}
\mathcal{O}_{x_{i,1}} & \text{if }i=1, \\
\mathcal{O}_{x_{i,1}} \setminus \cup_{k=1}^{i-1} \mathcal{O}_{x_{k,1}} & \text{if } 2 \leq i \leq m.
\end{cases}
\end{align*}
We claim that $\mathcal{U}$ is the disjoint union
\begin{align}
\label{eqn:unionUVi}
\mathcal{U} = \bigcup_{i=1}^m \mathcal{U}_{V_i}^\varphi.
\end{align}
In fact, it is straightforward from the definition of the sets $V_i$, that $\varphi(r(\mathcal{U}))$ is the disjoint union $\varphi(r(\mathcal{U})) = V_1 \cup \hdots \cup V_m$. Thus the sets $\mathcal{U}_{V_i}^\varphi$ are disjoint. Let $(u, v) \in \mathcal{U}$.  Then there exists a unique $i$ such that $\varphi(\sigma(u)) \in V_i$. Hence $(u,v) \in \mathcal{U}_{V_i}^\varphi$. This implies that $\mathcal{U} \subset \mathcal{U}_{V_1}^\varphi \cup \hdots \cup \mathcal{U}_{V_m}^\varphi$. Since each $\mathcal{U}_{V_i}^\varphi$ is a subset of $\mathcal{U}$, then \eqref{eqn:unionUVi} holds.

Now fix $i = 1, \hdots, m$. For each $j =1,\hdots, n_i$, define $V_{i,j} = \sigma\vert_{\mathcal{O}_{x_{i,j}}}^{-1}(\sigma(V_i))$. Note that the sets $V_{i,j}$ are disjoint. We claim that
\begin{align}
\label{eqn:UVivarphi}
\mathcal{U}_{V_i}^\varphi = R(\sigma) \cap \bigcup_{j,l=1}^{n_i} V_{i,j} \times V_{i,l}.
\end{align}
Indeed, given $(u,v) \in \mathcal{U}_{V_i}^\varphi$, let $x = \varphi(\sigma(u))$. Then $x \in V_i \subset \mathcal{O}_{x_i}$. By item (d) of the proof, there exists a unique $j$ such that $u \in \mathcal{O}_{x_i,j}$. Then
\begin{align*}
u = \sigma\vert_{\mathcal{O}_{x_{i,j}}}^{-1}(\sigma(x)) \in \sigma\vert_{\mathcal{O}_{x_{i,j}}}^{-1}(\sigma(V_i)) = V_{i,j}.
\end{align*}
Since $\mathcal{U} = \widetilde{\mathcal{U}}$, we have $v \in s(\mathcal{U}) = r(\mathcal{U})$. By the same arguments used for $u$, there exists a unique $l$ such that $v \in V_{i,l}$. Then $(u,v) \in V_{i,j} \times V_{i,l} \cap R(\sigma)$.

So far, we have proved that $\mathcal{U}_{V_i}^\varphi$ is the subset of the union in \eqref{eqn:UVivarphi}. Then, to prove the equality, we only need to show that $V_{i,j} \times V_{i,l} \cap R(\sigma) \subset \mathcal{U}_{V_i}^\varphi$ for $i = 1, \hdots, m$ and $j,l = 1, \hdots, n_i$. Indeed, fix $i,j$ and $l$. Let $(u,v) \in V_{i,j} \times V_{i,l} \cap R(\sigma)$. Then
\begin{align*}
u \in V_{i,j} \subset \mathcal{O}_{x_{i,j}} \subset r(\mathcal{U})
\hspace{20pt}\text{and}\hspace{20pt}
v \in V_{i,l} \subset \mathcal{O}_{x_{i,l}} \subset r(\mathcal{U}).
\end{align*}
Since $\mathcal{U} = \widetilde{\mathcal{U}}$, this implies that $(u,v) \in \mathcal{U}$. Therefore \eqref{eqn:UVivarphi} holds.

It is straightforward from the definition of the sets $V_i$ that properties (i) and (ii) are satisfied.
\end{proof}

The result of the previous lemma will be used now to show that $C(\mathcal{U}_V^\varphi)$ is isomorphic to the C*-algebra $C(V, M_{n})$. This fact will be important to find the local isomorphisms $\alpha_{k,l}$ later.

\begin{lemma}
\label{lemma:betai}
Let $\sigma: X \rightarrow W$ be a surjective local homemorphism between locally compact Hausdorff second countable totally disconnected spaces. Let $\varphi: W \rightarrow X$ be a continuous section of $\sigma$ which is also a local homemorphism. Let $\mathcal{U} \subset R(\sigma)$ be a compact open subset such that $\mathcal{U} = \widetilde{\mathcal{U}}$. Choose $V_1, \hdots, V_m \subset X$ and $V_{i,j} \subset X$ for $i=1,\hdots,m$, $j= 1, \hdots, n_i$, as in Lemma \ref{lemma:UVIprod}. Then, for each $i$, there exists an isomorphism $\beta_i: C(\mathcal{U}_{V_i}^\varphi) \rightarrow C(V_i, M_{n_i})$ given by
\begin{align*}
\beta_i(f)(x) = [f(\sigma\vert_{V_{i,j}}^{-1}(\sigma(x)),\sigma\vert_{V_{i,l}}^{-1}(\sigma(x)))]_{j,l}
\hspace{20pt}\text{for }f \in C(\mathcal{U}_{V_i}^\varphi), x \in V_i,
\end{align*}
such that
\begin{align}
\label{eqn:betaisupport}
\beta_i(f)(x) = 0
\Leftrightarrow
f(u,v) = 0 \text{ for all $u,v \in r(\mathcal{U}_{V_i})$ with $\sigma(u) = \sigma(v) = \sigma(x)$.}
\end{align}
\end{lemma}
\begin{proof}
First we show that $\beta_i(f)$ is well-defined. Note that, for each $i,j$, the maps $\sigma_{V_{i,l}}^{-1}: \sigma(V_i) \rightarrow V_{i,l}$ and $\sigma$ are continuous. By definition of $\beta_i$, given $f \in C(\mathcal{U}_{V_i}^\varphi)$, we have that $x \mapsto \beta_i(f)(x)_{jl}$ is continuous for all $j,l$. Hence, $\beta_i(f) \in C(V_i, M_{n_i})$.

Next we prove that $\beta_i$ is a homomorphism. It is clear that $\beta_i$ is linear. Let $f, f_1, f_2 \in C(\mathcal{U}^\varphi_{V_i})$, $x \in V_i$ and $j,l = 1, \hdots, n_i$. Then
\begin{align*}
\beta_i(f^*)(x)_{jl}
&= f^*(\sigma\vert_{V_{i,j}}^{-1}(\sigma(x)), \sigma\vert_{V_{i,l}}^{-1}(\sigma(x)) \\
&= \overline{f(\sigma\vert_{V_{i,l}}^{-1}(\sigma(x)), \sigma\vert_{V_{i,j}}^{-1}(\sigma(x)))} \\
&= \overline{\beta_i(f)(x)_{lj}} \\
&= \beta_i(f)(x)^*_{jl}.
\end{align*}
Also,
\begin{align}
\beta_i(f_1 \cdot f_2)(x)_{jl}
&= (f_1 \cdot f_2)(\sigma\vert_{V_{i,j}}^{-1}(\sigma(x)), \sigma\vert_{V_{i,l}}^{-1}(\sigma(x))) \nonumber\\
&= \sum_{y: \sigma(y) = \sigma(x)}
    f_1(\sigma\vert_{V_{i,j}}^{-1}(\sigma(x)), y)
    f_2(y, \sigma\vert_{V_{i,l}}^{-1}(\sigma(x))) \label{eqn:betaif1f2}
\end{align}
From Lemma \ref{lemma:UVIprod}, we have that $r(\mathcal{U}_{V_i}^\varphi) = V_{i,1} \cup \hdots \cup V_{i,n_i}$. In the right hand side \eqref{eqn:betaif1f2}, we only need to consider $y \in X$ such that the term in the sum is non-zero. Since $f_1 \in C(\mathcal{U}_{V_i})$, we have
\begin{align*}
f_1(\sigma\vert_{V_{i,j}}^{-1}(\sigma(x)), y) \neq 0
\Rightarrow
y \in \bigcup_{l=1}^n V_{i,l}.
\end{align*}
Hence, since $\sigma\vert_{V_{i,l}} \rightarrow \sigma(V_i)$ is a homeomorphism for all $l = 1, \hdots, n_i$, we can rewrite \eqref{eqn:betaif1f2} as
\begin{align*}
\beta_i(f_1 \cdot f_2)(x)
&= \sum_{p = 1}^{n_i} f_1(\sigma\vert_{V_{i,j}}^{-1}(\sigma(x)), \sigma\vert_{V_{i,p}}^{-1}(\sigma(x))) f_2(\sigma\vert_{V_{i,p}}^{-1}(\sigma(x)), \sigma\vert_{V_{i,l}}^{-1}(\sigma(x))) \\
&= \sum_{p = 1}^{n_i} \beta_i(f_1)_{i,p} (x)\beta_i(f_2)_{p, j} (x) \\
&= [\beta_i(f_1) \cdot \beta_i(f_2)](x)_{i,j}.
\end{align*}
Then $\beta_i$ is a homeomorphism.

Now we show \eqref{eqn:betaisupport}. Let $f \in C(\mathcal{U}_{V_i}^\varphi)$ and $x \in V_i$. Then
\begin{align*}
\beta_i(f)(x) = 0
&\Leftrightarrow
f(\sigma\vert_{V_{i,j}}^{-1}(\sigma(x)), \sigma\vert_{V_{i,l}}^{-1}(\sigma(x))) = 0 \hspace{15pt}\text{for }j,l = 1, \hdots, n_i \\
&\Leftrightarrow f(u,v) = 0
\hspace{15pt}\text{for $u \in V_{i,j}, v \in V_{i,l}$ with $\sigma(u) = \sigma(v) = \sigma(x)$}\\
&\Leftrightarrow f(u,v) = 0
\hspace{15pt}\text{for $u,v \in r(\mathcal{U}_{V_i}^\varphi)
$ with $\sigma(u) = \sigma(v) = \sigma(x)$.}
\end{align*}
Hence, \eqref{eqn:betaisupport} holds. It follows from this property that $\beta_i$ is injective.

Finally, we prove that $\beta_i$ is also surjective. let $g \in C(V_i, M_{n_i})$. Define $f \in \mathcal{U}_{V_i}$ by
\begin{align*}
f(u,v) = g(\varphi(\sigma(u))_{jl}
\hspace{20pt}\text{if } (u,v) \in V_{i,j} \times V_{i,l} \cap R(\sigma),
\text{ for $j,l = 1, \hdots, n_i$, $i = 1,\hdots, m$.}
\end{align*}
Note that $f$ is continuous because it is a composition of continuous functions. Moreover, $\beta_i(f) = g$. This implies that $\beta_i$ is surjective. Therefore $\beta_i$ is an isomorphism.
\end{proof}

Now that we have studied the properties of sets with $\mathcal{U} = \widetilde{\mathcal{U}}$, we will find the local representation of $\Gamma_{\varphi}$.

\begin{definition}
\label{def:fixUk}
Consider the notation from Definition \ref{def:AFvarphi}. From Remark \ref{rmk:UinUtilde}, we can fix
\begin{itemize}
\item an increasing sequence of compact open sets $\mathcal{U}_k$ that cover $R(\sigma)$ such that $\mathcal{U}_k = \widetilde{\mathcal{U}}_k$ for all $k$.
\item a partition $V_{k,1}, \hdots, V_{k,m_k}$ of $r(\mathcal{U}_k)$ for $k \geq 1$, such that, for each $1 \leq l \leq m_k$, we have the compact open sets $V_{k,l,1}, \hdots, V_{k,l,n_{k,l}}$ with the properties given by Lemma \ref{lemma:UVIprod}.
\end{itemize}
then for each $k,l$, we define $\Gamma_{\varphi, k} = \Gamma_\varphi(\mathcal{U}_k)$ and $\Gamma_{\varphi,k,l} = \Gamma_\varphi(\mathcal{U}_k)\vert_{V_{k,l}}$.
\end{definition}

\begin{lemma}
\label{lemma:alphaklvarphi}
Consider the notation of Definition \ref{def:fixUk}. Then, for $k \geq 1, 1 \leq l \leq m_k$, there exists a support preserving isomorphism $\alpha_{k,l}: \Gamma_{\varphi, k, l} \rightarrow C(V_{k,l}, M_{n_{k,l}})$ given by
\begin{align*}
%\alpha_{k,l}(\pi_\varphi(f)) = \beta_{k,l}(f)
\alpha_{k,l}(\pi_\varphi(f))(x) = 
[f(\sigma\vert_{V_{k,l,i}}^{-1}(\sigma(x)), \sigma\vert_{V_{k,l,j}}^{-1}(\sigma(x)))]_{ij}
\hspace{20pt}\text{for }f \in C((\mathcal{U}_k)_{V_{k,l}}^\varphi)
\text{ and }
x \in V_{k,l}.
\end{align*}
\end{lemma}
\begin{proof}
Fix $k$ and $l$. By definition, $\Gamma_{\varphi, k, l} = \Gamma_\varphi((\mathcal{U}_k)_{V_{k,l}}^\varphi)$. We will show that $\Gamma_{\varphi,k,l} = \Gamma_\varphi((\mathcal{U}_k)_{V_{k,l}}^\varphi)$.

We begin by proving $\Gamma_{\varphi}(\mathcal{U}_k)\vert_{V_{k,l}} \subset \Gamma_{\varphi, k,l}$. Let $f \in C(\mathcal{U}_k)$ be such that $\pi_\varphi(f) \in \Gamma_\varphi(\mathcal{U}_k)\vert_{V_{k,l}}$. Hence $\pi_\varphi(f)$ has support in $V_{k,l}$. We will study the elements $(u,v)$ such that $f(u,v) \neq 0$ and we will conclude that $f \in C((\mathcal{U}_k)^\varphi_{V_{k,l}})$.

Choose $(u,v) \in R(\sigma)$ be such that $f(u,v) \neq 0$. Then $\pi_{\varphi(\sigma(u))}9f) \neq 0$. By definition of $\pi_\varphi(f)$, we must have $\varphi(\sigma(u)) \in V_{k,l}$. Thus, $(u,v) \in \mathcal{U}_{V_{k,l}}^\varphi$ and, then, $f \in C(\mathcal{U}_{V_{k,l}}^\varphi)$. This implies that $\Gamma_\varphi((\mathcal{U}_k)_{V_{k,l}}^\varphi)$. Therefore, $\Gamma_{\varphi,k,l} \subset \Gamma_\varphi((\mathcal{U}_k)_{V_{k,l}}^\varphi)$.

Now we prove that $\Gamma_\varphi((\mathcal{U}_k)^\varphi){V_{k,l}}) \subset \Gamma_{\varphi,k,l}$. Let $f \in C((\mathcal{U}_k)^\varphi_{V_{k,l}})$. Since $(\mathcal{U}_k)^\varphi_{V_{k,l}} \subset \mathcal{U}_k$, we have $f \in C(\mathcal{U}_k)$. We only need to prove that $\pi_\varphi(f) \in \Gamma_{\varphi, k,l}$.

Let $x \in X_\varphi$ be such that $\pi_x(f) \neq 0$. Then there exists $(u,v) \in R(\sigma)$ such that $f(u,v) \neq 0$ and $\varphi(\sigma(u)) = x$. Since $(\mathcal{U}_\varphi)^\varphi_{V_{k,l}}$ contains the support of $f$, we have $(u,v) \in (\mathcal{U}_\varphi)^\varphi_{V_{k,l}}$. This implies that $x \in V_{k,l}$. Since $x$ is arbitrary, we have $\pi_\varphi(f) \in \Gamma_\varphi(\mathcal{U}_k)\vert_{V_{k,l}} = \Gamma_{\varphi, k,l}$. Therefore, $\Gamma_{\varphi, k,l} = \Gamma_\varphi((\mathcal{U}_k)_{V_{k,l}^\varphi})$.

Finally, we define $\alpha$. Note from Lemma \ref{lemma:pihomomorphism} that the map $\pi_\varphi$ is an injective $\ast$-homomorphism. In particular, the restriction $T_{k,l}$ of $\pi_\varphi$:
\begin{align*}
T_{k,l}: C((\mathcal{U}_k)_{V_{k,l}}^\varphi) \rightarrow \Gamma_{\varphi, k,l}
\end{align*}
is an isomorphism.

By Lemma \ref{lemma:betai}, there exists an isomorphism $\beta_{k,l}: C((\mathcal{U}_k)_{V_{k,l}}^\varphi) \rightarrow C(V_{k,l}, M_{n_{k,l}})$ given by
\begin{align*}
\beta_{k,l}(f)(x) = [f(\sigma\vert_{V_{k,l,i}}^{-1}(\sigma(x)), \sigma\vert_{V_{k,l,j}}^{-1}(\sigma(x)))]_{ij}
\hspace{20pt}
\text{for $f \in C((\mathcal{U}_k)_{V_{k,l}}^\varphi)$.}
\end{align*}
Here we chose the sets $V_{k,l} = V_{k,l,1}, \hdots, V_{k,l,n_k}$ satisfying the properties of Lemma \ref{lemma:UVIprod}. Moreover, $\beta_{k,l}$ satisfies the following property:
\begin{align}
\label{eqn:betaklsupport}
\beta_{k,l}(f)(x) = 0
\Leftrightarrow
f(u,v) = 0 \text{ for all $u,v \in r(\mathcal{U}_{V_{k,l}})$ with $\sigma(u) = \sigma(v) = \sigma(x)$.}
\end{align}

Let $\alpha_{k,l} = \beta_{k,l} \circ T_{k,l}^{-1}$. By definition, this is an isomorphism from $\Gamma_{\varphi,k,l}$ to the C*-algebra $C(V_{k,l}, M_{n_{k,l}})$. We only need to check that $\alpha_{k,l}$ is also support preserving. Let $f \in C((\mathcal{U}_k)_{V_{k,l}}^\varphi)$ and $x \in V_{k,l}$. Then, by \eqref{eqn:betaklsupport}, we have
\begin{align*}
&\alpha_{k,l}(T_{k,l}(f))(x)
= \beta_{k,l}(f)(x) = 0 \\
\Leftrightarrow&
f(u,v) = 0
\hspace{15pt}
\text{for $u,v \in X$ with $\sigma(u) = \sigma(v) = \sigma(x)$}\\
\Leftrightarrow&
\pi_x(f) = 0.
\end{align*}
Therefore $\alpha_{k,l}$ is support preserving.
%Let $\alpha_{k,l}: \Gamma_{\varphi,k,l} \rightarrow C(V_{k,l}, M_{n_{k,l}})$ be defined by $\alpha_{k,l} = \beta_{k,l} \circ T_{k,l}^{-1}$, where $\beta_k$ is given by Lemma
\end{proof}

Finally, we prove that $\mathcal{A}_\varphi$ is an AF bundle, and we show that $\Gamma_0(\mathcal{A}_\varphi) \cong C^*(R(\sigma))$.

\begin{proposition}
\label{prop:AvarthetaAF}
Let $\sigma: X \rightarrow W$ be a surjective local homemorphism between locally compact Hausdorff second countable totally disconnected spaces. Fix a continuous section $\varphi: W \rightarrow X$ such that $\varphi$ is a local homeomorphism. Then
\begin{enumerate}[(i)]
\item There exists a unique topology on $\mathcal{A}_\varphi$ such that $\vartheta_\varphi: \mathcal{A}_\varphi \rightarrow X_\varphi$ is a C*-bundle.

\item $\Gamma_\varphi$ is dense in $\Gamma_0(\mathcal{A}_\varphi)$ and has local representation $(\Gamma_{\varphi, k}, V_{k,l}, \alpha_{k,l}, n_{k,l})_{(k,l) \in I}$.

\item For every projection $p \in C_c(R(\sigma))$, we have
\begin{align*}
\tr_{{\scriptscriptstyle\Gamma}_\varphi} \pi_\varphi(p) (x)
= \sum_{y: \sigma(y) = \sigma(x)} p(y,y)
\hspace{20pt}\text{for $x \in X_\varphi$.}
\end{align*}
\end{enumerate}
In particular, $\vartheta_\varphi: \mathcal{A}_\varphi \rightarrow X_\varphi$ is an AF bundle. Also, we can extend $\pi_\varphi$ to an isomorphism $\pi_\varphi: C^*(R(\sigma)) \rightarrow \Gamma_0(\mathcal{A}_\varphi)$.
\end{proposition}
\begin{proof}
First we will find a local representation of $\Gamma_\varphi$. By Remark \ref{rmk:UinUtilde} and by the topological properties of $R(\sigma)$, we can choose a sequence of compact open sets $\mathcal{U}_k \subset R(\sigma)$ such that, for each $k \geq 1$, $\mathcal{U}_k  = \widetilde{\mathcal{U}}_k$ and $\mathcal{U}_k \subset \mathcal{U}_{k+1}$. We can also assume that
\begin{align*}
R(\sigma) = \bigcup_{k=1}^\infty \mathcal{U}_k.
\end{align*}

For every $k \geq 1$, let $\Gamma_{\varphi, k} = \pi_\varphi(C(\mathcal{U}_k))$ as in Definition \ref{def:fixUk}. Then $\Gamma_\varphi$ is the increasing union
\begin{align*}
\Gamma_\varphi = \bigcup_{k=1}^\infty \Gamma_{\varphi, k}.
\end{align*}
Let also $V_{k,l}$ be as in that definition. Then we have, for every $k$,
\begin{align}
\label{eqn:Gammavarphik}
\Gamma_{\varphi, k}
= \Gamma_{\varphi}(\mathcal{U}_k)
= \bigoplus_{l=1}^{m_k} \Gamma_\varphi( (\mathcal{U}_k)^\varphi_{V_{k,l}})
= \bigoplus_{l=1}^{m_k} \Gamma_{\varphi,k,l},
\end{align}
since $V_{k,1}, \hdots, V_{k,m_k}$ is a partition of $r(\mathcal{U})$ and $r(\mathcal{U}) = s(\mathcal{U})$.

Also, for each $1 \leq l \leq m_k$, there are compact open sets  $V_{k,l,1}, \hdots, V_{k,l,n_k}$ satisfying the properties of Lemma \ref{lemma:betai}. Moreover, by Lemma \ref{lemma:alphaklvarphi}, there is a support preserving isomorphism $\alpha_{k,l}: \Gamma_{\varphi,k,l} \rightarrow C(V_{k,l}, M_{k,l})$ given by
\begin{align*}
%\alpha_{k,l}(\pi_\varphi(f)) = \beta_{k,l}(f)
\alpha_{k,l}(\pi_\varphi(f))(x) = 
[f(\sigma\vert_{V_{k,l,i}}^{-1}(\sigma(x)), \sigma\vert_{V_{k,l,j}}^{-1}(\sigma(x)))]_{ij}
\hspace{20pt}\text{for }f \in C((\mathcal{U}_k)_{V_{k,l}}^\varphi)
\text{ and }
x \in V_{k,l}.
\end{align*}
Then \eqref{eqn:Gammavarphik} implies that $\Gamma_{\varphi,k}$ is a C*-algebra. Hence condition (i) of Definition \ref{def:localrepresentation} on page \pageref{def:localrepresentation} holds.

We verify property (ii) of the same definition. For each $k$, we have
\begin{align*}
\bigcup_{l=1}^{m_k} V_{k,l}
= r(\mathcal{U}_k)
\subset
r(\mathcal{U}_{k+1})
= \bigcup_{l=1}^{m_{k+1}} V_{k+1,l}.
\end{align*}
Note that, for every $l$, the isomorphism $\alpha_{k,l}$ implies that $V_{k,l}$ is the support of $\Gamma_{\varphi,k,l}$. Equation \eqref{eqn:Gammavarphik} implies that the support of $\Gamma_{\varphi,k}$ is the union of these supports, i.e., it is
\begin{align*}
V_{k,1} \cup \hdots \cup V_{k,m_k} = r(\mathcal{U}_k).
\end{align*}
Then property (ii) of Definition \ref{def:localrepresentation} is also satisfied.

Note that $\alpha_{k,l}$ is support preserving by Lemma \ref{lemma:alphaklvarphi}. Then the properties of Definition \ref{def:localrepresentation} are satisfied. In other words, $(\Gamma_{\varphi, k}, V_{k,l}, \alpha_{k,l}, n_k)_{(k,l) \in I}$ is a local representation of $\Gamma_\varphi$.

Note that $\Gamma_\varphi(x)$ is dense in $\mathcal{A}_x$ for every $x \in X_\varphi$. In fact, for $x \in X_\varphi$, $\Gamma_\varphi(x) = \pi_x(C_c(R(\sigma)))$ is dense in $\mathcal{A}_x = \pi_x(C^*(R(\sigma)))$. Therefore, by Theorem \ref{thm:AFbundlecondition}, there exists a unique topology on $\mathcal{A}_\varphi$ such that $\vartheta_\varphi: \mathcal{A}_\varphi \rightarrow X_\varphi$ is a C*-bundle. Moreover, $\mathcal{A}_\varphi$ is AF and $\Gamma_\varphi$ is dense in $\Gamma_0(\mathcal{A}_\varphi)$.

Finally, we prove property (iii). It is straightforward that this property is holds for $p = 0$. Let $p \in C_c(R(\sigma))$ be a non-zero projection. There exists $k \geq 1$ such that $\pi_\varphi(p) \in \Gamma_{\varphi, k}$. Let $x \in X_\varphi$ be such that $\pi_\varphi(p)(x) \neq 0$. By definition of $\mathcal{U}_k$, there exists $1 \leq l \leq m_k$ such that $x \in V_{k,l}$. Also,
\begin{align*}
\sum_{y: \sigma(y) = \sigma(x)} p(y,y)
&= \sum_{\substack{y: \sigma(y) = \sigma(x) \\ (y,y) \in \mathcal{U}_k}} p(y,y)
\hspace{50pt}
\text{since $p \in C(\mathcal{U}_k)$} \\
&= \sum_{\substack{y: \sigma(y) = \sigma(x) \\ (y,y) \in \mathcal{U}_k^\varphi\vert_{V_{k,l}}}} p(y,y) \\
&= \sum_{y \in V_{k,l,1} \cup \hdots \cup V_{k,l,n_k}} p(y,y)
\hspace{20pt}
\text{by Lemma \ref{lemma:UVIprod}} \\
&= \sum_{i=1}^n p(\sigma\vert_{V_{k,l,i}}^{-1}(\sigma(x)),\sigma\vert_{V_{k,l,i}}^{-1}(\sigma(x))) \\
&= \tr \alpha_{k,l}(\pi_\varphi(p))(x) \\
&= \tr_{{\scriptscriptstyle\Gamma}_\varphi} \pi(p)(x).
\end{align*}
If $x$ is such that $\pi_x(p) = 0$, then
\begin{align*}
\sum_{y: \sigma(y) = \sigma(x)} p(y,y) =  \tr_{{\scriptscriptstyle\Gamma}_\varphi} \pi(p)(x) = 0.
\end{align*}
Thus property (iii) holds.
\end{proof}


==> delete/K0H0-RsigmaH0R0.tex <==
\subsection{The isomorphism $K_0(C^*(R(\sigma))) \cong H_0(R(\sigma))$}
\label{section:K0H0:RsigmaK0H0}

Since we have proved that $C^*(R(\sigma)) \cong \Gamma_0(\mathcal{A}_\varphi)$, we can use the results on AF bundles to study the K-theory the C*-algebra. As we will see, the trace operator defined for AF bundles will be useful to define an isomorphism $K_0(C^*(R(\sigma))) \cong H_0(R(\sigma))$.

We begin this subsection by applying the results from AF bundles to define a trace operator on $\mathcal{P}_\infty(C^*(R(\sigma)))$ that distinguish projections up to equivalence.

\begin{proposition}
\label{prop:tracevarphi}
Let $\sigma: X \rightarrow W$ be a surjective local homeomorphism between locally compact Hausdorff second countable totally disconnected spaces. Fix a continuous section $\varphi: W \rightarrow X$ of $\sigma$. Then we can define uniquely an operator $\tr_\varphi: \mathcal{P}_\infty(C^*(R(\sigma))) \rightarrow C_c(X, \mathbb{Z})$ such that
\begin{enumerate}[(i)]
\item $\tr_\varphi p = \sum_{i=1}^n \tr_\varphi p_{ii}$, for $p \in \mathcal{P}_ n(C^*(R(\sigma)))$.

\item for $p \in \mathcal{P}(C_c(R(\sigma)))$,
\begin{align*}
\tr_\varphi p(x) = \begin{cases}
\displaystyle\sum_{y: \sigma(y) = \sigma(x)} p(y,y)
&\text{if }x \in X_\varphi, \\
0 & \text{otherwise.}
\end{cases}
\end{align*}
\item $p \sim q$ if, and only if, $\tr_\varphi p = \tr_\varphi q$ for $p, q \in \mathcal{P}_\infty(C^*(R(\sigma)))$.
\end{enumerate}
\end{proposition}
\begin{proof}
By Lemma \ref{lemma:pihomomorphism} and Definition \ref{def:Gammavarphi}, $\pi: C_c(R(\sigma)) \rightarrow \Gamma_{\vartheta_\varphi}$  is an injective $\ast$-homomorphism with image $\pi_\varphi(C_c(R(\sigma))) = \Gamma_\varphi$.

Proposition \ref{prop:AvarthetaAF} implies that $\Gamma_\varphi$ is dense in $\Gamma_0(\mathcal{A}_\varphi)$. Hence, we can extend $\pi_\varphi$ continuously to an isomorphism between $C^*(R(\sigma))$ and $\Gamma_0(\mathcal{A}_\varphi)$. We also denote this isomorphism by $\pi_\varphi: C^*(R(\sigma)) \rightarrow \Gamma_0(\mathcal{A}_\varphi)$ with little risk of confusion.

From the theory of C*-algebras \cite[page 94]{Murphy}, for each $n \geq 1$, $\pi_\varphi$ induces the isomorphism $\pi_\varphi: M_n(C^*(R(\sigma))) \rightarrow M_n(\Gamma_0(\mathcal{A}_\varphi))$ given by
\begin{align*}
\pi_\varphi(a) = [\pi_\varphi(a_{ij})]_{i,j}
\hspace{20pt}\text{for $a \in M_n(C^*(R(\sigma)))$.}
\end{align*}
Then, given $p, q \in \mathcal{P}_\infty(C^*(R(\sigma)))$, we have $p \sim q$ if, and only if, $\pi_\varphi(p) \sim \pi_\varphi(q)$.

Let $\tr_\varphi: \mathcal{P}_\infty(C^*(R(\sigma))) \rightarrow C_c(X, \mathbb{Z})$ be defined by
\begin{align*}
\tr_\varphi p(x) = \begin{cases}
\tr_{\scriptscriptstyle\Gamma_\varphi} \pi_\varphi p(x) &\text{if $x \in X_\varphi$,}\\
0 & \text{otherwise.}
\end{cases}
\end{align*}
Then, for $p \in \mathcal{P}_n(C^*(R(\sigma)))$ and $n \geq 1$, Proposition \ref{prop:traceGammaextension} implies that
\begin{align*}
\tr_\varphi p = \tr_{\scriptscriptstyle\Gamma_\varphi} \pi_\varphi (p)
= \sum_{i=1}^n \tr_{\scriptscriptstyle\Gamma_\varphi} \pi_\varphi(p_{ii})
= \sum_{i=1}^n \tr_\varphi p_{ii}.
\end{align*}
Hence property (i) is satisfied.

Now let $p \in C_c(R(\sigma))$ be a projection, and let $x \in X_\varphi$. Then Proposition \ref{prop:AvarthetaAF} implies that
\begin{align*}
\tr_\varphi p(x)
= \tr_{\scriptscriptstyle\Gamma_\varphi} \pi_\varphi(p)(x)
= \sum_{y: \sigma(y) = \sigma(x)} p(y,y).
\end{align*}
So property (ii) holds.

Finally, we prove (iii). Let $p, q \in \mathcal{P}_\infty(C^*(R(\sigma)))$. Then
\begin{align*}
p \sim q
\Leftrightarrow
\pi_\varphi(p) \sim \pi_\varphi(q)
\Leftrightarrow
\tr_{\scriptscriptstyle\Gamma_\varphi} \pi_\varphi(p) \sim \tr_{\scriptscriptstyle\Gamma_\varphi} \pi_\varphi(q)
\Leftrightarrow
\tr_\varphi p = \tr_\varphi q.
\tag*{\qedhere}
\end{align*}
\end{proof}

Proposition \ref{prop:tracevarphi} gives a trace operator on $\mathcal{P}_\infty(C^*(R(\sigma)))$. We want to use this map to define an isomorphism $\nu: K_0(C^*(R(\sigma))) \rightarrow H_0(R(\sigma))$ given by $\nu([p]_0) = [\tr_\varphi p]$. In order to do that, we need to guarantee that $\nu$ does not depend on the choice of the continuous section $\varphi$.

Now we will study the relation between the trace and equivalences in $H_0(R(\sigma))$. If we see $\mathcal{P}(C_c(X, \mathbb{N})) = C_c(X, \lbrace 0, 1 \rbrace)$ as a subset of $\mathcal{P}(C^*(R(\sigma)))$ and extend the trace to $C_c(X, \mathbb{N})$, then the following Lemma shows that two functions are equivalent if, and only if, they have the same trace.

\begin{lemma}
%\label{lemma:traceH0Rsigma}
Let $X, W$ be a locally compact Hausdorff second countable totally disconnected spaces. Let $\sigma: X \rightarrow W$ be a surjective local homemorphism. Given $f_1, f_2 \in C_c(X, \mathbb{N})$, then $f_1 \sim f_2$ in $H_0(R(\sigma))$ if, and only if,
\begin{align}
\label{eqn:traceH0Rsigma}
\sum_{y: \sigma(x) = \sigma(y)} f_1(y) = \sum_{y: \sigma(x) = \sigma(y)} f_2(y)
\hspace{20pt}\text{for }y \in X.
\end{align}
\end{lemma}
\begin{proof}
Let $f_1$ and $f_2 \in C_c(X, \mathbb{N})$ be equivalent in $H_0(R(\sigma))$. Then there exists $F \in C_c(R(\sigma), \mathbb{Z})$ such that, for all $z \in X$,
\begin{align*}
f_1(z)
&= f_2(z) + \partial_1 F(z) \\
&= f_2(z) + s_\ast(F)(z) - r_\ast(F)(z) \\
&= f_2(z) + \sum_{y: \sigma(y) = \sigma(z)} [F(y,z) - F(z,y)].
\end{align*}
Fix $x \in X$. Then
\begin{align*}
\sum_{z: \sigma(z) = \sigma(x)} f_1(y)
&= \sum_{z: \sigma(z) = \sigma(x)} f_2(y)
+ \sum_{z: \sigma(z) = \sigma(x)} \sum_{y: \sigma(y) = \sigma(z)} [F(y,z) - F(z,y)] \\
&= \sum_{z: \sigma(z) = \sigma(x)} f_2(y)
+ \sum_{z: \sigma(z) = \sigma(x)} \sum_{y: \sigma(y) = \sigma(x)} [F(y,z) - F(z,y)] \\
&= \sum_{z: \sigma(z) = \sigma(x)} f_2(y)
+ \sum_{\substack{y : \sigma(y) = \sigma(x) \\ z: \sigma(z) = \sigma(x)}} F(y,z) - \sum_{\substack{y : \sigma(y) = \sigma(x) \\ z: \sigma(z) = \sigma(x)}} F(z,y).
\intertext{Making the change of variables $(y,z) \mapsto (z',y')$ in the third sum, we obtain}
\sum_{z: \sigma(z) = \sigma(x)} f_1(y)
&= \sum_{z: \sigma(z) = \sigma(x)} f_2(y)
+ \sum_{\substack{y : \sigma(y) = \sigma(x) \\ z: \sigma(z) = \sigma(x)}} F(y,z) - \sum_{\substack{y' : \sigma(y') = \sigma(x) \\ z': \sigma(z') = \sigma(x)}} F(y',z') \\
&= \sum_{z: \sigma(z) = \sigma(x)} f_2(y).
\end{align*}
Now we prove the converse. Let $T: C_c(X, \mathbb{N}) \rightarrow C_c(X, \mathbb{N})$ be given by
\begin{align*}
T(f)(x)
= \begin{cases}
\displaystyle\sum_{y: \sigma(y) = \sigma(x)} f(y) & \text{if } x \in X_\varphi, \\
0 & \text{otherwise.}
\end{cases}
\end{align*}
This operator is well-defined. In fact, if $V \subset X$ is a compact open, we have
\begin{align*}
T(1_V)(x)
= 
\begin{cases}
\tr_\varphi 1_V(x) & \text{if }x \in X_\varphi, \\
0 & \text{otherwise.}
\end{cases}
\end{align*}
Note that $\tr_\varphi 1_V \in C_c(X_\varphi, \mathbb{N})$ by Proposition \ref{prop:tracevarphi}. Since $X_\varphi$ is open in $X$, then we have $T(1_V) \in C_c(X, \mathbb{N})$. The set $C_c(X,\mathbb{N})$ is spanned by functions of the for $1_V$ of $V \subset X$ compact open. Then $T$ is well-defined.

Note that, for $f \in C_c(X, \mathbb{N})$ and $x \in X$, we have
\begin{align}
%\label{eqn:Tfvarphisigmax}
T(f)(\varphi(x))
= \sum_{y: \sigma(y) = \sigma(\varphi(\sigma(x))) } f(y)
= \sum_{y: \sigma(y) = \sigma(x) } f(y).
\end{align}

Let $f_1, f_2 \in C_c(X, \mathbb{N})$ be such that \eqref{eqn:traceH0Rsigma} holds. Then $T(f_1) = T(f_2)$. Also, define the set
\begin{align*}
K = \lbrace x \in X : x \in \mathrm{supp\hphantom{.}}f_1 \cup \mathrm{supp\hphantom{.}} f_2 \text{ and } T(f_1)(\varphi(\sigma(x))) \neq 0 \rbrace.
\end{align*}
This set is compact because it is the intesection of the compact set $\mathrm{supp\hphantom{.}}f_1 \cup \mathrm{supp\hphantom{.}} f_2$ and the closed set $(T(f) \circ \varphi)^{-1}(\mathbb{Z} \setminus \lbrace 0 \rbrace)$.

Let $F \in C_c(R(\sigma), \mathbb{Z})$ be defined by
\begin{align*}
F(x,y)
&= \begin{cases}
\displaystyle\frac{f_1(y)f_2(x)}{T(f_1)(\varphi(\sigma(x)))}
& \text{if } (x,y) \in K \times \mathrm{supp\hphantom{.}}f_2,\\
0 &\text{otherwise.}
\end{cases}
\end{align*}
Then, for $x \in K$, we have
\begin{align}
\sum_{y: \sigma(y) = \sigma(x)} F(x,y)
&= \frac{f_1(x)}{T(f_1)(\varphi(\sigma(x)))} \sum_{y: \sigma(y) = \sigma(x)} f_2(y) \nonumber\\
&= \frac{f_1(x)}{T(f_1)(\varphi(\sigma(x)))} T(f_2)(\varphi(x)) \text{\hspace{20pt} by \eqref{eqn:Tfvarphisigmax}} \nonumber\\
&= \frac{f_1(x)}{T(f_1)(\varphi(\sigma(x)))} T(f_1)(\varphi(x)) \text{\hspace{20pt} since $T(f_1) = T(f_2)$} \nonumber\\
&= f_1(x) %\label{eqn:partialFf1}
\end{align}
If $x \in X \setminus K$, we have
\begin{align}
%\label{eqn:partialFf1zero}
\sum_{y: \sigma(y) = \sigma(x)} F(x,y) = 0 = f_1(x).
\end{align}
By similar arguments, and by the equality $T(f_1) = T(f_2)$, we have
\begin{align}
%\label{eqn:partialFf2}
\sum_{y: \sigma(y) = \sigma(x)} F(y,x) = f_2(x)
\hspace{20pt}\text{for $x \in X$.}
\end{align}
Combining, \eqref{eqn:partialFf1}, \eqref{eqn:partialFf1zero} and \eqref{eqn:partialFf2}, we obtain for all $x \in X$,
\begin{align*}
f_1(x) = f_2(x) + \partial_1 F(x).
\end{align*}
Therefore $f_1 \sim f_2$.
\end{proof}

\begin{lemma}
\label{lemma:equivqinPnCcR}
Let $\sigma: X \rightarrow W$ be a surjective local homeomorphism between locally compact Hausdorff second countable totally disconnected spaces. Let $n \geq 1$. Given $p \in \mathcal{P}_n(C^*(R(\sigma))$, there exists $q \in \mathcal{P}_n(C_c(R(\sigma)))$ such that $p \sim q$.
\end{lemma}
\begin{proof}
Let $n \geq 1$. Proposition \ref{prop:AvarthetaAF} implies that $\pi_\varphi: C^*(R(\sigma)) \rightarrow \Gamma_0(\mathcal{A}_\varphi)$ is an isomorphism and that $\Gamma_\varphi = \pi_\varphi(C_c(R(\sigma)))$ is dense in $\Gamma_0(\mathcal{A}_\varphi)$. Also, Corollary \ref{corollary:nuniso} implies that $\nu_n: M_n(\Gamma_0(\mathcal{A}_\varphi)) \rightarrow \Gamma_0(\mathcal{A}_\varphi^{(n)})$ is an isomorphism.

Given $p \in \mathcal{P}_n(C^*(R(\sigma)))$, let $p_\varphi = \nu_n(\pi_\varphi(p)) \in \mathcal{P}(\Gamma_0(\mathcal{A}_\varphi^{(n)}))$. Proposition \ref{prop:pinGamma}, implies that there exists $q_\varphi \in \Gamma_\varphi^{(n)}$ such that $p_\varphi \sim q_\varphi$ in $\Gamma_0(\mathcal{A}_\varphi^{(n)})$. Let $q = \pi_\varphi ^{-1} \circ \nu_n^{-1}(q_\varphi)$. Then $p \sim q$ in $\mathcal{P}_n(C^*(R(\sigma)))$. 
\end{proof}

Now we prove that the candidate for the isomorphism $K_0(C^*(R(\sigma))) \rightarrow H_0(R(\sigma))$, with $[p]_0 \mapsto [\tr_\varphi p]$, does not depend on the choice of the continuous section $\varphi$.

\begin{lemma}
\label{lemma:tracevarphi1sim}
Let $\sigma: X \rightarrow W$ be a surjective local homemorphism between locally compact Hausdorff second countable totally disconnected spaces. Let $\varphi_1, \varphi_2$ be continuous sections of $\sigma$. If $p \in \mathcal{P}_\infty(C^*(R(\sigma)))$, then $\tr_{\varphi_1} p \sim \tr_{\varphi_2} p$ in $H_0(R(\sigma))$.
\end{lemma}
\begin{proof}
Fix $n \geq 1$ and let $p  \in \mathcal{P}_n(C^*(R(\sigma)))$. By Lemma \ref{lemma:equivqinPnCcR}, there exists $q \in \mathcal{P}_n(C_c(R(\sigma)))$ such that $p \sim_0 q$.

Fix $i = 1, \hdots, n$. Then, by item (ii) of Proposition \ref{prop:tracevarphi}, for $x \in X$ we have
\begin{align*}
\sum_{y: \sigma(y) = \sigma(x)} \tr_{\varphi_1} q_{ii}(y)
&= \tr_{\varphi_1} q_{ii} (\varphi_1(\sigma(x))) \\
&= \sum_{y: \sigma(y) = \sigma(\varphi_1(\sigma(x)))} q_{ii}(y,y) \\
&= \sum_{y: \sigma(y) = \sigma(\varphi_2(\sigma(x)))} q_{ii}(y,y) \\
&= \tr_{\varphi_2} q_{ii}(\varphi_2(\sigma(x))) \\
&= \sum_{y: \sigma(y) = \sigma(x)} \tr_{\varphi_2} q_{ii}(y).
\end{align*}
Since $x$ is arbitrary, Lemma \ref{lemma:traceH0Rsigma} implies that $\tr_{\varphi_1} q_{ii} \sim \tr_{\varphi_2} q_{ii}$. Since $i$ is also arbitrary, we have
\begin{align*}
\tr_{\varphi_1} p
&= \tr_{\varphi_1} q \hspace{20pt}\text{by Proposition \ref{prop:tracevarphi}} \\
&= \sum_{i=1}^n \tr_{\varphi_1} q_{ii} \\
&\sim \sum_{i=1}^n \tr_{\varphi_2} q_{ii}\\
&= \tr_{\varphi_2} q \\
&= \tr_{\varphi_2} p. \tag*{\qedhere}
\end{align*}
\end{proof}

Now we prove the isomorphism $K_0(C^*(R(\sigma))) \cong H_0(R(\sigma))$.

\begin{proposition}
\label{prop:isoK0H0}
Let $X, W$ be locally compact Hausdorff second countable totally disconnected spaces. Let $\sigma: X \rightarrow W$ be a surjective local homemomorphism. There exists a unique isomorphism of partially ordered groups $\nu: K_0(C^*(R(\sigma))) \rightarrow H_0(R(\sigma))$ such that
\begin{align}
\label{eqn:isoK0H0nu}
\nu([p]_0) = [\tr_\varphi p ]
\hspace{20pt}\text{for $p \in \mathcal{P}_\infty(C^*(R(\sigma)))$,}
\end{align}
where $\varphi$ is any continuous surjection of $\sigma$.
\end{proposition}
\begin{proof}
Let $\nu^+: K_0(C^*(R(\sigma)))^+ \rightarrow H_0(R(\sigma))^+$ be given by
\begin{align}
\label{eqn:isoK0H0plus}
\nu^+([p]_0) = [\tr_\varphi p].
\end{align}
By item (ii) of Proposition \ref{prop:tracevarphi}, if we fix the continuous section $\varphi$ of $\sigma$, then the map
\begin{align*}
[p]_0 \mapsto [\tr_\varphi p]
\hspace{20pt}\text{$p \in \mathcal{P}_\infty(C^*(R(\sigma)))$}
\end{align*}
is well-defined. We still need to prove that \eqref{eqn:isoK0H0plus} does not depend on the choice of $\varphi$. However, this follows from \ref{lemma:tracevarphi1sim}. Then $\nu^+$ is well-defined. It follows from the definition fo $\nu^+$ that it is a semigroup homomorphism.

We will prove that $\nu^+$ is an isomorphism by showing that $\tr_\varphi p \sim \tr_\varphi q$ implies that $p \sim q$. First we consider $p, q \in \mathcal{P}(C_c(R(\sigma)))$ with $\tr_\varphi p \sim \tr_\varphi q$ in $H_0(R(\sigma))$. Then Lemma \ref{lemma:traceH0Rsigma} implies that, for $x \in X$,
\begin{align*}
\sum_{y: \sigma(y) = \sigma(x)} \tr_\varphi p(y)
= \sum_{y: \sigma(y) = \sigma(x)} \tr_\varphi q(y).
\end{align*}
By definition of $\tr_\varphi$, this is equivalent to
\begin{align*}
\tr_\varphi p(\varphi(\sigma(x))) = \tr_\varphi q(\varphi(\sigma(x))).
\end{align*}
Since $x$ is arbitrary, we have by Proposition \ref{prop:tracevarphi} that $\tr_\varphi p = \tr_\varphi q$. Hence $p \sim_0 q$.

Now consider $p, q \in \mathcal{P}_n(C_c(R(\sigma)))$ such that $\tr_\varphi p \sim \tr_\varphi q$. By similar arguments, we can show that $\tr_\varphi p = \tr_\varphi q$ and then $p \sim_0 q$.

Now let $p, q \in \mathcal{P}_\infty(C^*(R(\sigma)))$ be such that $\tr_\varphi p \sim \tr_\varphi q$. Lemma \ref{lemma:equivqinPnCcR} implies that there are $p_0, q_0 \in \mathcal{P}_\infty(C_c(R(\sigma)))$ such that $p \sim p_0$ and $q \sim_0 q_0$. Since $p_0$ is equivalent to $\mathrm{diag}(p_0,0_k)$, we can assume, by renaming $p$ and $q$ if necessary, that there exists $n$ such that $p_0, q_0 \in \mathcal{P}_n(C_c(R(\sigma)))$. Then
\begin{align*}
\tr_\varphi p_0 = \tr_\varphi p \sim \tr_\varphi q = \tr_\varphi q_0.
\end{align*}
Then, as we have proved,
\begin{align*}
\tr_\varphi p = \tr_\varphi p_0 = \tr_\varphi q_0 = \tr_\varphi q.
\end{align*}
Proposition \ref{prop:tracevarphi} implies that $p \sim q$. Therefore, $\nu^+$ is an isomorphism.

Since $C^*(R(\sigma))$ is AF, we have that 
\begin{align*}
 K_0(C^*(R(\sigma))) = K_0(C^*(R(\sigma)))^+ - K_0(C^*(R(\sigma)))^+
\end{align*}
 by \cite[Section IV.2]{Davidson}. Then, we can extend $\nu^+$ uniquely to an isomorphism between $K_0(C^*(R(\sigma)))$ and $H_0(R(\sigma))$ given by \eqref{eqn:isoK0H0nu}.
\end{proof}


==> delete/K0H0-bundles.tex <==
\subsection{C*-bundles}
\label{subsection:K0H0:bundles}

We can see a C*-bundle $\vartheta: \mathcal{A} \rightarrow X$ as a disjoint union of C*-algebras $\mathcal{A}_x = \vartheta^{-1}(x)$ tied by continuity properties. Consider the space $\Gamma_0(\mathcal{A})$ of continuous functions $f: X \rightarrow \mathcal{A}$ vanishing at infinity and satisfying $f(x) \in \mathcal{A}_x$ for all $x \in X$. Then $\Gamma_0(\mathcal{A})$ is a C*-algebra. The image below illustrates $f \in \Gamma_0(\mathcal{A})$.

\Ninput{figures/fig-bundle}


In this subsection study some properties of C*-bundles described in Dana Williams's book \cite[Appendix C.2]{Williams-crossedproducts}.

\begin{definition}
Let $X$ be a locally compact Hausdorff space. A \newterm{C*-bundle} over $X$ is a continuous open surjection $\vartheta: \mathcal{A} \rightarrow X$ together with operations and norms making each fibre $\mathcal{A}_x = \vartheta^{-1}(x)$ into a C*-algebra such that the following axioms hold.
\begin{enumerate}[(i)]
\item The map $a \mapsto \Vert a \Vert$ is continuous from $\mathcal{A}$ to $\mathbb{R}$.
\item The involution $a \mapsto a^*$ is continuous from $\mathcal{A}$ to $\mathcal{A}$.
\item The maps $(a,b) \mapsto ab$ and $(a,b) \mapsto a + b$ are continuous from $\mathcal{A}^{(2)} \coloneqq \lbrace (a,b) \in \mathcal{A} \times \mathcal{A} : \vartheta(a) = \vartheta(b) \rbrace$ to $\mathcal{A}$.
\item For each $\lambda \in \mathbb{C}$, the map $a \mapsto \lambda a$ is continuous from $\mathcal{A}$ to $\mathcal{A}$.
\item If $\lbrace \lambda a_i \rbrace_i$ is a net in $\mathcal{A}$ such that $\Vert a_i \Vert \rightarrow 0$ and $\vartheta(a_i) \rightarrow x$ in $X$, then $a_i \rightarrow 0_x$, where $0_x$ is the zero element in $\mathcal{A}_x$.
\end{enumerate}
When we assume there is little risk of confusion, we omit $\vartheta$ and $X$, saying that $\mathcal{A}$ is a C*-bundle.
\end{definition}



\begin{definition}
If $\vartheta: \mathcal{A} \rightarrow X$ is any surjection, then $f: X \rightarrow \mathcal{A}$ is called a \newterm{section} if $\vartheta(f(x)) = x$ for all $x \in X$. The set of continuous sections of a C*-bundle is denoted $\Gamma(\mathcal{A})$.
\end{definition}

\begin{definition}
Let $\vartheta: \mathcal{A} \rightarrow X$ be a C*-bundle. We say that a continuous section $f \in \Gamma(\mathcal{A})$:
\begin{enumerate}[(a)]
\item is \newterm{compactly supported} if there exists a compact subset $K \subset X$ such that $f(x) = 0$ for $x \in X \setminus K$;
\item \newterm{vanishes at infinity} if, for every $\varepsilon > 0$, the set $\lbrace x \in X: \Vert f(x) \Vert \geq \varepsilon \rbrace$ is compact.
\end{enumerate}
We let $\Gamma_c(\mathcal{A})$ denote the set of continuous compactly supported sections of $\mathcal{A}$, and we define $\Gamma_0(\mathcal{A})$ as the set of continuous sections of $\mathcal{A}$ that vanish at infinity.
\end{definition}

The proposition below is an application of \cite[Proposition C.23]{Williams-crossedproducts}, which proves that $\Gamma_0(\mathcal{A})$ is a $C_0(X)$-algebra.
\begin{proposition} \cite[Proposition C.23]{Williams-crossedproducts}
\label{prop:Gamma0Cast}
Suppose that $\vartheta: \mathcal{A} \rightarrow X$ is a C*-bundle over $X$. Then $\Gamma_0(\mathcal{A})$ is a C*-algebra with respect to the sup-norm.
\end{proposition}

Note that Proposition \ref{prop:Gamma0Cast} implies that $\Gamma_c(\mathcal{A})$ is dense in $\Gamma_0(\mathcal{A})$.

\begin{example}
Let $X$ be a locally compact Hausdorff space. Then  $C_0(X, M_n)$ is an example of C*-algebra obtained from a C*-bundle. In fact, let $\mathcal{A} = X \times M_n$ and equip this space with the product topology. Let $\vartheta: \mathcal{A} \rightarrow X$ be defined by $\vartheta(x,a) = x$. Consider each $\mathcal{A}_x = \vartheta^{-1}(x) = \lbrace x \rbrace \times M_n$ to be the C*-algebra isomorphic to $M_n$. Then $\mathcal{A}$ is a C*-bundle. Moreover, $\Gamma_0(\mathcal{A})$ is isomorphic to $C(X, M_n)$ and the isomorphism $\mu: C_0(X, M_n) \rightarrow \Gamma_0(\mathcal{A})$ is given by
\begin{align*}
\mu(f)(x) = (x, f(x))
\hspace{18pt}
\text{for }
f \in C_0(X, M_n).
\end{align*}
\end{example}

\begin{definition}
Let $\vartheta: \mathcal{A} \rightarrow X$ be a surjection on a locally compact Hausdorff space $X$. Given a section $f \in \Gamma(\mathcal{A})$ and an open set $V \subset X$, we introduce the following notation: $f\vert_V: X \rightarrow \mathcal{A}$ is the section defined by
\begin{align*}
f\vert_V(x) = \begin{cases}
f(x) &\text{if }x \in V, \\ 0 &\text{otherwise.}
\end{cases}
\end{align*}
\end{definition}

\begin{remark}
Let $\vartheta: \mathcal{A} \rightarrow X$ be an C*-bundle and let $V \subset X$ be compact open subset. If $f \in \Gamma_0(\mathcal{A})$, then we have $f\vert_V \in \Gamma_c(\mathcal{A})$.
\end{remark}

The following results will be important in the study of AF bundles when we show that an AF bundle is, in fact, a C*-bundle. Fell's theorem studies when a surjection $\vartheta: \mathcal{A} \rightarrow X$ can be equipped with unique a topology that makes it C*-bundle. Proposition \ref{prop:Gammadense} studies when a subset $\Gamma$ is dense in the C*-algebra $\Gamma_0(\mathcal{A})$.

\begin{theorem} (Fell) \cite[Theorem C.25]{Williams-crossedproducts}
\label{thm:Fell}
Suppose that $\mathcal{A}$ is a set and $\vartheta: \mathcal{A} \rightarrow X$ is a surjection onto a locally compact space $X$ such that each $\mathcal{A}_x \coloneqq \vartheta^{-1}(x)$ is a C*-algebra. Let $\Gamma$ be a $\ast$-algebra of sections of $\mathcal{A}$ such that
\begin{enumerate}[(a)]
\item for each $f \in \Gamma$, $x \mapsto \Vert f(x) \Vert$ is continuous, and
\item for each $x \in X$, $\lbrace f(x) : f \in \Gamma \rbrace$ is dense in $\mathcal{A}_x$.
\end{enumerate}
Then there is a unique topology on $\mathcal{A}$ such that $\vartheta: \mathcal{A} \rightarrow X$ is a C*-bundle over $X$ with $\Gamma \subset \Gamma(\mathcal{A})$.
\end{theorem}

\begin{proposition} \cite[Proposition C.24]{Williams-crossedproducts}
\label{prop:Gammadense}
Suppose that $\vartheta: \mathcal{A} \rightarrow X$ is a C*-bundle over $X$ and that $\Gamma$ is a subspace of $\Gamma_0(\mathcal{A})$ such that
\begin{enumerate}[(a)]
\item $f \in \Gamma$ and $\varphi \in C_0(X)$ implies $\varphi \cdot f \in \Gamma$, and
\item for each $x \in X$, $\lbrace f(x) : f \in \Gamma \rbrace$ is dense in $\mathcal{A}_x$.
\end{enumerate}
Then $\Gamma$ is dense in $\Gamma_0(\mathcal{A})$.
\end{proposition}

%\begin{example}
%Let $X$ be a locally compact Hausdorff space. Then $C_0(X, M_n)$ is an example of C*-algebra obtained from a C*-bundle. Let $\mathcal{A} = X \times M_n$ and let $\vartheta: \mathcal{A} \rightarrow X$ be defined by $\vartheta(x,a) = x$. If we identify $\mathcal{A}_x = \vartheta^{-1}(x)$ with $M_n$, and let $\Gamma = C_0(X, M_n)$, then Fell's theorem and Proposition \ref{prop:Gammadense} imply that there exists a unique topology on $\mathcal{A}$ such that $\mathcal{A}$ is a C*-bundle and $C_0(X, M_n) = \Gamma_0(\mathcal{A})$.
%\end{example}

Now we introduce some notation.

\begin{definition}
Let $\vartheta: \mathcal{A} \rightarrow X$ be a C*-bundle. Given a subset $\Gamma \subset \Gamma_0(\mathcal{A})$ and a compact subset $K \subset X$, we define the set
\begin{align*}
\Gamma\vert_K = \lbrace f \in \Gamma : f(x) = 0 \text{ for } x \in X \setminus K \rbrace.
\end{align*}
\end{definition}

\begin{definition}
Let $\vartheta: \mathcal{A} \rightarrow X$ be a surjection such that $\mathcal{A}_x = \vartheta^{-1}(x)$ is a C*-algebra for all $x$. Let $\Gamma$ be a subset of (not necessarily continuous) sections $f: X \rightarrow \mathcal{A}$. Given $x \in X$, we define the set
\begin{align*}
\Gamma(x) = \lbrace f(x) : f \in \Gamma \rbrace.
\end{align*}
\end{definition}

Note that, if we want to apply Fell's theorem to a surjection $\vartheta: \mathcal{A} \rightarrow X$ equipped with a $\ast$-algebra of sections $\Gamma$, we need to verify condition (b), i.e., that $\Gamma(x)$ is dense in $\mathcal{A}_x$ for all $x \in X$. The following lemma shows that when $\mathcal{A}$ is an C*-bundle, this property holds for all dense subset $\Gamma \subset \Gamma_0(\mathcal{A})$.

We will need the result of the following lemma in Theorem \ref{thm:AFbundlecondition} when we apply Fell's theorem to show that certain C*-bundles $\mathcal{A}$, named AF bundles, induces othe C*-bundles $\mathcal{A}^{(n)}$ for $n$ arbitrary.

\begin{lemma}
\label{lemma:Gammaxdense}
Let $\vartheta: \mathcal{A} \rightarrow X$ be a C*-bundle, and fix $x \in X$, and fix $x \in X$. Then $\Gamma_0(\mathcal{A})(x) = \mathcal{A}_x$. Moreover, if $\Gamma$ is dense in $\Gamma_0(\mathcal{A})$, then $\Gamma(x)$ is dense in $\mathcal{A}_x$.
\end{lemma}
\begin{proof}
The equation $\Gamma_0(\mathcal{A})(x) = \mathcal{A}_x$ follows from \cite[Proposition C.23]{Williams-crossedproducts}. Since $\Gamma_0(\mathcal{A})$ is a C*-algebra equipped with the supremum norm, then we can define the continuous function $\vartheta_x: \Gamma_0(\mathcal{A}) \rightarrow \mathcal{A}_x$ by
\begin{align*}
\vartheta_x(f) = f(x) \hspace{20pt}\text{for $f \in \Gamma_0(\mathcal{A})$.}
\end{align*}
Since $\Gamma$ is dense in $\Gamma_0(\mathcal{A})$, we have that $\Gamma(x)$ is dense in $\Gamma_0(\mathcal{A})(x) = \mathcal{A}_x$.
\end{proof}


==> delete/homology-AF.tex <==
\subsection{AF groupoids}
\label{subsection:homology:AF}

\obs{....:....:....:....:....:....:....:....:....:....:....}

Now we define AF groupoids as in Farsi et al \cite[Definition 4.9]{FKPS}. We also prove that its homology group is an inductive limit of groups.

The definition of AF groupoids depends on the notion of inductive limits of group-oids, which can be found in Renault's book \cite[Section III.1]{Renault}.

\begin{definition}
Let $\lbrace G_n \rbrace_{n=1}^\infty$ be an increasing sequence of topological groupoids such that $G_n$ is open in $G_{n+1}$ and $G_n^{(0)} = G_{n+1}^{(0)}$ for all $n$. Let $G = \cup_{n=1}^\infty G_n$ and equip $G$ with the topology such that a subset $V \subset G$ is open if, and only if, $V \cap G_n$ is open in $G_n$ for all $n$. We say that $G$ is the \newterm{inductive limit} of the sequence, and we call its topology the \newterm{inductive limit topology}. We write $G = \displaystyle\lim_\rightarrow G_n$.
\end{definition}

Now we define AF groupoids.

\begin{definition}
\label{def:AFgroupoid}
A groupoid $G$ is \newterm{AF} if $G^{(0)} = X$ is a locally compact Hausdorff second countable totally disconnected and $G$ is an increasing union of a sequence of open subgroupoids $G_n$ such that, for each $n \geq 1$, $G_n^{(0)} = X$ and $G_n$ is isomorphic to $R(\psi_n)$ for some surjective local homeomorphism $\psi_n: X \rightarrow W_n$.
\end{definition}

\begin{remark}
\label{rmk:limK0}
Note that, for an AF groupoid $G = \displaystyle\lim_\rightarrow G_n$, we have $K_0(C^*(G)) = \displaystyle\lim_\rightarrow K_0(C^*(G_n))$ as an inductive limit of ordered groups. We also have $H_0(G) = \displaystyle\lim_\rightarrow H_0(G_n)$ by  Lemma \ref{lemma:limH0}. This property will be useful in the proof of the isomorphism $K_0(C^*(G)) \cong H_0(G)$ in Section \ref{section:K0H0}.
\end{remark}


\obs{....:....:....:....:....:....:....:....:....:....:....}

We define inductive limit of groupoids as in Renault's book \cite[Section III.1]{Renault}.

%\begin{definition}
%Let $G$ be a groupoid. Suppose that $G$ is the union of an increasing sequence of subgroupoids $G_n$, which all have the same unit space as $G$; then we say that $G$ is the inductive limit of the sequence $G_n$. If $G$ is topological, we require that each $G_n$ is an open subgroupoid of $G$.
%\end{definition}




==> delete/homology-inductive.tex <==
\section{Inductive limits of groups}
\label{subsection:homology:inductive}

\obs{Delete this section? Note that we have an appendix now}

\obs{Explained inductive limits in Renault's AF definition}

We define the inductive limit of groups as in Section 6.2 of R\o{}rdam, Larsen  and Laustsen's book on K-theory \cite{RLL-Ktheory}. %This reference defined this for categories in general, but here we restrict out attention to groups.





%When $\mathscr{C}$ is the category of groups or groupoids, we will use the notation of \cite[Corollary 5.2]{FKPS} and write
%\begin{align*}
%A = \lim_\rightarrow (A_n, \varphi_n),
%\end{align*}
%as the inductive limit of the inductive sequence in Definition \ref{def:inductivelimit}. If the connecting maps are implicit, we just write $A = \displaystyle\lim_\rightarrow A_n$.
%\end{remark}

%\begin{lemma}
%Consider the inductive sequence
%$$
%\begin{tikzcd}
%A_1 \arrow[r, hook, "\varphi_1"] &
%A_2 \arrow[r, hook, "\varphi_2"] &
%A_3 \arrow[r, hook, "\varphi_3"]  &
%\cdots
%\end{tikzcd}
%$$
%in a category $\mathscr{C}$ such that each $A_n$ is a set with $A_n \subset A_{n+1}$, and $\varphi_n: A_n \rightarrow A_{n+1}$ is the including map. Then
%\begin{align*}
%\bigcup_{n=1}^\infty A_n = \lim_\rightarrow A_n.
%\end{align*}
%\end{lemma}
%\begin{proof}
%Let $A = \cup_{n=1}^\infty A_n$, and let $\iota_n: A_n \rightarrow A$ be the inclusion map for all $n \geq 1$. Then $\iota_{n+1} \circ \varphi_n = \iota_n$.

%Let $(B, \lbrace \lambda_n \rbrace_{n=1}^\infty)$ be a pair such that $\lambda_n: A_n \rightarrow B$ is a morphism where $\lambda_n = \lambda_{n+1} \circ \varphi_n$ for all $n$. Since $A$ is precisely the union of the sets $A_n$, there exists a unique morphism $\lambda: A \rightarrow B$ making the diagram
%$$
%\begin{tikzcd}
%& A_n \arrow[dl, hook', "\iota_n", swap] \arrow[dr, "\lambda_n"] \\
%A \arrow[rr, "\lambda"] && B
%\end{tikzcd}
%$$
%commutative. Therefore $A = \displaystyle\lim_\rightarrow A_n$.
%\end{proof}

%SEE 2021-09-27apagar.txt


==> figures/delete/fig-diagram-iso1.tex <==
\begin{figure}[!h]
\center
\begin{subfigure}{0.4\textwidth}
\begin{tikzcd}
      K_0(B) \arrow[r, "K_0(\beta)"]
      & K_0(B) \\
      H_0(\mathcal{G}(c)) \arrow[u, ""] \arrow[r, "{[\widetilde{\beta}]}_{\mathcal{G}(c)}"] & H_0(\mathcal{G}(c)) \arrow[u, ""]
\end{tikzcd}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\begin{tikzcd}
      {[f]}_{K_0(B)} \arrow[r, "", mapsto]
      & {[\beta(f)]}_{K_0(B)} \\
      {[f]}_{\mathcal{G}(c)} \arrow[u, "", mapsto] \arrow[r, "",mapsto] & {[\beta(f)]}_{\mathcal{G}(c)}  \arrow[u, "", mapsto]
\end{tikzcd}
\end{subfigure}
\end{figure}



==> figures/delete/fig-diagram-iso2.tex <==
\pagebreak
\begin{figure}[!h]
\center
\begin{subfigure}{0.4\textwidth}
\begin{tikzcd}
      H_0(\mathcal{G}(c)) \arrow[r, "{[\widetilde{\beta}]}_{\mathcal{G}(c)}"] & H_0(\mathcal{G}(c))\\
      H_0(c^{-1}(0)) \arrow[u,"H_0(\eta)"] \arrow{r}{[ \gamma ] = [\sigma_\ast] }[swap]{} & H_0(c^{-1}(0))  \arrow{u}{}[swap]{H_0(\eta)}
\end{tikzcd}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\begin{tikzcd}
      {[\eta_\ast^{(0)}(f)]}_{\mathcal{G}(c)} \arrow[r, "", mapsto]
      & {[\widetilde{\beta} \circ \eta_\ast^{(0)}(f)]}_{\mathcal{G}(c)} \\
      {[f]} \arrow[u, "", mapsto] \arrow[r, "",mapsto] & {[\sigma_\ast(f)]}  \arrow[u, "", mapsto]
\end{tikzcd}
\end{subfigure}
\end{figure}



==> figures/delete/fig-diagram-iso3.tex <==
\begin{figure}[!h]
\center
\begin{subfigure}{0.4\textwidth}
\begin{tikzcd}
      H_0(R(\sigma^n)) \arrow[r, "\iota_n"] \arrow[d, "{[\sigma_\ast]_n}"] & H_0(c^{-1}(0)) \arrow[d, "{[\sigma_\ast]_n}"]\\
      H_0(R(\sigma^n)) \arrow{r}{\iota_n}[swap]{} & H_0(c^{-1}(0))
\end{tikzcd}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\begin{tikzcd}
      {[f]}_n \arrow[r, "", mapsto] \arrow[d, "", mapsto]
      & {[f]} \arrow[d, "", mapsto] \\
      {[\sigma_\ast(f)]}_n \arrow[r, "", mapsto]
      & {[\sigma_\ast(f)]}
\end{tikzcd}
\end{subfigure}
\end{figure}



==> figures/delete/fig-diagram-iso4.tex <==
\begin{figure}[!h]
\center
\begin{subfigure}{0.4\textwidth}
\begin{tikzcd}
      H_0(R(\sigma^n)) \arrow[r, "{[\sigma_\ast]}_n"] \arrow[d, "H_0(\rho_n)"] & H_0(R(\sigma^n))  \arrow[d, "H_0(\rho_n)"]\\
      C_c(X,\mathbb{Z}) \arrow{r}{\sigma_\ast}[swap]{} & C_c(X,\mathbb{Z})
\end{tikzcd}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\begin{tikzcd}
      {[f]}_n \arrow[r, "", mapsto] \arrow[d, "", mapsto]
      & {[\sigma_\ast(f)]}_n \arrow[d, "", mapsto] \\
      \sigma_\ast^n(f) \arrow[r, "", mapsto]
      & \sigma_\ast^{n+1}(f)
\end{tikzcd}
\end{subfigure}
\end{figure}



==> figures/delete/fig-diagram.tex <==
\begin{figure}[h!]
 \centering
\begin{tikzcd}
      K_0(B) \arrow[r, "K_0(\beta)"]
      & K_0(B) \\
      H_0(\mathcal{G}(c)) \arrow[u, "\circledRed{1}"] \arrow[r, "{[\widetilde{\beta}]}_{\mathcal{G}(c)}"] & H_0(\mathcal{G}(c)) \arrow[u, ""]\\
      H_0(c^{-1}(0)) \arrow[u,"\circledRed{2}"] \arrow{r}{[ \gamma ] = [\sigma_\ast] }[swap]{} & H_0(c^{-1}(0))  \arrow[u,""] \\
      \displaystyle\lim_{\longrightarrow} H_0(R(\sigma^n)) \arrow{u}{\circledRed{3}}[swap]{} \arrow{r}{[ \sigma_\ast ]_n }[swap]{}
      &\displaystyle\lim_{\longrightarrow} H_0(R(\sigma^n)) \arrow[u, "\cong"]\\
      \displaystyle\lim_{\longrightarrow} (C_c(X, \mathbb{Z}), \sigma_\ast)
      \arrow{r}{\tau}[swap]{} \arrow{u}{\circledRed{4}}[swap]{\cong}
      & \displaystyle\lim_{\longrightarrow} (C_c(X, \mathbb{Z}), \sigma_\ast)
       \arrow[u, "\cong"]
\end{tikzcd}
\end{figure}


==> figures/delete/fig-diagram123.tex <==
\begin{tikzcd}
H_0(R(\sigma^m))
\arrow[r,"\iota_{m,n}"]
\arrow[d,""]
&  H_0(R(\sigma^{m+n})) \arrow[d,""]
& \left[f\right]_m
\arrow[r,"\iota_{m,n}",mapsto]
\arrow[d,"", mapsto]
& \left[f\right]_{m+n}
\arrow[d,"", mapsto]\\
C_c(X, \mathbb{Z}) \arrow[r,"\sigma_\ast^n"]
& C_c(X, \mathbb{Z})
& \sigma_\ast^m(f) \arrow[r,"\sigma_\ast^n"]
& \sigma_\ast^{m+n}(f)
\end{tikzcd}


==> figures/fig-bundle.tex <==
\begin{figure}[H]
%\label{eqn:diagram}
%\label{fig:diagram}
 \centering
\begin{tikzpicture}[scale=1.5]
\draw[-{Latex[length=1.5mm]}] (0,.13) to (4,.13);
\node at (4.18,.12) {\small$X$};

\draw[dotted] (2,0.12) to (2,1.5);
\node at (2.25,.7) {\small$\mathcal{A}_x$};

\node at (2,0) {\small$x$};

\draw (0,.5) to[out=10,in=180] (2,1.5) to[out=0,in=160] (3.9,.7);
\node at (2.1,1.7) {\footnotesize$f(x)$};

%\draw[-{Latex[length=1.5mm]}] (0,0) to[out=60,in=180] (5,0);
\end{tikzpicture}
\caption{A element $f$ of the C*-algebra $\Gamma_0(\mathcal{A})$.}
\end{figure}


==> figures/fig-coveringmap.tex <==
\begin{figure}[H]
%\label{eqn:diagram}
%\label{fig:diagram}
 \centering
\begin{tikzpicture}[scale=0.7]

\draw (0,0)  to[out=330,in=210]
      (1,0)  to[out=30, in=320]
      (1,.7) to[out=140, in=40]
      (0,.7) to[out=220, in=140] cycle;

\draw (2.5,0)  to[out=330,in=210]
      (3.5,0)  to[out=30, in=320]
      (3.5,.7) to[out=140, in=40]
      (2.5,.7) to[out=220, in=140] cycle;

\draw (5,0)  to[out=330,in=210]
      (6,0)  to[out=30, in=320]
      (6,.7) to[out=140, in=40]
      (5,.7) to[out=220, in=140] cycle;
      
\draw[-{Latex[length=1.5mm]}] (0.5,1.1) to[out=70, in=220] (1.7, 2.5);
\draw[-{Latex[length=1.5mm]}] (3,1.1) to[out=90, in=270] (2.1, 2.4);
\draw[-{Latex[length=1.5mm]}] (5.1,.95) to[out=120, in=300] (2.5, 2.5);
\draw[-{Latex[length=1.5mm]}] (4,2.2) to[out=160, in=330] (2.7, 2.7);

\node at (0,1.05) {\scriptsize $\mathcal{U}_1$};
\node at (2.5,1.05) {\scriptsize $\mathcal{U}_2$};
\node at (4.7,.9) {\scriptsize $\mathcal{U}_3$};

% \draw (3,3) ellipse (.5cm and .5cm);
\draw (2.1,3) ellipse (.5cm and .5cm);
\node at (2.1,3.75) {\scriptsize $W$};

\node[rotate=342] at (4.4,2.05) {\scriptsize $\dots$};
\node at (7.2,.3) {\large $\dots$};

\node at (.9,2.05) {\scriptsize $\sigma$};
\node at (2.1,1.7) {\scriptsize $\sigma$};
\node at (3.2,1.6) {\scriptsize $\sigma$};
\node at (3.4,2.1) {\scriptsize $\sigma$};


%\draw[-{Latex[length=1.5mm]}] (0,.13) to (4,.13);
%\node at (4.18,.12) {\small$X$};

%\draw[dotted] (2,0.12) to (2,1.5);
%\node at (2.25,.7) {\small$\mathcal{A}_x$};

%\node at (2,0) {\small$x$};

%\draw (0,.5) to[out=10,in=180] (2,1.5) to[out=0,in=160] (3.9,.7);
%\node at (2.1,1.7) {\footnotesize$f(x)$};

\end{tikzpicture}
%\caption{A element $f$ of the C*-algebra $\Gamma_0(\mathcal{A})$.}
%\caption{When $\sigma$ is a covering map, locally we can decompose $\sigma^{-1}(W)$ are disjoint union of sets $\mathcal{U}_i$ which are homeomorphic to $W$ by $\sigma$.}
\caption{Locally, a covering map has the property represented by this figure.}
\end{figure}


==> figures/fig-diagram-iso1.tex <==
\begin{figure}[!ht]
\center
\begin{subfigure}{0.4\textwidth}
\begin{tikzcd}
      K_0(B) \arrow[r, "K_0(\beta)"]
      & K_0(B) \\
      H_0(\mathcal{G}(c)) \arrow[u, ""] \arrow[r, "{[\widetilde{\beta}]}_{\mathcal{G}(c)}"] & H_0(\mathcal{G}(c)) \arrow[u, ""]
\end{tikzcd}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\begin{tikzcd}
      {[f]}_{K_0(B)} \arrow[r, "", mapsto]
      & {[\beta(f)]}_{K_0(B)} \\
      {[f]}_{\mathcal{G}(c)} \arrow[u, "", mapsto] \arrow[r, "",mapsto] & {[\beta(f)]}_{\mathcal{G}(c)}  \arrow[u, "", mapsto]
\end{tikzcd}
\end{subfigure}
\end{figure}



==> figures/fig-diagram-numbered.tex <==
\begin{figure}[!ht]
 \centering
\begin{tikzcd}
      K_0(B) \arrow[r, "K_0(\beta)"]
      & K_0(B) \\
      H_0(\mathcal{G}(c)) \arrow{u}{\circledRed{1}}[swap]{\cong} \arrow[r, "{[\widetilde{\beta}]}_{\mathcal{G}(c)}"] & H_0(\mathcal{G}(c)) \arrow{u}{\cong}[swap]{}\\
      H_0(c^{-1}(0)) \arrow{u}{\circledRed{2}}[swap]{\cong} \arrow{r}{[\sigma_\ast] }[swap]{} & H_0(c^{-1}(0))  \arrow{u}{\cong}[swap]{} \\
      \displaystyle\lim_{\longrightarrow} H_0(R(\sigma^n)) \arrow{u}{\circledRed{3}}[swap]{\cong} \arrow{r}{}[swap]{}
      &\displaystyle\lim_{\longrightarrow} H_0(R(\sigma^n)) \arrow[u, "\cong"]\\
      \displaystyle\lim_{\longrightarrow} (C_c(X, \mathbb{Z}), \sigma_\ast)
      \arrow{r}{\tau}[swap]{} \arrow{u}{\circledRed{4}}[swap]{\cong}
      & \displaystyle\lim_{\longrightarrow} (C_c(X, \mathbb{Z}), \sigma_\ast)
       \arrow[u, "\cong"]
\end{tikzcd}
\end{figure}


==> figures/fig-diagram-part3.tex <==
\begin{figure}[!ht]
\center
\begin{subfigure}{0.4\textwidth}
\begin{tikzcd}
      H_0(R(\sigma^n)) \arrow[r, ""] \arrow[d, "{[\sigma_\ast]_n}"] & H_0(c^{-1}(0)) \arrow[d, "{[\sigma_\ast]_n}"]\\
      H_0(R(\sigma^n)) \arrow{r}{}[swap]{} & H_0(c^{-1}(0))
\end{tikzcd}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\begin{tikzcd}
      {[f]}_n \arrow[r, "", mapsto] \arrow[d, "", mapsto]
      & {[f]} \arrow[d, "", mapsto] \\
      {[\sigma_\ast(f)]}_n \arrow[r, "", mapsto]
      & {[\sigma_\ast(f)]}
\end{tikzcd}
\end{subfigure}
\end{figure}



==> library.tex <==
\chapter{Library requirements}\label{C:lib}

This Chapter describes some things done to be in accordance with the `Library Requirements for the Deposit of Theses' booklet, which can be obtained from the VUW library.

\section{Font size}
\textit{12 point font is recommended.} 

Set this yourself with the \verb+12pt+ option to the document class.

\section{Single or double sided}
\textit{Typing on one side preferred, text on both sides acceptable for longer works.} 

Use the \verb+oneside+ or \verb+twoside+ option to the document class. The \textsf{book} class default is \verb+twoside+.


\section{Line spacing}
\textit{Lines should be double spaced, or at least 1.5 spaces apart.} 

1.5 spacing for 12 point is set using:
\begin{itemize}
\item \verb+\renewcommand{\baselinestretch}{1.24}+  
\end{itemize}

To set anything else use, e.g  \verb+\renewcommand{\baselinestretch}{1.0}+ in the preamble. See p 53 of \cite{GMS94} for more information.


\section{Margins}
\textit{Uniform margins of at least 4cm on binding side, other three sides to have at least 1.5 cm}

\LaTeX\ styles often leave a lot of white space, and \textsf{book} is no exception. We only have to worry about the binding side.

For \verb+twoside+ we use these settings:
\setlength{\textheight}{19.8cm}
\setlength{\oddsidemargin}{1.46cm}
\setlength{\evensidemargin}{0.83cm}

For \verb+oneside+, if we use:
\begin{verbatim}
\setlength{\textheight}{19.8cm}
\setlength{\oddsidemargin}{1.46cm}
\end{verbatim}

Then \textsf{book} gives a margin of 4cm on the binding side, and about 3.2cm elsewhere.

If you want to change these then use the \textsf{layout} package.

\section{Paper size}
\textit{High quality A4 paper, all pages of equal size}

Set this yourself with the \verb+a4paper+ option to the document class.

==> result.tex <==
\chapter{Main result}
\label{section:result}

Our main result is Theorem \ref{thm:AFEDR}, where we give a condition on $\sigma: X \rightarrow X$ that makes $C^*(\mathcal{G})$ AF embeddable. The condition is
\begin{align}
\label{eqn:maincondition}
C^*(\mathcal{G}) \text{ is AFE }
\Leftrightarrow
(\sigma_\ast - \mathrm{id}) \cap C_c(X, \mathbb{N}) = \lbrace 0 \rbrace.
\end{align}

We prove this condition by applying the commutative diagram of Chapter \ref{section:diagram} to find a condition which is equivalent to the equation $H_\beta \cap K_0(B) = \lbrace 0 \rbrace$ of Brown's theorem (Theorem \ref{thm:brown} on page \pageref{thm:brown}).

It follow from the commutative diagram that $C^*(\mathcal{G})$ is \textit{not} AFE if, and only if, there is an $F \in C_c(X, c^{-1}(0))$ and if there are nonzero functions $f \in C_c(X, \mathbb{Z})$, $h \in C_c(X, \mathbb{N})$ such that
\begin{align}
\label{eqn:maincondition2}
\sigma_\ast(f) - f = h + \partial_1 F.
\end{align}

We simplify the condition above by excluding $\partial_1 F$ from the equation. As we will see, for a sufficiently large $n$, we have $\sigma_\ast^n (\partial_1 F) = \partial_1 \sigma_\ast^n (F) = 0$. If we let $\widetilde{f} = \sigma_\ast^n(f)$, $\widetilde{h} = \sigma_\ast^n(h)$ and if we apply $\sigma_\ast^n$ to both sides of \eqref{eqn:maincondition2}, we get
\begin{align}
\label{eqn:maincondition3}
\sigma_\ast(\widetilde{f}) - \widetilde{f} = \widetilde{h}.
\end{align}
With this equation, we obtain the condition \eqref{eqn:maincondition} by negation.

We begin this chapter by defining $\sigma_\ast(F)$ for functions $F \in C_c(c^{-1}(0), \mathbb{Z})$, using the fact that $c^{-1}(0)$ is the increasing union of the sets $R(\sigma^n)$.

\begin{lemma}
\label{lemma:sigmaastRsigma}
Fix $n \in \mathbb{N}$ and let $F \in C_c(R(\sigma^n), \mathbb{Z})$. We define $\sigma_\ast(F) \in C_c(R(\sigma^n), \mathbb{Z})$ by
\begin{align}
\label{eqn:sigmaastRsigma}
 \sigma_\ast(F)(x,y) = \sum_{\substack{u: \hphantom{f} \sigma(u) = x \\ v: \hphantom{f} \sigma(v) = y}} F(u,v).
\end{align}
Then $\sigma_*(F)$ is well-defined. In particular, if $n \geq 1$, we have $\sigma_\ast(F) \in C_c(R(\sigma^{n-1}), \mathbb{Z})$.
\end{lemma}
\begin{proof}
When $n = 0$, this map is well-defined because we identify $R(\sigma^0)$ with $X$ and then apply Definition \ref{def:sigmaast}.

Fix $n \geq 1$. Note that $C_c(R(\sigma^n), \mathbb{Z})$ is spanned by the characteristic functions of the sets
\begin{align*}
\mathcal{U}_{A,B}^{n}  = \lbrace (x,y) : x \in A, y \in B, \sigma^n(x) = \sigma^n(y) \rbrace,
\end{align*}
for $A, B \subset X$ compact open with $\sigma^n(A) = \sigma^n(B)$, and $\sigma^n$ injective on $A$ and $B$. Since the map $F \mapsto \sigma_\ast^n(F)$ is linear, we only need to show that the map is well-defined for these characteristic functions. In particular, we will show that $\sigma_\ast(1_{\mathcal{U}_{A,B}^{n}}) = 1_{\mathcal{U}_{\sigma(A),\sigma(B)}^{n-1}} \in C_c(R(\sigma^{n-1}), \mathbb{Z})$. In fact,
\begin{itemize}
\item Suppose $1_{\mathcal{U}_{\sigma(A),\sigma(B)}^{n-1}}(x,y) = 1$.

Then $(x,y) \in \mathcal{U}_{\sigma(A),\sigma(B)}^{n-1}$.

Then there exists $u \in A$ and $v \in B$ with $\sigma(u) = x$ and $\sigma(v) = y$. Moreover,
\begin{align*}
\sigma^n(u) = \sigma^{n-1}(\sigma(x)) = \sigma^{n-1}(\sigma(y)) = \sigma^n(v).
\end{align*}
Since $\sigma$ is injective on $A$ and $B$, such $(u,v)$ is unique. By equation \eqref{eqn:sigmaastRsigma}, we have that
\begin{align*}
\sigma_\ast(1_{\mathcal{U}_{A,B}^{n}})(x,y) = 1_{\mathcal{U}_{A,B}^{n}}(u,v) = 1.
\end{align*}
\item Suppose $\sigma_\ast(1_{\mathcal{U}_{A,B}^n})(x,y) \neq 0$.

Then, by \eqref{eqn:sigmaastRsigma} there are $u,v$ such that
\begin{align*}
& \sigma(u) = x, \text{\hspace{10pt}}
\sigma(v) = y, \text{\hspace{10pt}}
\sigma^n(u) = \sigma^n(v), \text{\hspace{10pt}}
u \in A,\text{\hspace{10pt}and }
v \in B.
\end{align*}
Since $\sigma$ is injective on $A$ and $B$, it follows that $u, v$ are unique. Thus we have $\sigma_\ast(1_{A,B}^n)(x,y) = 1$. Moreover,
\begin{align*}
&
x \in \sigma(A), \text{\hspace{10pt}}
y \in \sigma(B), \text{\hspace{10pt}}
\sigma^{n-1}(x) = \sigma^{n-1}(y)\\
\Rightarrow\text{\hspace{10pt}}&
(x,y) \in \mathcal{U}_{\sigma(A),\sigma(B)}^{n-1}\\
\Rightarrow\text{\hspace{10pt}}&
1_{\mathcal{U}_{\sigma(A),\sigma(B)}^{n-1}}(x,y) = 1.
\end{align*}
\end{itemize}
Therefore $\sigma_\ast(1_{\mathcal{U}_{A,B}^{n}}) = 1_{\mathcal{U}_{\sigma(A),\sigma(B)}^{n-1}}$.
\end{proof}

\begin{remark}
Note that the definition above coincides with Definition \ref{def:sigmaast} of page \pageref{def:sigmaast} when $F \in C_c(c^{-1}(0), \mathbb{Z})$ has support on the unit space, that we identify with $X$. In this case, we have
for $x \in X$,
\begin{align*}
\sigma_\ast F(x)
= \sum_{\substack{y: \sigma(y) = x \\ z: \sigma(z) = x}} F(y,z)
= \sum_{y: \sigma(y) = x} F(y).
\end{align*}
\end{remark}

Now we prove that $\sigma_\ast$ and $\partial_1$ commute.

\begin{lemma}
\label{lemma:partialsigmacommute}
Let $F \in C_c(R(\sigma^n), \mathbb{Z})$. Then $\partial_1^{(n)}(\sigma_\ast(F)) = \sigma_\ast(\partial_1^{(n)}(F))$. Here, $\partial_1^{(n)}: C_c(R(\sigma^n), \mathbb{Z}) \rightarrow C_c(X, \mathbb{Z})$ denotes the operator from Lemma \ref{lemma:partial1F}.
\end{lemma}
\begin{proof}
Note that the result holds for $n = 0$ because $\partial_1^{(0)} = 0$. Fix $n \geq 1$ and let $x \in X$. Then
\begin{align*}
\sigma_\ast(\partial^{(n)}_1(F))(x)
&= \sum_{y: \sigma(y) = x} \partial_1^{(n)}(F)(y) \\
&= \sum_{y: \sigma(y) = x} \left(\sum_{z: \sigma^n(z) = \sigma^n(y)} [F(z,y) - F(y,z)] \right)\\
&= \sum_{y: \sigma(y) = x} \left( \sum_{z: \sigma^n(z) = \sigma^{n-1}(x)} [F(z,y) - F(y,z)] \right) \hspace{30pt}\text{because $n \geq 1$,} \\
&= \sum_{y: \sigma(y) = x} \left( \sum_{v: \sigma^{n-1}(v) = \sigma^{n-1}(x)} \left( \sum_{z: \sigma(z) = v} [F(z,y) - F(y,z)] \right) \right) \\
&= \sum_{v: \sigma^{n-1}(v) = \sigma^{n-1}(x)} \left( \sum_{\substack{y: \sigma(y) = x \\ z:\sigma(z) = v}} [F(z,y) - F(y,z)] \right)\\
&= \sum_{v: \sigma^{n-1}(v) = \sigma^{n-1}(x)} [\sigma_\ast(F)(v,x) - \sigma_\ast(F)(x,v)] \\
&= \partial_1^{(n-1)}(\sigma_\ast(F))(x)
%&= \partial_1^{(n)}(\sigma_\ast(F))(x).
\end{align*}
Note that $\sigma_\ast(F) \in C_c(R(\sigma^{n-1}), \mathbb{Z})$ by Lemma \ref{lemma:sigmaastRsigma}. Then $\partial^{(n)}_1(\sigma_\ast(F)) = \partial^{(n-1)}_1(\sigma_\ast(F))$ by Lemma \ref{lemma:partial1F}. Therefore $\sigma_\ast(\partial_1^{(n)}(F)) = \partial_1^{(n)}(\sigma_\ast(F))$.
\end{proof}

%Recall from the introduction that the C*-algebra $C^*(\mathcal{G})$ is AF embeddable if, and only if, $H_\beta \cap H_0(B)^+ = \lbrace 0 \rbrace$. Using the commutative diagram from the previous section, we prove the theorem below, that gives a condition on $\sigma$ that characterises when $C^*(\mathcal{G})$ is AFE.

Now we prove our main result. The following theorem finds a condition on $\sigma$ that characterises when $C^*(\mathcal{G})$ is AFE.

%Let $B = C^*(\mathcal{G}(c))$. We outline the proof as follows: first we use the isomorphism $\omega: C^*(\mathcal{G}) \rtimes_{\alpha^c} \mathbb{T} \rightarrow C^*(G(c))$ of Proposition \ref{prop:omega} to find an action $\beta: \mathbb{Z} \rightarrow \mathrm{Aut}(B)$ induced from $\alpha^c$. Then we can apply Brown's theorem (Theorem \ref{thm:brown}) and get the following condition:
%\begin{align*}
%C^*(\mathcal{G}) \rtimes_{\alpha^c} \mathbb{T} \rtimes_{\widehat{\alpha^c}} \mathbb{Z} \text{ is AFE }
%\Leftrightarrow
%C^*(\mathcal{G}(c)) \rtimes_\beta \mathbb{Z}
%\text{ is AFE }
%\Leftrightarrow
%H_\beta \cap K_0(B)^+ = \lbrace 0 \rbrace.
%\end{align*}
%Recall from Takai duality (Theorem \ref{thm:Takaiduality}) that $C^*(\mathcal{G}) \rtimes_{\alpha^c} \mathbb{T} \rtimes_{\widehat{\alpha}^c} \mathbb{Z}$ is stably isomorphic to $C^*(\mathcal{G})$. Since the AFE property is preserved by stable isomorphisms, we have
%\begin{align*}
%C^*(\mathcal{G}) \text{ is AFE }
%\Leftrightarrow
%H_\beta \cap K_0(B)^+ = \lbrace 0 \rbrace.
%\end{align*}
%We will use the commutative diagram of the previous section to a condition on $\sigma$ that characterises the AFE property.

%Let us find the action $\beta$ on $C^*(\mathcal{G}(c))$.

\begin{customthm}{1}
%\label{thm:AFEDR}
The following are equivalent:
\begin{enumerate}[(i)]
\item $C^*(\mathcal{G})$ is AFE,
\item $C^*(\mathcal{G})$ is quasidiagonal,
\item $C^*(\mathcal{G})$ is stably finite,
\item $\mathrm{Im}(\sigma_\ast - \mathrm{id}) \cap C_c(X, \mathbb{N}) = \lbrace 0 \rbrace$.
\end{enumerate}
\end{customthm}
\begin{proof}
Let $c: \mathcal{G} \rightarrow \mathbb{Z}$ be the continuous cocycle given by $c(x,k,y) = k$ for $(x,k,y) \in \mathcal{G}$. By \cite[Corollary 5.2]{FKPS}, we have that $\mathcal{G}(c)$ is an AF groupoid. Let $B = C^*(\mathcal{G}(c))$. Then $C^*(\mathcal{G}(c))$ is AF.

Let $\beta$ be the action on $B$ from Section \ref{subsection:crossedproducts:beta}. Brown's theorem (Theorem \ref{thm:brown}) gives the equivalence of the for conditions below.
\begin{enumerate}[(i')]
\item $B \rtimes_\beta \mathbb{Z}$  is AFE,
\item $B \rtimes_\beta \mathbb{Z}$ is quasidiagonal,
\item $B \rtimes_\beta \mathbb{Z}$ is stably finite,
\item $H_{\beta} \cap K_0(B)^+ = \lbrace 0 \rbrace$.
\end{enumerate}

By Proposition \ref{prop:beta}, $B \rtimes_\beta \mathbb{Z}$ and $C^*(\mathcal{G}) \rtimes_{\alpha^c} \mathbb{T} \rtimes_{\widehat{\alpha}^c} \mathbb{Z}$ are isomorphic. By Takai duality, $C^*(\mathcal{G}) \rtimes_{\alpha^c} \mathbb{T} \rtimes_{\widehat{\alpha}^c} \mathbb{Z}$ and $C^*(\mathcal{G})$ are stably isomorphic. So $B \rtimes_\beta \mathbb{Z}$ and $C^*(\mathcal{G})$ are stably isomorphic.

Since AF embeddability, quasidiagonality and stable finiteness are preserved under stable isomorphisms, we have the equivalence below:
\begin{enumerate}[(i)]
\item $C^*(\mathcal{G})$  is AFE,
\item $C^*(\mathcal{G})$ is quasidiagonal,
\item $C^*(\mathcal{G})$ is stably finite,
\item[\refstepcounter{enumi}(iv')] $H_{\beta} \cap K_0(B)^+ = \lbrace 0 \rbrace$.
\end{enumerate}

Now we study the condition (iv'). By the commutative diagram, (iv') is false if, and only if, there are $f \in C_c(X, \mathbb{Z})$ and $h \in C_c(X, \mathbb{N})$ such that
\begin{align}
\label{eqn:AFEDR1}
[\sigma_\ast(f) - f] = [h].
\end{align}
Suppose \eqref{eqn:AFEDR1} holds. Then there exists $F \in C_c(c^{-1}(0), \mathbb{Z})$ such that
\begin{align*}
%\label{eqn:AFEDR2}
\sigma_\ast(f) - f = h + \partial_1 F.
\end{align*}
By the topological properties of $c^{-1}(0)$, there exists $n \geq 0$ such that $F \in C_c(R(\sigma^n), \mathbb{Z})$. By Lemma \ref{lemma:partial1F}, we have
\begin{align}
\label{eqn:AFEDR2}
\sigma_\ast(f) - f = h + \partial_1^{(n)} F.
\end{align}
Recall from Lemma \ref{lemma:sigmaastRsigma} that $\sigma_\ast^n(F) \in C_c(X, \mathbb{Z})$. Then $\partial_1(\sigma_\ast^n(F)) = 0$.

Let $\widetilde{f} = \sigma_\ast^n(f)$ and $\widetilde{h} = \sigma_\ast(h)^n \in C_c(X, \mathbb{N})$. By applying $\sigma_\ast^n$ to both sides to equation \ref{eqn:AFEDR2}, we obtain
\begin{align*}
\sigma_\ast(\widetilde{f}) - \widetilde{f}
&= \widetilde{h} + \sigma_\ast^n(\partial_1^{(n)} F) \\
&= \widetilde{h} + \partial_1^{(n)}(\sigma_\ast^n( F))
\hspace{15pt}\text{by Lemma \ref{lemma:partialsigmacommute}}\\
&= \widetilde{h}.
\end{align*}
We have just proved that if $C^*(\mathcal{G})$ is not AFE, then $\mathrm{Im}(\sigma_\ast - \mathrm{id}) \cap C_c(X, \mathbb{N}) \neq \lbrace 0 \rbrace$. We will prove the converse.

Now suppose that $\mathrm{Im}(\sigma_\ast - \mathrm{id}) \cap C_c(X, \mathbb{N}) \neq \lbrace 0 \rbrace$. Then there are $f \in C_c(X, \mathbb{N})$ and $h \in C_c(X, \mathbb{N})$ such that
\begin{align*}
\sigma_\ast(f) - f = h.
\end{align*}
Then equation (iv') holds, which implies that $C^*(\mathcal{G})$ is not AFE.
\end{proof}

\begin{corollary}
\label{corollary:sigmanNotAFE}
Let $X$ be a locally compact Hausdorff second countable totally disconnected space. Let $\sigma: X \rightarrow X$ be a surjective local homeomorphism. Let $\mathcal{G}$ be the Deaconu-Renault groupoid. Then the following are equivalent:
\begin{enumerate}[(1)]
\item $C^*(\mathcal{G})$ is AFE,
\item $\mathrm{Im}(\sigma_\ast - \mathrm{id}) \cap C_c(X, \mathbb{N}) = \lbrace 0 \rbrace$,
\item $\mathrm{Im}(\sigma_\ast^n - \mathrm{id}) \cap C_c(X, \mathbb{N}) = \lbrace 0 \rbrace$ for some $n \geq 1$, and
\item $\mathrm{Im}(\sigma_\ast^n - \mathrm{id}) \cap C_c(X, \mathbb{N}) = \lbrace 0 \rbrace$ for all $n \geq 1$.
\end{enumerate}
\end{corollary}
\begin{proof}
The equivalence $(1) \Leftrightarrow (2)$ follows from Theorem \ref{thm:AFEDR}. The implications $(4) \Rightarrow (2) \Rightarrow (3)$ are straightforward. We show $(3) \rightarrow (4)$ by contrapositive.

Suppose (4) is false. Then, for some $m \geq 1$, there are nonzero $f \in C_c(X, \mathbb{Z})$ and $h \in C_c(X, \mathbb{N})$ such that $\sigma_\ast^m(f) - f = h$. Let $n \geq 1$ be arbitrary. Then, for all $k = 0, 1, \dots, n$, we have
\begin{align*}
\sigma_\ast^k(\sigma_\ast^m(f)) - \sigma_\ast^k(f) = \sigma_\ast^*(f).
\end{align*}

Let $F = \sigma_\ast^m(f)$ and $H = h + \sigma_\ast(h) + \dots + \sigma_\ast^{n-1}(h)$. Note that $H \in C_c(X, \mathbb{N})$ and is nonzero. By a telescoping sum, we have
\begin{align*}
\sigma_\ast^n(F) - F
&= \sigma_\ast^n(\sigma_\ast(f)) - \sigma_\ast^m(f) \\
&= \sum_{k=0}^{n-1} [ \sigma_\ast^{k+1}(\sigma_\ast^m(f)) - \sigma_\ast^k(\sigma_\ast^n(f))] \\
&= \sum_{k=0}^{n-1} \sigma_\ast^k(h) \\
&= H.
\end{align*}
Thus $\mathrm{Im}(\sigma_\ast^n - \mathrm{id}) \cap C_c(X, \mathbb{N}) \neq \lbrace 0 \rbrace$. Since $n$ is arbitrary, $(3)$ is false. Therefore, $(3) \Rightarrow (4)$.
\end{proof}

\begin{remark}
\label{rmk:sigmakgeq}
Using the same telescoping sums of the corollary before, we can show that, for $f \in C_c(X, \mathbb{Z})$ satisfying $\sigma_\ast(f) \geq f$, we have $\sigma_\ast^n(f) \geq \sigma_\ast^{n-1}(f) \geq \hdots \geq f$ for all $n \geq 1$.  This property will be useful in Corollary \ref{corollary:graphAFE} on page \pageref{corollary:graphAFE}, where we study the AFE property of graph algebras as an example of our main theorem.
\end{remark}


==> template/binding.tex <==
\chapter{Binding}\label{C:bin}

The Library states:
\begin{itemize}
\item Thesis must be fully bound and cased in cloth or buckram in optional colour. (I think they mean you can pick the colour!)
\item Author's surname and initials and (short) title lettered on spine. (The thesis's title, not the author's, presumably.)
\item Author's full name and full title lettered on front cover. (Again, the thesis's title, not the author's, presumably.)
\item Two copies of a PhD thesis and one copy of a Master's thesis must be deposited. A signed availability slip must accompany the thesis.
\item  The principal supervisor is responsible for the deposit.
\end{itemize}

==> template/library.tex <==
\chapter{Library requirements}\label{C:lib}

This Chapter describes some things done to be in accordance with the `Library Requirements for the Deposit of Theses' booklet, which can be obtained from the VUW library.

\section{Font size}
\textit{12 point font is recommended.} 

Set this yourself with the \verb+12pt+ option to the document class.

\section{Single or double sided}
\textit{Typing on one side preferred, text on both sides acceptable for longer works.} 

Use the \verb+oneside+ or \verb+twoside+ option to the document class. The \textsf{book} class default is \verb+twoside+.


\section{Line spacing}
\textit{Lines should be double spaced, or at least 1.5 spaces apart.} 

1.5 spacing for 12 point is set using:
\begin{itemize}
\item \verb+\renewcommand{\baselinestretch}{1.24}+  
\end{itemize}

To set anything else use, e.g  \verb+\renewcommand{\baselinestretch}{1.0}+ in the preamble. See p 53 of \cite{GMS94} for more information.


\section{Margins}
\textit{Uniform margins of at least 4cm on binding side, other three sides to have at least 1.5 cm}

\LaTeX\ styles often leave a lot of white space, and \textsf{book} is no exception. We only have to worry about the binding side.

For \verb+twoside+ we use these settings:
\setlength{\textheight}{19.8cm}
\setlength{\oddsidemargin}{1.46cm}
\setlength{\evensidemargin}{0.83cm}

For \verb+oneside+, if we use:
\begin{verbatim}
\setlength{\textheight}{19.8cm}
\setlength{\oddsidemargin}{1.46cm}
\end{verbatim}

Then \textsf{book} gives a margin of 4cm on the binding side, and about 3.2cm elsewhere.

If you want to change these then use the \textsf{layout} package.

\section{Paper size}
\textit{High quality A4 paper, all pages of equal size}

Set this yourself with the \verb+a4paper+ option to the document class.

==> template/thesis-acknowledge.tex <==
\chapter*{Acknowledgments}\label{C:ack} 

Any acknowledgments should go in here, between the title page and the
table of contents.  The acknowledgments do not form a proper chapter,
and so don't get a number or appear in the table of contents.


==> template/thesis-conclusion.tex <==
\chapter{Conclusions}\label{C:con}

If all the economists in the world were laid end-to-end they wouldn't
reach a conclusion, and neither shall I.


==> template/thesis-introduction.tex <==
\chapter{Introduction}\label{C:intro}
The \textsf{vuwthesis} style attempts to do 2 things:
\begin{enumerate}
\item produce the correct front pages -- explained in Chapter \ref{C:ex};
\item meet the library requirement for the deposit of theses -- explained in Chapter \ref{C:lib}.
\end{enumerate}

We try to set the front pages up after the fashion of the example on p58
of the 2002 PhD handbook. (Available at
\url{http://www2.vuw.ac.nz/home/publications/phd_handbook.pdf}, March
2003).

I assume that you are using \textsf{report.sty} or, preferably,
\textsf{book.sty}. The book style has things like \verb+\frontmatter+
defined, which make life a little easier. 

Although the style alters the margins, and so on,  if you'd prefer to do
something else then feel free to set them all yourself. In this case you
will probably want to look at the \textsf{layout} package.

==> template/thestyle.tex <==
\chapter{The front pages}\label{C:ex}

You can declare:
\begin{itemize}
\item an author using  \verb+\author{}+ -- your full name;
\item a title using \verb+\title{}+-- ALL IN CAPITALS IN THE EXAMPLE, but we use \verb#\Large# and \verb#\bf#, so normal case will do;
\item a subject using \verb+\subject{}+-- probably Computer Science, but you can pick anything you like;
\item an abstract using \verb+\abstract{}+-- this should be fewer then 500 words for a PhD. The handbook states ``A length of about 300 words is recommended.'' The \textsf{book} style does not have an \verb+abstract+ environment defined, so this is a bit of a hack.
\end{itemize}

You can also specify what degree you are submitting the thesis for by using:
\begin{itemize}
\item  \verb+\phd+, which produces ``\ldots in fulfilment of \ldots Doctor of Philosophy''
\item  \verb+\mscthesisonly+, which produces ``\ldots in fulfilment of \ldots Master of Science''
\item  \verb+\mscwithhonours+, which produces ``\ldots in partial fulfilment of \ldots Master of Science with Honours''
\item  \verb+\mscbothparts+, which produces ``\ldots in partial fulfilment of \ldots Master of Science''
\item  \verb+\otherdegree{DEGREE OR DIPLOMA NAME}+, which produces ``\ldots in fulfilment of \ldots DEGREE OR DIPLOMA NAME''
\end{itemize}


==> teste.tex <==
\chapter{Introduction}
\label{C:intro}
A problem that has received much interest during the last decades is the classification of C*-algebras. This problem consists of finding an invariant that identifies all C*-algebras of a certain class up to isomorphism. One of the first results in the area is Glimm's \cite{Glimm} classification of some uniformly hyperfinite C*-algebras. Glimm's result was interesting because uniformly hyperfinite algebras are the C*-algebraic version of the $\text{II}_1$ %factors for von Neumann algebras, but unlike the von Neumann case \cite{MurrayvonNeumann} (see also \cite[Theorem V.1.13]{Connes}), uniformly hyperfinite C*-algebras are not all isomorphic.


==> thesis-conclusion.tex <==
\chapter{Conclusions}\label{C:con}

If all the economists in the world were laid end-to-end they wouldn't
reach a conclusion, and neither shall I.


==> thesis-introduction.tex <==
\chapter{Introduction}\label{C:intro}
The \textsf{vuwthesis} style attempts to do 2 things:
\begin{enumerate}
\item produce the correct front pages -- explained in Chapter \ref{C:ex};
\item meet the library requirement for the deposit of theses -- explained in Chapter \ref{C:lib}.
\end{enumerate}

We try to set the front pages up after the fashion of the example on p58
of the 2002 PhD handbook. (Available at
\url{http://www2.vuw.ac.nz/home/publications/phd_handbook.pdf}, March
2003).

I assume that you are using \textsf{report.sty} or, preferably,
\textsf{book.sty}. The book style has things like \verb+\frontmatter+
defined, which make life a little easier. 

Although the style alters the margins, and so on,  if you'd prefer to do
something else then feel free to set them all yourself. In this case you
will probably want to look at the \textsf{layout} package.

==> thestyle.tex <==
\chapter{The front pages}\label{C:ex}

You can declare:
\begin{itemize}
\item an author using  \verb+\author{}+ -- your full name;
\item a title using \verb+\title{}+-- ALL IN CAPITALS IN THE EXAMPLE, but we use \verb#\Large# and \verb#\bf#, so normal case will do;
\item a subject using \verb+\subject{}+-- probably Computer Science, but you can pick anything you like;
\item an abstract using \verb+\abstract{}+-- this should be fewer then 500 words for a PhD. The handbook states ``A length of about 300 words is recommended.'' The \textsf{book} style does not have an \verb+abstract+ environment defined, so this is a bit of a hack.
\end{itemize}

You can also specify what degree you are submitting the thesis for by using:
\begin{itemize}
\item  \verb+\phd+, which produces ``\ldots in fulfilment of \ldots Doctor of Philosophy''
\item  \verb+\mscthesisonly+, which produces ``\ldots in fulfilment of \ldots Master of Science''
\item  \verb+\mscwithhonours+, which produces ``\ldots in partial fulfilment of \ldots Master of Science with Honours''
\item  \verb+\mscbothparts+, which produces ``\ldots in partial fulfilment of \ldots Master of Science''
\item  \verb+\otherdegree{DEGREE OR DIPLOMA NAME}+, which produces ``\ldots in fulfilment of \ldots DEGREE OR DIPLOMA NAME''
\end{itemize}

